Computing Local Sensitivities of Counting Queries with Joins

Local sensitivity of a query Q given a database instance D, i.e. how much the output Q(D) changes when a tuple is added to D or deleted from D, has many applications including query analysis, outlier detection, and in differential privacy. However, it is NP-hard to find local sensitivity of a conjunctive query in terms of the size of the query, even for the class of acyclic queries. Although the complexity is polynomial when the query size is fixed, the naive algorithms are not efficient for large databases and queries involving multiple joins. In this paper, we present a novel approach to compute local sensitivity of counting queries involving join operations by tracking and summarizing tuple sensitivities -- the maximum change a tuple can cause in the query result when it is added or removed. We give algorithms for the sensitivity problem for full acyclic join queries using join trees, that run in polynomial time in both the size of the database and query for an interesting sub-class of queries, which we call 'doubly acyclic queries' that include path queries, and in polynomial time in combined complexity when the maximum degree in the join tree is bounded. Our algorithms can be extended to certain non-acyclic queries using generalized hypertree decompositions. We evaluate our approach experimentally, and show applications of our algorithms to obtain better results for differential privacy by orders of magnitude.

==> acyclicjoin.tex <==
\section{Acyclic Join Query}\label{sec:acyclic}

\begin{algorithm}[t]
	\scriptsize
	\caption{Compute Local Sensitivity of an Acyclic Join Query and the corresponding Most Sensitive Tuple}
	\label{algo:as_pathquery}
	\begin{algorithmic}[1]
		\Require Acyclic join query
		$\Qajoin(\attr_0 \ldots \attr_m)$, the database $\database$
		\Ensure The local sensitivity $\LS$, and the most sensitive tuple $\kingtuple$
		\Procedure {LS}{$\Qajoin, \database$}
		\Statex I) Prepare botjoin
		\For{$i$ in postoder}
		\If{$\R{i}$ is a leaf}
		\State $\botjoin(\R{i}) = \aggregate{\attributes_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{R_i}$
		\Else
		\State $T = \aggregate{\attributes_{i, p(i)}, \attributes_j \forall j \in C(i)}{count(*) \as C_i}{\R{i}}$
		\State $S = \Qsjoin(T, \{\botjoin(\R{j})  \mid j \in C(i) \})$
		\State $\botjoin(\R{i}) = \aggregate{\attributes_{i,p(i)}}{sum(C_i \underset{j \in C(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}} S$
		\EndIf
		\EndFor
		\Statex II) Prepare topjoin
		\For{$i$ in preoder}
		\If{$\R{i}$ is the root}
		\State pass
		\Else
		\State $T = \aggregate{\attributes_{i, p(i)}, \attributes_{p(i), p(p(i))}, \attributes_j \forall j \in C(i)}{count(*) \as C_i}{\R{p(i)}}$
		\State $S = \Qsjoin(T, \{\topjoin(\R{p(i)})\} \cup \{\botjoin(\R{j})  \mid j \in N(i) \})$
		\State $\botjoin(\R{i}) =\aggregate{\attributes_{i,p(i)}}{sum(C_i \cdot \cntt{p(i)}{p(p(i))} \cdot  \underset{j \in N(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}}{S}$
		\EndIf
		\EndFor
		\Statex III) Select most sensitive tuple
		\For{$i=1, \dots, m$}
		\If {$\R{i}$ is the root}
		\State $\Qafreq^i = \pi_{\attributes_{i}, ~ \underset{j \in C(i)}{\product} \cntt{i}{j} \as  \tsens_i} \underset{\forall j \in C(i)}{\superjoin} \botjoin(\R{j})$		
		\ElsIf {$\R{i}$ is a leaf}
		\State $\Qafreq^i = \pi_{\attributes_{i}, ~ \cntt{i}{p(i)} \as  \tsens_i} \topjoin(\R{j})$
		\Else 
		\State $\Qafreq^i = \pi_{\attributes_{i}, ~ \cntt{i}{p(i)} \underset{j \in C(i)}{\product} \cntt{i}{j} \as  \tsens_i}
		\big( \topjoin(\R{i}) \superjoin ( \underset{\forall j \in C(i)}{\superjoin} \botjoin(\R{j})) \big)$
		\EndIf
		\State $t_i = \argmax_{\tsens} \pi_{\tsens_i \as \tsens} T$
		\EndFor
		\State $t = \argmax_{\tsens}{t_1, \ldots, t_m}$
		\State $\LS = t.\tsens$
		\State $\kingtuple = t.\attributes$
		\State \textbf{return} $\LS, \kingtuple$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

\todo{State what I'm going to do in this section. Repeat this to each section.}

\note{A conjunction tree}

Path join queries only cover a small subset of all conjunctive queries. There is a more general class, called acyclic join queries, that not only covers path join queries, but also shares good characteristics for efficient evaluation. 


Acyclic join queries can always be written into a join plan such that each operation is polynomial in time and space. 

For a conjunctive query $q$, we define $H(q) = (V, E)$ as a hypergraph of $q$ such that $V$ contains all attributes from $q$ and each hyperedge of $E$ includes every attribute from the associated relation. \note{make a reference}

We denote $GYO$ as the algorithm by Graham, Yu and Ozsoyoglu. It takes a hypergraph as input and iteratively removes hypernodes and hyperedges. A conjunctive query $q$ is acyclic if $GYO(H(q))$ is the empty hypergraph. \note{make a reference}

Consider a general acyclic join in the form as: 
\begin{align*}
\Qajoin(\attributes_\database) = \relation_1(\attributes_1), \ldots, \relation_m(\attributes_m) 
\end{align*}
, where $\attributes_i$ is the attribute set of the table $\relation_i$. We assume $\forall i$, $\attributes_i$ is covered by the union among $\attributes_{p(i)}$ and $\attributes_j$ $\forall j \ in C(i)$. If it is not covered, we simply ignore those attributes that are not covered since they cannot affect the sensitivity.

\subsection{General Approach}
To compute the local sensitivity of an acyclic join, the general approach is similar to the one of the path join case. 

(1) For path join queries, we define $\Qajoin^i(\attributes_\database)$ as:
\begin{align}\label{eq:general_aj_sub_query}
\Qajoin^i(\attributes_\database)
\datalogEQ
& \relation_1(\attributes_1), \ldots, \relation_m(\attributes_{i-1}), \nonumber \\
& \relation_1(\attributes_{i+1}), \ldots, \relation_m(\attributes_m) 
\end{align}
which is a sub-query from the original acyclic join query by removing the relation $\relation_i$. 

(2) Then we do a counting group by on attributes $\attributes_i$.
\begin{align}\label{eq:general_aj_freq}
\Qafreq^i(\attributes_\database) = {\aggregate{\attributes_i}{count(*) \as c}{\Qajoin^i(\attributes_\database)}}
\end{align}
to count the frequency of each tuple.

(3) To find the most sensitive tuple, we pick the tuple from the above query who has the largest frequency $c$.
\begin{align} \label{eq:general_aj_most_sensitive_tuple}
t^*_i = \argmax_{c} \Qafreq^i(\attributes_\database)
\end{align}

\begin{proposition}
	The $t^*_i$ from the equation \ref{eq:general_aj_most_sensitive_tuple} contains the most sensitive tuple as $t^*_i.\attributes_i$ and its tuple frequency $t^*_i.c$ from the domain of table $\relation_i$.
\end{proposition}
\begin{proof}
	By definition, equation (\ref{eq:general_aj_freq}) computes the tuple sensitivity as $count(*)$ $\as$ $c$ for each $\attributes_i$ appears in $\Qajoin^i(\attributes_\database)$. We further show that these tuples forms the \representative domain $\reprdomain^{\attributes_i}$.
	\todo{Change the rest of the proof} The cross product of $\topjoin(R_{i})$ and $\botjoin(R_{i+1})$ includes all tuples from $\actdomain^{A_{i-1}} \times \actdomain^{A_{i}}$, which by definition is the representative domain $\reprdomain^{A_{i-1},A_{i}}$ about $\R{i}$.  Since all tuples outside this domain has sensitivity 0, searching tuples within this domain can guarantee finding the global most sensitive tuple and corresponding sensitivity. 
\end{proof}

\todo{change the statement. Even the third step is exponential in combined complexity}

Although this approach gives us the correct result, the size of the sub-query $\Qajoin^i(\attributes_\database)$ in worst case could be $O(n^{m-1})$.
%which is also linearly related to the time complexity of evaluating this sub-query and finding the most frequent tuple. 
In conclusion, this naive approach is polynomial in data complexity, but may be exponential in combined complexity.


\subsection{Algorithm Details}

\todo{Equivalence: correctness}

\todo{efficiency analysis: not efficient}

\note{make a reference} According to the $GYO$ algorithm, it can also be expressed by a join tree $T(V,E)$, where $V=\{R_1,\ldots,R_m\}$, and $E=\{\attributes_{i,j}| R_i \bowtie R_j \in \Qajoin\}$. 
We denote the set of join attributes between $R_i$ and $R_j$ by $\attributes_{i,j}$.
As $T$ is a tree, $|E| = m$. As $\Qajoin$ is acyclic, if an attribute $A$ that appear in node $R$
and not its parent in the join tree, this attribute will not appear in any ancestor.
Let $p(i)$ denote the index of the parent of node $R_i$ in the join tree,
$C(i)$ denote the set of indices of the children of $R_i$,
and $N(i)$ denote the set of indices of the neighbors of $R_i$, i.e. $C(p(i)) \setminus \{i\}$.

We denote $\subtree(R_i)$ as the subtree rooted at $R_i$, while $\comptree(R_i)$ is the complementary graph of $\subtree(R_i)$ on the tree $T(V, E)$.

\todo{I need a symbol that is either a cross-product or natural join. Here the command name is superjoin}

Now we can rewrite the equation (\ref{eq:general_aj_sub_query}) in step (1) as 
\begin{align}
\Qajoin^i(\attributes_\database) = \comptree(R_i) \superjoin \underset{\forall j \in C(i)}{\superjoin} \subtree(R_j)
\end{align}

\begin{figure}
	%\centering
	\includegraphics[scale=0.45]{acyclic_join_recursion.pdf}
\end{figure}

Given a table $R_i$ in $T$, as long as we know the maximum frequency of tuples projected on $\attributes_i$ from the joint output between tables other than $R_i$ in a join tree of $\Qajoin$, as defined by $\Qajoin^i$, we immediately get the max change to the final joint output due to adding or removing a tuple to $R_i$, and hence the local sensitivity of the query. We define the following invariants to compute the tuple sensitivity of an acyclic query.

For each table $R_i$, we denote $\botjoin(R_i)$ and $\topjoin(R_i)$ as tables that computes the frequency of tuples projected on attributes shared by $\relation_i$ and its parent $\relation_{p(i)}$ from $\subtree(\R{i})$ and $\comptree(\R{i})$.
\begin{align}
\botjoin(R_i) &=  \aggregate{A_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{T(\R{i})}
\\
\topjoin(R_i) &= \aggregate{A_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{\comptree(\R{i})}
\end{align}

Now, equation (\ref{eq:general_aj_freq}) can be rewritten as:
\begin{align}
\Qafreq^i =  \pi_{\attributes_{i}, ~ \cntt{i}{p(i)} \underset{j \in C(i)}{\product} \cntt{i}{j} \as  \tsens_i}
\big( \topjoin(\R{i}) \superjoin ( \underset{\forall j \in C(i)}{\superjoin} \botjoin(\R{j})) \big)
\end{align}
For corner cases,
\begin{align}
&\Qafreq^i = \nonumber \\
&\begin{cases}
\pi_{\attributes_{i}, ~ \underset{j \in C(i)}{\product} \cntt{i}{j} \as  \tsens_i} \underset{\forall j \in C(i)}{\superjoin} \botjoin(\R{j}) &, \text{$\R{i}$ is the root} \\
\pi_{\attributes_{i}, ~ \cntt{i}{p(i)} \as  \tsens_i} \topjoin(\R{j}) &, \text{$\R{i}$ is a leaf}
\end{cases}
\end{align}

\note{Show why this is equivalent to 8}

\note{Explain the algorithm box \ref{algo:as_pathquery}.}

\note{Prove the equivalence of the recursive top/bot join.}

The last step is the same.

Define $\Qsjoin(\R{0}, \R{1} \ldots \R{m})$ as a star join, which can be expressed by a tree $T_S(V, E)$, where V = $\{\R{0}, \R{1} \ldots \R{m}\}$ and E = $\{(\R{0}, \R{i}) \mid i \in \{1 \ldots m\} \}$.

\paratitle{Algorithm} Here is the algorithm box \ref{algo:as_pathquery}. \note{This paragraph is the same as in the path join section. How shall we change it?} The algorithm basically prepares topjoin and botjoin first and then use them to find the most sensitive tuple. Note that computing topjoin (\ref{eq:pj_topjoin}) and botjoin (\ref{eq:pj_botjoin}) again may require exponential combined complexity, so we give an iterative approach in algorithm \ref{algo:as_pathquery} to compute them in polynomial combined complexity. After preparing topjoin and botjoin, the third step is to combine them together and find the most sensitive tuple. We assume all joins are merge-sort joins.

To prepare topjoin (\ref{eq:pj_topjoin}), \note{change this para to match the algorithm} we first compute $\topjoin(\R{2})$ as a base case in the way as topjoin is defined in equation (\ref{eq:pj_topjoin}). Next, we iteratively compute $\topjoin(\R{i})$ for $i$ from 3 to m in the way as:
\begin{align*}
\topjoin(\R{i}) = \aggregate{A_{i-1}}{sum(\cnt{}{i-2}) \as \cnt{}{i-1}}{\topjoin(\R{i-1}) \bowtie \relation_{i-1}}
\end{align*}
\note{Add several steps to show the correctness or equivalence} The correctness follows from replacing $\topjoin(\R{i-1})$ by the definition of topjoin as equation (\ref{eq:pj_topjoin}) shows, and proving by induction.

To prepare botjoin, \note{change this para to match the algorithm} we follow a similar way as preparing topjoin does.

To combine topjoin and botjoin together and find the most sensitive tuple, \note{remove the max boost} we need to construct $\Qpfreq^i(\attributes_\database)$ on top of $\topjoin(\R{i})$ and $\botjoin(\R{i+1})$ as equation (\ref{eq:pj_fast_freq}) shows. Notice that the next step as equation (\ref{eq:general_most_sensitive_tuple}) shows is to choose the tuple from $\Qpfreq^i(\attributes_\database)$ that has the maximum $(\cnt{}{i-1} * \cnt{}{i}) \rightarrow c$. Since $\max(\cnt{}{i-1} * \cnt{}{i}) = \max(\cnt{}{i-1}) * \max(\cnt{}{i})$, we construct two tuples to find the maximum count as lines 14 and 15 shows, and combine together as lines 16 and 17 shows. Lines 10 to 12 are for corner cases. At the end, lines 19 to 21 extract the most sensitive tuple and corresponding sensitivity.



\subsection{Double Acyclic join}

\todo{equivalence: correctness}

\todo{discuss efficiency}

In the previous section, we have shown how to compute topjoin and botjoin efficiently in polynomial time combined complexity. However, for step 2, there is no guarantee that this sub query can be computed by an algorithm in polynomial time combined complexity.

\note{Definition} Here we introduce a sub class of the acyclic join query class: double acyclic join queries. For an acyclic join query $\Qajoin(\attributes_\database)$, if removing one relation from the query body and the remaining query $\Qajoin^i(\attributes_\database)$ is still an acyclic join query, we call this query as a double acyclic join query.

\note{Efficiency} Since it is double acyclic, we can find a query plan to compute step 2 in polynomial time combined complexity. 

\note{We argue that for a double acyclic join query, any acyclic join tree is also a double acyclic join tree.}

The efficiency can be further boosted by propagating the max operator in step 3 to step 2. We leave this as the future work.

\begin{theorem}
	For double acyclic join queries, algorithm~\ref{algo:as_pathquery} computes the local sensitivity of a path join query and also  finds the corresponding most sensitive tuple. The time complexity is $O(mn \log n)$ where $m = $ the number of attributes and $n = |D|$.
\end{theorem}


==> acyclicjoin_old.tex <==



\section{Acyclic Join Query}\label{sec:acyclic}

\todo{5.1 Join tree review by GYO decomposition (short, example) 5.2 Algorithm for general acyclic queries (intuition, pseuudocode, text how it works, correctness, complexity) -- say why it is not poly-time, 5.3 Doubly acyclic (define, and give the algorithm)   }

\todo{How to generate a join tree from a CQ? Using GYO? What is the complexity?}

\label{sec:join_doublyacyclic}
Consider a general acyclic join: $\Qajoin(R_1,\ldots,R_m)$, which can be expressed by a tree $T(V,E)$, where $V=\{R_1,\ldots,R_m\}$, and $E=\{\attributes_{i,j}| R_i\bowtie R_j \in q\}$.
We denote the set of join attributes between $R_i$ and $R_j$ by $\attributes_{i,j}$.
As $T$ is a tree, $|E| = m$. As $\Qajoin$ is acyclic, if an attribute $A$ that appear in node $R$
and not its parent in the join tree, this attribute will not appear in any ancestor.
Let $p(i)$ denote the index of the parent of node $R_i$ in the join tree,
$C(i)$ denote the set of indices of the children of $R_i$,
and $N(i)$ denote the set of indices of the neighbors of $R_i$, i.e. $C(p(i)) \setminus \{i\}$.

We denote $\subtree(R_i)$ as the subtree rooted at $R_i$, while $\comptree(R_i)$ is the complementary graph of $\subtree(R_i)$ on the tree $T(V, E)$.

\begin{figure}
%\centering
\includegraphics[scale=0.45]{acyclic_join_recursion.pdf}
\end{figure}

Given a table $R_i$ in $T$, as long as we know the maximum frequency in the joint output between tables other than $R_i$ in join tree of $\Qajoin$, we can compute the changes to the final joint output if adding or removing any tuple to $R_i$, and hence the local sensitivity of the query. We define the following invariants to compute the tuple sensitivity of an acyclic query.

\subsubsection{Invariant Definition}
For each table $R_i$,
(1)  let $\botjoin(R_i)$ denote the joint output of the sub-tree at $R_i$ in $T$ grouped by the joint attributes between $R_i$ and the parent of $R_i$, i.e.,
\begin{align}
\botjoin(R_i) =  \aggregate{A_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{T(\R{i})}
\end{align}
(2) let $\topjoin(R_i)$ denotes the joint output of the nodes not in the sub-tree of $R_i$ in $T$ grouped by the joint attributes between $\R{i}$ and the parent of $R_i$, i.e.,
\begin{align}
\topjoin(R_i) = \aggregate{A_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{\comptree(\R{i})}
\end{align}

\subsubsection{Computing Tuple Sensitives}
It is similar to the path join case, except that
\begin{align}
&\RTS{i} = \nonumber \\
&\begin{cases}
\pi_{\Ar{i-1} \as \Al{i},~ \Al{i+1} \as \Ar{i},~ C_{i-1}^r * C_{i+1}^l \as  \tsens_i }\\
\big( \topjoin(\R{i}) \leftouterjoin ( \underset{\forall j \in C(i)}{\cartproduct} \botjoin(\R{j})) \big) \\
&, \text{other} \\
\pi_{\Al{i+1} \as \Ar{i}, C_{i+1}^l \as  \tsens_i} ( \underset{\forall j \in C(i)}{\cartproduct} \botjoin(\R{j})) &, \text{$\R{i}$ is the root} \\
\pi_{\Ar{i-1} \as \Al{i}, C_{i-1}^r \as  \tsens_i} \topjoin(\R{i}) &, \text{$\R{i}$ is a leaf}
\end{cases}
\end{align}



\subsubsection{Correctness Analysis}

\begin{theorem}
$\RTS{i}$ covers tuples from the representative domain $\reprdomain^{\attributes_{R_i}}$
\end{theorem}

\begin{proof}
It's similar to the path join case. 
\end{proof}

\begin{theorem}
$\RTS{i}$ computes the correct tuple sensitivity for each tuple.
\end{theorem}

\begin{proof} 
It's similar to the path join case. Notice that the query can be rewritten as
$$\comptree(\R{i}) \bowtie \R{i} \bowtie (\underset{j \in C(i)}{\bowtie} \subtree(\R{j}))$$


\end{proof}


\subsubsection{Efficiency Analysis}



Define $\Qsjoin(\R{0}, \R{1} \ldots \R{m})$ as a star join, which can be expressed by a tree $T_S(V, E)$, where V = $\{\R{0}, \R{1} \ldots \R{m}\}$ and E = $\{(\R{0}, \R{i}) \mid i \in \{1 \ldots m\} \}$

The recursive approach:

\begin{align}
& \botjoin(R_i) = \\ \nonumber
& \begin{cases}
     \aggregate{\attributes_{i,p(i)}}{sum(C_i \underset{j \in C(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}} \\
     \quad \Qsjoin(\aggregate{\attributes_{i, p(i)}, \attributes_j \forall j \in C(i)}{count(*) \as C_i} \\
     \quad{\R{i}}, \{\botjoin(\R{j})  \mid j \in C(i) \}) &, \text{$\R{i}$ is not a leaf}    \\
     \aggregate{\attributes_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{R_i} &, \text{$\R{i}$ is a leaf}
\end{cases} \\
& \topjoin(R_i) = \\ \nonumber
& \begin{cases}
     \aggregate{\attributes_{i,p(i)}}{sum(C_i \cdot \cntt{p(i)}{p(p(i))} \cdot  \underset{j \in N(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}}{} \\ 
     \quad \Qsjoin(\aggregate{\attributes_{i, p(i)}, \attributes_{p(i), p(p(i))}, \attributes_j \forall j \in C(i)}{count(*) \as C_i}{\R{p(i)}}, \\
     \quad \{\topjoin(\R{p(i)})\} \cup \{\botjoin(\R{j})  \mid j \in N(i) \})
     &, \text{not root}    \\
     \text{not defined} &, \text{root}
\end{cases}
\end{align}



If $\topjoin(\R{i})$ is not defined and a query includes this, simply ignore this. If $p(p(i))$ is not defined, $\cntt{p(i)}{p(p(i))} = 1$

Notice that when $\R{0}$ joins with $\R{i}$, we assume it is a left outer join. If it joins a NULL attribute, we change the corresponding counting attribute $C$ by default as 0.

\begin{lemma}\label{lem:qsum-eq}
Given a query $q$ as
\begin{align}
    \aggregate{\attributes_0}{sum(\underset{j \in \{1 \ldots m\}}{\product} C_j)}{\Qsjoin(\R{0}, \R{1} \ldots \R{m})}
\end{align}
, where $\attributes_j$ is the join attributes between $\R{0}$ and $\R{j}$, $C_j$ is the attribute of $\R{j}$, $\attributes_0$ is the group by attributes of $\R{0}$. Suppose $\attributes_j$ is a primary key for $j \in \{1 \ldots m\}$, we have an equivalent query of $q$ as:
\begin{align}
    & \aggregate{\attributes_0}{sum(C_0 \cdot \underset{j \in \{1 \ldots m\}}{\product} C_j)} \nonumber \\
    & \quad {\Qsjoin(\aggregate{\attributes_0, \attributes_1, \ldots, \attributes_m}{count(*) \as C_0}{\R{0}}, \R{1} \ldots \R{m})}
\end{align}
\end{lemma}

\begin{proof}
The semantic meaning of the query is to compute the size of the join group by a specific attribute.
\end{proof}

\begin{theorem}
The recursive $\botjoin$ and $\topjoin$ satisfy the invariant definition.
\end{theorem}

\begin{proof}
For $\botjoin$, 
\begin{enumerate}
    \item when $\R{i}$ is a leaf. The recursive equation is exactly the invariant definition.
    \item when $\R{i}$ is not a leaf. According to the lemma \ref{lem:qsum-eq}, the query can be rewritten as:
\begin{align*}
    & \aggregate{\attributes_{i,p(i)}}{sum(\underset{j \in C(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}}{\Qsjoin(\R{i}, \{\botjoin(\R{j})  \mid j \in C(i) \})}  
\end{align*}

    Suppose the statement that the recursive $\botjoin$ equals to the invariant definition works for all the children of $\R{i}$. Now we have another equivalent query:
\begin{align*}
    & \aggregate{\attributes_{i,p(i)}}{sum(\underset{j \in C(i)}{\product} \cntt{i}{j}) \as \cntt{i}{p(i)}}{}\\
    & \quad {\Qsjoin(\R{i}, \{\aggregate{\attributes_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{\subtree(R_i)}  \mid j \in C(i) \})}  
\end{align*}

    The semantic meaning of this query is compute the join size of the star query group by $\attributes_{i,p(i)}$. We rewrite it as:
\begin{align*}
    & \aggregate{\attributes_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{\Qsjoin(\R{i}, \{\subtree(R_i) \mid j \in C(i) \})}  
\end{align*}    
    
    According to the structure as the tree $T$, the star join is equal to the subtree of $\R{i}$. So we can further rewrite it as:
\begin{align*}
    & \aggregate{\attributes_{i,p(i)}}{count(*) \as \cntt{i}{p(i)}}{\subtree(\R{i})}
\end{align*}    
    , which is exactly the invariant definition
\end{enumerate}
For topjoin, the proof is similar, except that the final step is given by
\begin{align*}
    \comptree(\R{i}) = \Qsjoin(\R{i}, \{\topjoin(\R{p(i)})\} \cup \{\botjoin(\R{j})  \mid j \in N(i) \}))
\end{align*}
\end{proof}

Denote $deg(\R{i})$ as the degree of the node $\R{i}$ in the tree $T$. Denote $deg^*$ as the maximum degree.
Let the height of the tree be $H$, and the level of a node $R_i$ by $h(R_i)$.

\begin{theorem}
The time complexity of $\botjoin$ and $\topjoin$ is $O(n \log n (deg^*-1))$. The size of $\botjoin$ and $\topjoin$ is $O(n)$.
\end{theorem}

\begin{proof}
For $\botjoin$, the first step is to compute a group by on $\R{i}$, which takes $O(nlog(n))$ time. The second step is to compute a star join on primary keys. Since the number of relations of the star join is at most $deg^*-1$, the time complexity is $O(n \log n (deg^*-1))$. The third step is to compute an outer group by. Since the size of the star join is the same as $\R{i}$, the time complexity of this step is $O(nlog(n))$. In conclusion, the time complexity is $O(n \log n (deg^*-1))$.

For $\topjoin$, the proof is similar. Notice that the maximum number of relations in the star join is also $deg^*-1$.

\end{proof}

\note{Add double acyclic join here}

\begin{definition}
An acyclic join query is a double acyclic join query if removing any relation from the query, the remaining query is still an acyclic join query.
\end{definition}

\begin{theorem}
If a query $\CQ$ is a double acyclic join, for any join tree of $\CQ$, and for any node in the join tree, the $\topjoin$ and the $\botjoin$s of its children form an acyclic join.
\end{theorem}

\begin{proof}
If $\topjoin$ and $\botjoin$s form an cyclic join, the original join tree must not be a valid acyclic join tree. Details need to be continued.

The basic idea is that, for any table that forms $\topjoin$, it must share the similar attributes to the $\topjoin$. Thus if $\topjoin$ and $\botjoin$ cannot form a acyclic join tree, adding these tables cannot help forming a acyclic join tree.
\end{proof}

\note{To find the most sensitive tuple of a relation, since it is guaranteed that the topjoin and botjoin around the relation can form an acyclic join, we can compute it in polynomial time in aspect to the input data size.}

To find the most sensitive tuple, 

\begin{align}
    \startuple_{i, j} = 
\begin{cases}
    \argmax_{t \in \botjoin(\R{j})}
        t[C_{i, j}]
        &, j \in C(i) \\
    \argmax_{t \in \topjoin(\R{i})}
        t[C_{i, j}]
        &, j = p(i)
\end{cases}
\end{align}

\begin{align}
    \startuple_i = 
\begin{cases}
 	\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\startuple_{i,j} \mid j \in C(i) \cup \{ p(i)\} \}) &, other \\
 	\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\startuple_{i,j} \mid j \in C(i) \}) &,  \text{$R_i$ is the root} \\
 	\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\startuple_{i,j} \mid j \in \{ p(i)\} \}) &, \text{$R_i$ is a leaf}
\end{cases}
\end{align}


\begin{theorem}
The time complexity to find the most sensitive tuple and the local sensitivity of a acyclic join query is $O(m n \log n (deg^*-1))$.
\end{theorem}

\note{The total time complexity can be tighter. It should be $O(mn \log n)$. The reason is that $deg$ is different for each table, so the sum of $deg-1$ should equals to the number of tables, which is $m$.}

\begin{proof}
Since there are $m$ $\topjoin$ and $\botjoin$ to compute, it takes $O(mn \log n (deg^*-1))$. To find $t^*_i$, it takes another $O(mn(deg^*-1))$ time. In conclusion, the time complexity is $O(mn \log n (deg^*-1))$.
\end{proof}

\subsection{Correctness Analysis}

\begin{lemma}
	The query of the equation (\ref{eq:pj_tuple_sensitivity}) correctly finds the most sensitive tuple and its tuple sensitivity.
\end{lemma}
\proof{
	To illustrate the correctness, we decompose the query into two parts:
	(a) $Q_{list} = \pi_{\attr_{i-1}, \attr_{i}, \cnt{}{i-1} * \cnt{}{i} \as \tsens_i } \topjoin(\R{i}),~\botjoin(\R{i+1})$
	(b) $Q_{max} = \pi_{\attr_{i-1}, \attr_{i}, max(\tsens_i)} Q_{list}$
	
	For each row $r$ in the query result $Q_{list}$, $r.A_{i-1}A_{i}$ is a tuple from the domain $\domain_i$, and $r.\tsens_i$ is its corresponding tuple sensitivity.  We first show that the sensitivity computed is correct, then we show the query computes sensitivities for tuples from the \representative domain. If both are proved to be true, the most sensitive tuple and its tuple sensitivity is naturally given by $Q_{max}$
	\begin{enumerate}
		\item The tuple sensitivity is correctly computed. \note{Move it to 4.1 briefly. }
		
		Rewrite the entire path join query $\Qpjoin(\R{1},\ldots,\R{m})$ as 
		$$\Qpjoin(\R{1},\ldots,\R{i-1}) \bowtie \R{i} \bowtie \Qpjoin(\R{i+1},\ldots,\R{m})$$
		
		so the change of a given tuple $t$ from $\R{i}$ can be expressed as:
		$$\Qpjoin(\R{1},\ldots,\R{i-1}) \bowtie t \bowtie \Qpjoin(\R{i+1},\ldots,\R{m})$$
		
		the change of join size can be expressed as 
		\begin{align*}
		\aggregate{\attr_{i-1}}{count(*) \as  \cnt{}{i-1}}{\Qpjoin(\relation_1 \ldots \relation_{i-1})} \bowtie t \\ \bowtie \aggregate{\attr_{i}}{count(*) \as \cnt{}{i}}{\Qpjoin(\relation_{i+1} \ldots \relation_m)}    
		\end{align*}
		, which is
		$$\topjoin(\R{i})  \bowtie t \bowtie \botjoin(\R{i+1})$$
		
		\item The query computes tuple sensitivities for tuples from the \representative domain.
		
		The cross product of $\topjoin(R_{i})$ and $\botjoin(R_{i+1})$ includes all tuples from $\actdomain^{A_{i-1}} \times \actdomain^{A_{i}}$, which by definition is the representative domain $\reprdomain^{A_{i-1},A_{i}}$ about $\R{i}$. 
		
		In conclusion, since the most sensitive tuple is included in the \representative domain, correctly computing its tuple sensitivity result in finding the most sensitive tuple.
		
	\end{enumerate}
}

\begin{theorem}
	The algorithm \ref{algo:ls_pathquery} computes the local sensitivity of a path join query and find the corresponding most sensitive tuple.
\end{theorem}

\proof{
	The algorithm is divided into three parts: (1) prepare topjoin, (2) prepare botjoin, (3) combine topjoin and botjoin. We prove it by first showing that (1) and (2) is equivalent to the definition of topjoin (equation \ref{eq:pj_topjoin}) and botjoin (equation \ref{eq:pj_botjoin}). Next, we show that (3) is equivalent to the query as the equation \ref{eq:pj_tuple_sensitivity} shows.
	
	\begin{enumerate}
		\item Equivalence of topjoin
		\begin{align*}
		\topjoin(\R{i}) =
		\begin{cases}
		\aggregate{A_{i-1}}{sum(C_{i-2}) \as C_{i-1} }{}\\
		\quad \topjoin(\R{i-2}) \bowtie \R{i-1} &, i > 2 \\
		\aggregate{A_{i-1}}{count(*) \as C_{i-1}}{\R{i-1}} &, i = 2
		\end{cases}
		\end{align*}
		
		\item Equivalence of botjoin
		\begin{align*}
		\botjoin(\R{i}) =
		\begin{cases}
		\aggregate{A_{i-1}}{sum(C_{i}) \as C_{i-1} }{} \\
		{\quad  \botjoin(\R{i+1}) \bowtie \R{i} } &, i < m \\
		\aggregate{A_{i-1}}{count(*) \as C_{i-1}}{\R{i}} &, i = m
		\end{cases}
		\end{align*}
		
		\item Equivalence of selecting most sensitive tuple
		\begin{align*}
		t_{top}^i &= \pi_{\attr_{i-1}, \max(\cnt{}{i-1}) \as \tsens_{i-1} } ~ \topjoin(\R{i}) \\
		t_{bot}^i &= \pi_{\attr_{i}, \max(\cnt{}{i}) \as \tsens_{i} } ~ \botjoin(\R{i+1})
		\end{align*}
		\begin{align*}
		\tsens^* = \argmax_{\tsens}
		\begin{cases}
		\pi_{\attr_1, \tsens_1 \as \tsens} ~ t_{bot}^2 \\
		\pi_{\attr_{m-1}, \tsens_{m-1} \as \tsens} ~ t_{top}^m \\
		\pi_{\attr_{i-1}, \attr_{i},\tsens_{i-1} *  \tsens_{i} \as \tsens} ~ t_{top}^i, t_{bot}^i
		\end{cases}    
		\end{align*}    
	\end{enumerate}
}

\subsection{Efficiency Analysis}

\note{Merge Lemma 4.3 and 4.4 to theorem 4.5}

\begin{lemma}\label{lem:top_bot_join}
	The time complexity of computing topjoin $\topjoin$ or botjoin $\botjoin$ for all tables is $O(m n \log n)$.
\end{lemma}

\begin{proof} For bases cases, there is a single group by query, so it takes $O(n \log n)$ time. For analyzing one step of the recursion, the time complexity only depends on the data size of the subroutine, not its running time. For topjoin or botjoin, they both join a relation to the subroutine on the primary key of the size $n$, so it takes $O(n)$ and outputs a $O(n)$ temporary table. The further group by query takes $O(n \log n)$ time. In total, it takes $O(n \log n)$ time. Since we need to compute topjoin and botjoin for $m$ relations, the total time is $O(m n \log n)$.
\end{proof}

\begin{lemma}\label{lem:most_sens_tuple}
	The time complexity of selecting most sensitive tuple is $O(mn)$
\end{lemma}

\begin{proof}
	For each relation, we do at most 2 aggregation query as finding the max frequency from related topjoin or botjoin, which takes $O(n)$ time. This is repeated for $m$ relations, so the total time complexity is $O(mn)$. 
\end{proof}

\begin{theorem}
	Algorithm~\ref{algo:ls_pathquery} computes the local sensitivity of a path join query and also  finds the corresponding most sensitive tuple is $O(mn \log n)$ time where $m = $ the number of attributes and $n = |D|$.
\end{theorem}

\begin{proof}
	This is the immediate result from lemma \ref{lem:top_bot_join} and lemma \ref{lem:most_sens_tuple} 
\end{proof}

==> complexity-SAVED.tex <==
\section{Complexity Analysis}\label{sec:complexity}
In this section, we study the complexity of the local sensitivity problem. First, we review the notions of complexity in databases below.

\paratitle{Query, Data, and Combined Complexity.~} For evaluation of database queries, both the query size (the number of relations and attributes $m, k$) and the instance size (the number of tuples $n$) are inputs, and therefore based on the parameter that is considered as variable, three different notions of complexity are considered \cite{Vardi82}.  \emph{Query or expression complexity} treats the query size ($m, k$) as variable and the data size ($n$) as  constant. \emph{Data complexity} treats data size as variable and query size as constant, whereas \emph{combined complexity}  treats both query size and data size as variables. It is known that even query evaluation for general CQs is NP-hard for query and combined complexity (e.g., by a simple reduction from the clique problem), but is polynomial in data complexity. 

\subsection{Polynomial Data Complexity}
%\am{Review what is data complexity -- complexity in the size of the data assuming query size is fixed.}
The naive solution of computing the local sensitivity is to check the tuple sensitivity of all possible tuples from all tables. While for downward tuple sensitivity, we need to consider deletion of at most $n$ tuples from the database, for the upward tuple sensitivity when we consider inserting a tuple, the domain of a possible tuple can be arbitrarily larger than $n$ (and even infinite if any attribute has infinite, e.g., integer domain). However, we show below that we can always have a polynomial data complexity by narrowing down the domain of interest.

\par
\emph{Active domain} of an attribute with respect to a given instance typically refers to the set of values of that attribute appearing in the instance. In our context, given an instance $D$, a relation $R_i$ in $D$, and an attribute $\attr \in \attributes_i$, we use $\actdomain^{A, i} = \cup_{t \in R_i} t.A \subseteq \domain^{\attributes_i}$ to denote the active domain of $A$ with respect to $R_i$ in $D$. If an attribute $A$ appears in two relations $R_i, R_j$, it may happen that $\actdomain^{A, i} \neq \actdomain^{A, j}$.

\eat{
\sr{edited up to here.. PLEASE DO NOT READ OR EDIT THIS SECTION}

\am{There are several concepts here -- full, active, idle, representative, bounded, completementary trivial. Do we need all these terms here? There is no definition of "bounded", and representative and complementary-trivial seem to mean the same thing. 

Shouldn't representative depend on the query (the notation and the discussion after Def 3.1 does not mention a query)? If a query joins two datasets or has a selection then the size of he representative domain is smaller than if the query joins three datasets. Also, definition 3.1 is undefined in the absence of a query. 

I wonder if Lemma 3.1 should just say: ``$\reprdomain^{\attributes_i}$ as defined in Equation?? is $\representative$ and has size $O(n^k)$, where $n$ is the number of rows in each relation and $k$ is the number of attributes in the query (?).''}
}

\eat{
For this $v$, We also define the frequency of $v$ as
$ \freq{v}^i = \sum_{t \in \relation_i} \oneFunction_{[t.\attributes = v]} $.
If the context is clear, we simply write it as $\freq{v}$.
}

\begin{definition}\textbf{Representative domain.} For an attribute $\attr \in \attributes_\database$, we define the \emph{representative domain}  $\reprdomain^{\attr} \subseteq \domain^{\attr}$ as the sub-domain of interest for $A$ as: 
\begin{equation}
    \reprdomain^{\attr} = \bigcap_{i ~:~ \attr \in \attributes_i }
\end{equation}
\end{definition}

%a partition the domain $\domain^{\attributes_i}$  into two disjoint sub-domains:  and the idle domain $\idldomain$.  $$\domain = \actdomain \cup \idldomain$$

The active domain $\actdomain = \{ v \in \domain \mid \freq{v} > 0 \}$ is defined as the set of attribute values that are existing in the table. 
The idle domain $\idldomain = \{ v \in \domain \mid \freq{v} = 0 \}$ is the complementary set of $\actdomain$ regard to the full domain $\domain$, where values do not appear in the table.


\paratitle{\representative and Bounded Sub Domain}
Instead of considering the full domain, we show that there is a \representative sub domain of the full domain which is bounded and all tuples outside this sub domain has tuple sensitivity as 0. 

\begin{definition}
Given a query $\CQ$, a database $\database$, for any table $R_i$, a sub domain $\sidldomain$ of the full domain $\domain^{\attributes_i}$ is \representative if it is
\begin{enumerate}
    \item complementary-trivial. For any tuple $t$ in $\domain^{\attributes_S} \setminus \sidldomain$, tuple sensitivity $\tsens$ is 0.
\end{enumerate}

\end{definition}

The full domain is a trivial \representative domain. We will soon show that we can construct a domain that not only it is \representative, but also bounded. . The basic idea is to relax the active domain to include more interesting tuples.

\note{Construct \representative domain in a more general and easier way, such as joining from the rest of relations.}

Denote $\reprdomain$ as the \representative domain that we are going to construct. For a single attribute $A$, it is defined as follows:

$$\reprdomain^A =  \bigcap_{\substack{\forall~\text{table}~R \\ \forall B \in \attributes_R}} \actdomain^B \oneFunction_{[\bowtie_{R.B = S.A} \in q ]} $$

Notice that $\reprdomain^A$ doesn't necessarily include the active domain of $A$.

For general attributes $\attributes = A_1 \ldots A_m$, it is defined as:
$$\reprdomain^\attributes = \reprdomain^{A_1} \times \ldots \times \reprdomain^{A_m}$$

\am{Should this be rewritten taking into account the query.}

\begin{lemma}
$\reprdomain^{\attributes_i} $ is $\representative$ and bounded.
\end{lemma}

\begin{proof}~

\begin{enumerate}
    \item bounded. For a single attribute, the domain size of $\reprdomain^{A}$ is the smallest active domain of any single attribute domain, which is $O(n)$. For general attributes, it is the cross product of all \representative active domain of single attributes, so it is exponential to the degree of $|\attributes| = k$. In conclusion, the size is $O(n^k)$. \am{Should this be rewritten taking into account the query.}
    \item complementary-trivial. Adding a tuple from $\domain^{\attributes_i} \setminus \reprdomain^{\attributes_i}$ will not change the join size, because at least one attribute of this tuple cannot join any tuple in other tables.
\end{enumerate}
\end{proof}

\begin{lemma}
Computing the tuple sensitivity of a tuple $t$ about the CQ query $\CQ$ on a database $\database$ is polynomial in data complexity. 
\end{lemma}

\proof{The complexity of computing a single tuple sensitivity is equivalent to of evaluating a CQ query, which is polynomial in data complexity.}

\begin{theorem}
Computing local sensitivity and finding a tuple of the maximum tuple sensitivity is polynomial in data complexity.
\end{theorem}

\proof{We can iterate all tuples in the \representative and bounded domain $\reprdomain$ for each table and compute its tuple sensitivities to find the maximum one.}

\subsection{NP-hardness for Combined Complexity}
\am{Review how combined complexity is different from data complexity, and why we want to study this? For instance, say that an algorithm that is $O(n^k)$ would not scale even for queries that join 3 relations each of size a million rows.}
It is known that evaluating a CQ query can be NP-hard in combined complexity if this query is non-acyclic. However, although evaluating acyclic queries is of polynomial time in the size of the input and output data \note{If it is polynomial to the output size, it means it can be exponential in the combined complexity. Shall we emphasize this? since our solution to the double acyclic query can find LS in polynomial time in combined complexity}, computing local sensitivty of acyclic queries can be NP-hard.

\begin{theorem} Given an CQ query $\CQ$ on a database $\database$ with $m$ tables, each of which contains $k$ attributes and $n$ tuples, checking whether $LS(\CQ, \database)>0$ is NP-hard for combined complexity in terms of $m, n$ and $k$, even for the class of the acyclic queries.
\end{theorem}
\am{This theorem statement needs to be rewritten. It reads ... the problem if hard for \textit{every} query Q (which would be data complexity)? Rather the theorem statement should read: The problem of checking whether $LS(Q,D)>0$, where $Q$ and $D$ are input query and database respectively is NP-hard with respect to the combined complexity of the inputs $Q$ and $D$.}

It is followed that computing an exact local sensitivity of a CQ query is NP-hard.

\begin{proof}
The local sensitivity of a CQ query is defined as the maximum change to the query output size if adding to one of the tables or removing a tuple from one of the tables.
The changes to the query output size when removing a tuple is upper bounded by the changes to the query output when adding a tuple. Hence, we will just show that checking if the changes to the query output size is greater than 0 if adding a tuple to one of table is NP-hard.

To show the hardness of this problem, we solve it by reduction from 3SAT with $m$ clauses
($C_1,\ldots,C_m$) and $l$ variables ($v_1,\ldots,v_l$).
For each clause in 3SAT instance, we reduce each clause into a table as follows:
for each clause $C_i$ that has three literals associated to three variables $v_{i_1},v_{i_2},v_{i_3}$, we add a table $R_i$ consisting the corresponding 3 boolean attributes $A_{i_1},A_{i_2},A_{i_3}$ and insert all possible tuples of boolean values that satisfy the clause $C_i$ to $R_i$ to form $x_i$. For example, if $C_i$ is $v_{i_1}\lor \bar{v}_{i_2} \lor \bar{v}_{i_3}$,
then all $(0,0,0), (0,0,1),\ldots,(1,1,1)$ except $(0,1,1)$ are inserted to $D_i$.
In addition, we create a relation $R_0(A_1,\ldots,A_l)$ with an empty table $x_0$. \note{Change this dummy relation to a simpler relation:  $R_0(A_1)$}
This leads to a database of $(m+1)$ tables $(D_0,D_1,\ldots, D_m)$ with $l$ attributes $(A_1,\ldots,A_l)$.

The query can rewritten as:
\begin{align*}
    \CQ(A_1 ,\ldots, A_l) = \underset{i = 1 \ldots m}{\wedge} \R{i}(A_{i_1},A_{i_2},A_{i_3})
\end{align*}

We first show that if 3SAT is satisfiable, then the joint output of $(D_1,\ldots,D_m)$ is not empty, and hence adding a tuple to $D_0$ that match a joint tuple from $(D_1,\ldots,D_m)$ can cause a positive change to the joint output size of $(m+1)$ tables $(D_0,D_1,\ldots, D_m)$, i.e., $LS_{q}(D)>0$, where $q:=COUNT(\bowtie_{i=0,\ldots, m} R_i)$ is an SPJA* query. If there is an assignment to the $l$ variables in the 3SAT problem such that every clause $C_i$ is True, then the corresponding tuple must be present in $D_i$ which can form a joint tuple between the $k$ tables $(D_1,\ldots,D_m)$.
We then show that if the joint output between $(D_1,\ldots,D_m)$ is not empty, then 3SAT is satisfiable. Let $t$ be one of the joint output tuples where $a_1,\ldots, a_l$ are the corresponding values assigned to $A_1,\ldots, A_l$ respectively. Then the projection of this output tuple $t$ over the attributes of each table is an tuple existing in the table, which satisfy the corresponding clause.
All the corresponding clauses will be evaluated True and hence 3SAT is satisfiable.
\end{proof}

\begin{corollary} Given an CQ query $\CQ$ on a database $\database$ with $m$ tables, each of which contains $k$ attributes and $n$ tuples, and a tuple $t$, checking whether $\tsens(t, \CQ, \database)>0$ is NP-hard for combined complexity in terms of $m, n$ and $k$.
\end{corollary}

\begin{proof}
It is similar to the proof above. Just rewrite the dummy relation ($R_0$) as a single attribute relation, and run algorithm twice on v = 0 and v = 1.
\end{proof}
\am{What is the difference between LS and $\delta$?}

The hardness of finding a tuple whose tuple sensitivity matches the local sensitivity (\am{use the term "sensitivity problem"}) follows that it can indicate whether $LS > 0$ or not.

\am{I think we need to end this section with a para or a theorem statement (without proof) that says that notwithstanding the hardness result, we next show an algorithm for solving the sensitivity problem that has polynomial combined complexity for ``doubly acyclic" queries. Also add a line about general queries ... ask Sudeepa how to write the parameterized complexity statement. }

==> discussion.tex <==
\red{the paper may be updated once we understand these}

\begin{itemize}
    \item handling selection: \am{Do we need to add the ability to select subsets of rows? Can we handle selections in our algorithms? Remember that Elastic sensitivity can not reduce the local sensitivity based on selections on tables. If our algorithms can handle selections, it will be a \textit{major} contribution}
It can also be written in the relation algebra form as derived from the join tree. We interchangeably use the datalog and relation algebra notation.

\item 
\todo{(1) how about reporting top-$k$ most sensitive tuple (add a discussion that how this can be generalized -- SELECT TOP ... LIMIT BY ./..0, (2) make sure that it takes care of both deletion and insertion}
\end{itemize}

==> double_acyclic_join.tex <==
\subsection{Double Acyclic join}\label{sec:double-acyclic}

Recall that the complexity of algorithm ($\ref{algo:gj_query}$) is $O(m p q  \log n \cdot n^{pq} )$ for a database with $n$ tuples and a general join query with $m$ relations, hypertree width $p$ and double hypertree width $q$. If both $p$ and $q$ reduce do 1, the complexity reduces to $O(m n \log n)$ as sub-quadratic to $n$ and linear to $m$. We name queries that share this property as double acyclic join queries, since hypertree equals to 1 matches the definition of an acyclic join query and we have two levels of acyclicity. 

Notice that a path join query is a special case of double acyclic join query. The hypertree width is one by definition and the double hypertree width is also one since for each $\R{i}$, $\topjoin(\R{i})$ and $\topjoin(\R{i+1})$ share no attribute and thus each of them forms a single-relation join group which has a trivial hypertree width as one.

==> evaluation_backup/exp_dp.tex <==
\subsection{Differential Privacy}\label{sec:exp_dp}

\paratitle{Baseline}. \PrivSQL is a differentially private SQL answering engine that uses the truncation mechanism that truncates the database and adds the noise according to the global sensitivity of query after truncation to generate database synopses which support ad-hoc high-utility SQL query answering. It introduces the concept of policy that given primary private relations, the sensitivity of other related relations should be updated to be non-zero according to the database key constraints. We assume \texttt{CUSTOMER} is the primary private relation for q1 and q3, and \texttt{SUPPLIER} is the primary private relation for q2, so the sensitivity of \texttt{ORDERS} is affected by \texttt{CUSTOMER} and the sensitivity of \texttt{PARTSUPP} is affected by \texttt{SUPPLIER}. The sensitivity of \texttt{LINEITEM} is affected by either of them.

\PrivSQL uses the maximum frequency as the truncation threshold, which is different from using tuple sensitivity to truncate the database. Any tuple whose frequency is beyond the max frequency will be dropped from the database. \PrivSQL runs SVT to learn the truncation threshold for each relation; however, the noise scale of SVT depends on the sensitivity of the relation while it is constantly 1 in \TSensDP. 

Although the privacy budget allocation strategy affects the performance of DP algorithm, we skip exploring the effect of budget allocation and assume \PrivSQL and \TSensDP divide the privacy budget into two halves, one for the threshold learning and the other for adding noise to the query result after truncation. We disable the synopsis generation phase of \PrivSQL and just use Laplace mechanism to answer the SQL query directly.


\begin{figure*}[t]
	\centering
	\includegraphics[trim={25, 80, 25, 50}, clip, width=.9\textwidth]{{"figures/TPSens - DP - Sheet1"}.pdf}
	\vspace{-10pt}
	\caption{Application to Differential Privacy: Comparing \TSensDP error to \PrivSQL error}
	\label{fig:dp}
	\vspace{-10pt}
\end{figure*}

\paratitle{Result and Analysis}. Figure \ref{fig:dp} shows the statistics of releasing differential private query results by \TSensDP or \PrivSQL. We assume the table size is given and assume the maximum tuple sensitivity of q1 is 100, of q2 is 500 and of q3 is 10. We run each algorithm 10 times and report the average of global sensitivity, the average of relative absolute bias and the average of relative absolute error. 

\TSensDP has $\leq4$\% error for $q_1$ and $q_3$, and $\leq 25$\% error for $q_2$. In contrast, \PrivSQL has more than $100$\% relative error on $q_2$ and $q_3$. This means that the error in \PrivSQL answers for these queries is worse than returning 0 as the answer without looking at the data. The reasons for the poor error are different. In $q_2$ \PrivSQL truncates too much of the data, while in $q_3$ it estimate a very loose bound on sensitivity.  

\revm{Table 2 shows the statistics of releasing differential private query results by \TSensDP and \PrivSQL for Facebook data. We assume assume the maximum tuple sensitivity of $\qtri$ is 100, of $\qpath$ is 100k, of $\qstar$ is 1k and of $\qtri$ is 30. We randomly assign one relation in the query as the primary private relation. We run each algorithm 10 times and report the median of global sensitivity, the median of relative absolute bias, the median of relative absolute error and the average of running time in seconds. 

\TSensDP achieves $< 5\%$ error for $\qtri$, $\qpath$, $\qstar$, while \PrivSQL get $> 700\%$ error for $\qcycle$ and $\qstar$. Since there is no FK-PK join for the Facebook queries, we have only one primary private table, which means we don't need to truncate tables and thus has 0 bias in \PrivSQL. However, \PrivSQL has $\times 2$ to $\times 200k$ larger global sensitivity than \TSensDP, which dominates the error. }

\revb{To find how the estimated upper bound of tuple sensitivity $\ell$ affect performance, we also changed $\ell$ among 1, 30, 50, 80, 100, 1000 for a triangle query, whose actual local sensitivity is 24. We list median global sensitivity,  median bias error and median relative error as triples for each bound: [(13.0, 5.48\%, 4.72\%),  (18.5, 0.00\%, 4.60\%),  (11.0, 18.87\%, 21.48\%),  (12.5, 10.36\%, 21.19\%),  (33.0, 0.00\%, 3.72\%),  (6.5, 55.45\%, 93.80\%)]. The optimal $\ell$ in this case is 30, where the median relative error is 4.6\%, while the worst error is 93.8\% when $\ell = 1000$. Notice that as $\ell$ increases, the noise of $\hat{\CQ}$ in the $SVT$ routine is larger, thus it is harder to find the optimal tuple sensitivity bound. }

%a stable error for simple or complex queries as its relative error is always below 25\%. It can be more than 1,000,000\% accurate than \PrivSQL for q3. Although \TSens has within 2\% higher relative bias than \PrivSQL for q1 and q3, the global sensitivity is 2x and 800,000x smaller than \PrivSQL.



==> evaluation_backup/exp_head.tex <==
We evaluate the efficiency and accuracy of \TSens. Experiments are designed to answer following questions:
\squishlist
\item How tight is the local sensitivity computed by \TSens compared to other algorithms like elastic sensitivity\cite{DBLP:journals/corr/JohnsonNS17}?
\item How does \TSens' runtime compared to that of (a) the elastic sensitivity algorithm and (b) query evaluation?
\item Does the truncation with \TSens mechanism result in more accurate differentially private query answering than prior work like \PrivSQL \cite{kotsogiannis2019privatesql}?
\squishend
\eat{
Although it is proved that \TSens achieved the tightest local sensitivity, it is unknown how much it improves the bound of local sensitivity and how much it increases the time usage in practice. What's more, since \TSens can also track tuple sensitivity as a side product, it can truncate the database to be of a fixed global sensitivity and at the meanwhile guarantee a low bias, but it is unknown to which extent it improves the utility. 
}

We use synthetic datasets from TPC-H benchmark \cite{TPCH} and designed three full conjunctive queries with different query complexities to evaluate the performance of \TSens. These queries are also used to evaluate the performance of DP mechanism supported by \TSens. The results are compared with the sensitivity engine \Elastic from `Flex' \cite{DBLP:journals/corr/JohnsonNS17} and with the 
differentially private SQL answering engine \PrivSQL from `PrivateSQL' \cite{kotsogiannis2019privatesql}. We name our sensitivity algorithm as \TSens and its DP application as \TSensDP. 

\eat{
\TSens is implemented by 1.5k lines of python and it uses Postgres as the database engine. We extend 'Elastic Sensitivity' so it can compute the sensitivity of a cross product. As to the DP experiment, we also borrow the concept of policy and primary private relation from 'PrivateSQL' and assume the query has already been rewritten according to the policy. 
}

%The experiments results validate that \TSens can improve the tightness of local sensitivity with a reasonable performance cost and improve the utility of the truncation mechanism for DP. In particular:
A summary of our key findings: 
\squishlist
	\item \TSens achieves at most 2,200,000 times smaller local sensitivity compared to \Elastic for a simple cyclic query for a database with 866,602 tuples.
	\item \TSens has \revb{on average} 80\% - 320\% overhead compared to query evaluation for different queries. It is 2 - 47 times slower than \Elastic, but returns a local sensitivity value that is 6 - 60,000 times smaller \revb{on average}.
	\item \PrivSQL has more than 100\% relative error (worse than just returning 0 as the answer) for two of the three queries. \TSensDP answers 2 queries with $\leq 4\%$ relative error and the third query with $\leq 25\%$ relative error.
\squishend


==> evaluation_backup/exp_methodology.tex <==
%\vspace{-1.5em}
\subsection{Setup}

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[b]{0.15\textwidth}
		\centering
		\includegraphics[width=\textwidth]{{"TPSens - q1"}.pdf}
		\caption{q1 join plan}
		\label{fig:tpch_q1_graph}
	\end{subfigure}~~~
	\begin{subfigure}[b]{0.14\textwidth}
		\centering
		\includegraphics[width=\textwidth]{{"TPSens - q2"}.pdf}
		\caption{q2 join plan}
		\label{fig:tpch_q2_graph}
	\end{subfigure}~~~
	\begin{subfigure}[b]{0.25\textwidth}
		\centering
		\includegraphics[width=\textwidth]{{"TPSens - q3 - graph"}.pdf}
		\caption{q3 join graph}
		\label{fig:tpch_q3_graph}
	\end{subfigure}~~~
	\begin{subfigure}[b]{0.25\textwidth}
		\centering
		\includegraphics[width=\textwidth]{{"TPSens - q3 - join plan"}.pdf}
		\caption{q3 join plan}
		\label{fig:tpch_q3_tree}
	\end{subfigure}
	\caption{TPC-H query graphs and join plans 	}
	\vspace{-10pt}
\end{figure*}

%We evaluate our algorithm on synthetic TPC-H datasets with different scales and on three queries. 

\paratitle{Dataset}. We consider a database schema from TPC-H benchmark. The schema involves following attributes: \\
\texttt{RegionKey}(RK), \texttt{NationKey}(NK), \texttt{CustKey}(CK), \texttt{OrderKey}(OK), \texttt{SuppKey}(SK), \texttt{PartKey(PK)}\\
Relations in the database include: \\
\texttt{Region}(R:RK), \texttt{Nation}(N:RK,NK), \texttt{Customer}(C:NK,CK), \texttt{Orders}(O:CK,OK), \texttt{Supplier}(S:NK,SK), \texttt{Part}(P:PK), \texttt{Partsupp}(PS:SK,PK), \texttt{Lineitem}(L:OK,SK,PK).\\
We generate synthetic datasets (as per  \cite{DBGEN}) to get databases of different scales. At scale 1, the sizes of for these relations are 5, 25, 1e4, 1.5e5, 2e5, 8e5, 1.5e6, 6e6 respectively. The same schema and datasets were used to evaluate prior work on differentially private SQL query answering \cite{DBLP:journals/corr/JohnsonNS17, kotsogiannis2019privatesql}.
%relation is REGION(5), NATION(25), SUPPLIER(1e4), CUSTOMER(1.5e5), PART(2e5), PARTSUPP(8e5), ORDERS(1.5e6) and LINEITEM(6e6).

\revm{We also consider a database schema about Facebook ego-networks from SNAP (Stanford Network Analysis Project). An ego-network of a particular user is about how his/her friends are categorized into "social circles"  \cite{leskovec2012learning}. The dataset \footnote{http://snap.stanford.edu/data/ego-Facebook.html} provided by SNAP consists 10 ego-networks, 4233 circles, 4039 nodes and 88234 edges. We further create tables $R_i(x, y)$ including all edges that both end nodes are from the circle $i$, and tables $R_i(x, y, z)$ including all triangles that all end nodes are from the circle $i$. All edges are undirected.  }

\paratitle{Queries}. Figures~\ref{fig:tpch_q1_graph}-\ref{fig:tpch_q3_tree} show the join plans of 3 TPC-H queries . 
%\vspace{-5pt} 
\squishlist
\item[(q1)] Figure \ref{fig:tpch_q1_graph} shows a path join counting query  $q1(RK,NK,CK,OK)$ $:-$  $R(RK),$ $N(RK,NK),$ $C(NK,CK),$ $O(CK,OK),$ $L(OK)$ that goes through R, N, C, O and L.
%It builds an extensive table that tracks the detail of each lineitem in aspect to customers' nationalities.
\item[(q2)] Figure \ref{fig:tpch_q2_graph} shows an acyclic join counting query $q2(SK,PK) :- S(SK), P(PK), PS(SK,PK), L(SK,PK)$ whose root is PS and leaf relations are P, S and L. 

\item[(q3)] Figure \ref{fig:tpch_q3_graph} shows a simple cyclic join counting query $ q3(RK,NK,CK,OK,SK,PK)$ $:-$ $R(RK),$ $N(RK,NK),$ $C(NK,CK),$ $O(CK,OK),$ $S(NK,SK),$ $P(PK),$ $PS(SK,PK),$ $L(SK,PK)$ that combines q1 and q3 together. Figure \ref{fig:tpch_q3_tree} also shows its corresponding join plan. This query builds a universal table with an extra constraint that the supplier and customer should be from the same nation.
\squishend

%The joins in these queries are all foreign-primary key joins, so these queries themselves express the schema constraints and thus we can know how sensitive a tuple is in one relation that will affects other relations due to the schema constraints.

We set scales as 0.0001, 0.001, 0.01, 0.1, 1, 2, 10 to evaluate the scalability of the algorithm, which corresponds to a 200 kB, 1500 kB, 12 MB, 120 MB, 1.2 GB, 2.3 GB and 12 GB database. 

\revm{We also prepared 4 types of queries for Facebook data:  Triangle query $\qtri(A,B,C)$ $:-$ $R_1(A,B)$, $R_2(B,C)$, $R_3(C,A)$, path join query  $\qpath(A,B,C,D,E)$ $:-$ $R_1(A,B)$, $R_2(B,C)$, $R_3(C,D)$, $R_4(D,E)$ , 4-cycle query $\qcycle(A,B,C,D)$ $:-$ $R_1(A,B)$, $R_2(B,C)$, $R_3(C,D)$, $R_4(D,A)$, star join query $\qstar(A,B,C)$ $:-$ $R_1(A,B,C)$, $R_2(A,B)$, $R_3(B,C)$, $R_4(C,A)$. Relations with the same index in any two queries are not necessarily refer to the same table. Each query is tested on 4 sets of different tables and we choose one set to show in the paper as they have similar results.  }

We use a machine with 2 processors, 512G SSD and 16G memory to run experiments. Each query is repeated 10 times.

\eat{
\begin{figure}
	\centering
	\begin{subfigure}[b]{0.2\textwidth}
		\centering
		\includegraphics[width=\textwidth]{table_tpch_attributes.png}
		\caption{TPC-H Attributes}
		\label{fig:tpch_attr}
	\end{subfigure}
	\begin{subfigure}[b]{0.25\textwidth}
		\centering
		\includegraphics[width=\textwidth]{table_tpch_tables.png}
		\caption{TPC-H Tables}
		\label{fig:tpch_table}
	\end{subfigure}
	\caption{TPC-H Schema}
\end{figure}


\begin{figure}
	\centering
	\includegraphics[width=0.5\textwidth]{db_size.pdf}
	\caption{TPC-H Relation Size Histogram}
	\label{fig:tpch_dbsize}
\end{figure}
}


  

==> evaluation_backup/exp_sensitivity.tex <==
\vspace{-1em}
\subsection{Local Sensitivity}\label{sec:exp_ls}
\noindent\textbf{Baseline}. \Elastic assumes the maximum frequency of the join attributes in each table is given. This algorithm traverses the join tree to update the local sensitivity by tracking the change of max frequency. We remove the assumption and let \Elastic pre-process the database to compute the max frequency thus the algorithm output is a local sensitivity upper bound. We also extend the algorithm to support cross-product by assigning the max frequency of empty attributes as the size of the table. Since we represent a general join counting query as a join plan, we change the input to \Elastic to be the join plan as \TSens uses so that the join order in the experiment is the same. We define the join order as a post-traversal of the join plan.

\TSens reports the most sensitive tuple by tracking each tuple sensitivity and it also finds the most sensitive tuple for each relation within the procedure; however, \Elastic cannot find the most sensitive tuple, although it can find the local sensitivity upper bound. We report the most sensitive tuple for each relation while also reports its elastic sensitivity by setting this relation as the only sensitive table for \Elastic.

\revm{We also compare the algorithm running time to query evaluation time. We apply Yannakakis algorithm to compute the size of query output. For queries that are not acyclic, we first compute the join for each node in the generalized hypertree, and then apply Yannakakis algorithm.}

\paratitle{Result and Analysis}.
Figure \ref{fig:sens_change_by_n} shows the local sensitivity trend in aspect to the scale. Notice that after scale 0.001, \TSens has \revb{on average} 7x smaller and 6x smaller of the local sensitivity for q1 and q2 \revb{than} \Elastic has. Moreover, for q3, \TSens achieves 2,200,000x smaller value for the local sensitivity than \Elastic does when scale equals to 0.1. We didn't run q3 for scale larger than 0.1 due to the memory limit issue. \revb{For q3, our algorithm maintains frequency tables that grow nearly quadratically in the number of rows in the table increases. For instance, for the database with 8 thousand rows (at scale 0.001), we have intermediate tables with 1780 thousand rows.}

%\am{What does scale of 0.01 mean? If you had a large machine on AWS, would that query complete?}

Figure \ref{fig:time_change_by_n} shows the time cost for both \TSens and \Elastic for different queries and scales. The second line $q_i\_query$ is the time to evaluate the join plan as a counting query efficiently. For q1 and q2, both \TSens and \Elastic shows a tight relation to the time of query evaluation, which takes \revb{on average} 1.8x and 0.9x of the query evaluation time after scale 0.001. For q3, although \Elastic is much faster, \TSens only takes \revb{on average} 4.2x of the query evaluation time to find \revb{on average} 60,000x smaller local sensitivity before scale 1.

Figure \ref{fig:sens_tuple} shows the most sensitive tuple for each relation for q3 at scale = 0.01. Each tuple sensitivity is below 1,000 while the least elastic sensitivity is beyond 10,000. We skip finding the most sensitive tuple in LINEITEM since it has the superkey in the query head and thus the tuple sensitivity is at most 1.

\revm{Table 1 shows the local sensitivity $LS$ and time usage of 4 query types for \TSens and \Elastic. The sensitivity bound improvement ranges from $\times 2$ to $\times 480k$. Although \TSens spends $\times 6$ to $\times 60$ more time than \Elastic, it is comparable to query evaluation time. Notice that the size of active domain and representative domain for $\qtri$ is 12296 + 46224, for $\qpath$ is 11660 + 9797, for $\qcycle$ is 3570 + 13134, for $\qstar$ is 127250 + 8160, if we repeat query evaluation as removing tuples from the active domain and inserting tuples from the representative domain one at a time, it will take $\times 10k+$ time than \TSens to find the maximum tuple sensitivity.} 

\begin{figure*}[t!]
	\centering
		\begin{subfigure}[b]{0.44\textwidth}
		\centering
        	\includegraphics[width=.8\textwidth, trim={0 0 10 0}, clip]{sens_change_by_n.pdf}
        	\caption{Local sensitivity reported by \TSens and \Elastic for queries q1, q2 and q3 on datasets of differing scales }
        	\label{fig:sens_change_by_n}
        \end{subfigure} \ 
        \begin{subfigure}[b]{0.48\textwidth}
        	\centering
        	\includegraphics[trim={45, 120, 45, 50}, clip, width=.8\textwidth]{{"figures/TPSens - Experiment - MostSensitiveTuple2"}.pdf}
        	\caption{Most sensitive tuples and their tuple sensitivities for each relation of q3 when scale = 0.01. %The right column is the corresponding elastic sensitivity when setting each relation as the only sensitive relation.
        	}
        	\label{fig:sens_tuple}
        \end{subfigure}
   	\vspace{-10pt}
    \caption{Local sensitivity reported by \TSens versus \Elastic}
    \vspace{-10pt}
\end{figure*}

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth, trim={10 16 10 10}, clip]{time_change_by_n.pdf}
	\vspace{-20pt}
	\caption{The trend of time usage in terms of various scales for queries q1, q2 and q3 and algorithms \TSens and \Elastic. The base line `query' shows the query evaluation time.}
	\label{fig:time_change_by_n}
	\vspace{-10pt}
\end{figure*}


\begin{table}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
& \multicolumn{2}{c|}{LS} & \multicolumn{3}{c|}{Time (seconds)} \\ \cline{2-6}
& \tsens & \elastic & \tsens & \elastic & Evaluation \\ \hline
$\qtri$ & 76& 7524& 0.440& 0.007& 0.388\\ \hline
$\qpath$ & 115650& 225720& 0.227& 0.010& 0.178\\ \hline
$\qcycle$ & 218& 65610& 0.115& 0.005& 0.128\\ \hline
$\qstar$ & 29& 14008500& 0.371& 0.059& 0.195\\ \hline
\end{tabular}
\caption{Local sensitivity and time usage of 4 query types for TSens and Elastic. }
    \vspace{-20pt}
\end{table}


\begin{table}[t!]
\small
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
& $|Q(D)|$ & Algorithm & \multicolumn{1}{c|}{Error} & \multicolumn{1}{c|}{Bias} & \multicolumn{1}{c|}{GS} & \multicolumn{1}{c|}{Time}\\ \hline
$\qtri$ &20751 & TSensDP & 0.99\%  & 0.72\% & 54 & 0.515\\ \cline{3-7}&& PrivateSQL & 43.46\%  & 0.00\% & 4950 & 0.223\\ \cline{3-7}\hline$\qpath$ &2012183 & TSensDP & 4.16\%  & 0.71\% & 28885 & 1.007\\ \cline{3-7}&& PrivateSQL & 5.89\%  & 0.00\% & 71280 & 1.790\\ \cline{3-7}\hline$\qcycle$ &3825 & TSensDP & 63.67\%  & 8.37\% & 548 & 0.312\\ \cline{3-7}&& PrivateSQL & 744.56\%  & 0.00\% & 31590 & 0.163\\ \cline{3-7}\hline$\qstar$ &1369 & TSensDP & 1.77\%  & 0.00\% & 38 & 0.569\\ \cline{3-7}&& PrivateSQL & 599589.38\%  & 0.00\% & 8405100 & 0.628\\ \cline{3-7}\hline\end{tabular}
\caption{Application to Differential Privacy: Comparing \TSensDP error to \PrivSQL error. Time is in seconds.}
    \vspace{-20pt}
\end{table}



==> evaluation_backup/tables.tex <==
\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsens    & \elastic    & \tsens    & \elastic  & \tsens    & \elastic  & \tsens    & \elastic  \\ \hline
$s_1$	& 24	& 2430	& 38610	& 155520	& 1207	& 376200	& 19	& 996480	\\ \hline
$s_2$	& 76	& 7524	& 115650	& 376200	& 906	& 225720	& 19	& 1195776	\\ \hline
$s_3$	& 76	& 7524	& 115650	& 225720	& 218	& 65610	& 29	& 14008500	\\ \hline
$s_4$	& 42	& 2880	& 30780	& 65610	& 304	& 155520	& 29	& 13018800	\\ \hline
\end{tabular}
\caption{Local sensitivity of 4 query types under 4 query settings for TSens and Elastic. $\qtri$ is a triangle query, $\qpath$ is a path query of 4 nodes, $\qcycle$ is a 4-cycle query, $\qstar$ is a star query of 4 nodes}
\end{table*}
\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
\def\qtime{$Q(D)$}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{3}{l|}{$\qtri$} & \multicolumn{3}{l|}{$\qpath$} & \multicolumn{3}{l|}{$\qcycle$} & \multicolumn{3}{l|}{$\qstar$} \\ \cline{2-13} 
                  & \tsens    & \elastic    & \qtime    & \tsens    & \elastic  & \qtime    & \tsens    & \elastic  & \qtime    & \tsens    & \elastic  & \qtime    \\ \hline
$s_1$	& 0.109	& 0.004	& 0.111	& 0.215	& 0.009	& 0.164	& 0.506	& 0.008	& 0.459	& 0.311	& 0.007	& 0.175	\\ \hline
$s_2$	& 0.391	& 0.006	& 0.393	& 0.221	& 0.010	& 0.167	& 0.453	& 0.008	& 0.395	& 0.404	& 0.008	& 0.180	\\ \hline
$s_3$	& 0.440	& 0.007	& 0.391	& 0.227	& 0.010	& 0.177	& 0.115	& 0.005	& 0.132	& 0.371	& 0.059	& 0.184	\\ \hline
$s_4$	& 0.120	& 0.004	& 0.128	& 0.217	& 0.007	& 0.169	& 0.221	& 0.005	& 0.163	& 0.386	& 0.068	& 0.175	\\ \hline
\end{tabular}
\caption{Time of computing local sensitivity of 4 query types under 4 query settings for TSens, Elastic and query evaluation (in seconds).}
\end{table*}


\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsensdp    & \privatesql    & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  \\ \hline
$s_1$	& 7.97\%	& 179.53\%	& 17.17\%	& 8.49\%	& 0.34\%	& 238.20\%	& 6.20\%	& 95015.23\%	\\ \hline
$s_2$	& 10.03\%	& 39.53\%	& 2.00\%	& 2.59\%	& 16.06\%	& 614.71\%	& 13.94\%	& 70474.03\%	\\ \hline
$s_3$	& 0.99\%	& 43.46\%	& 4.16\%	& 5.89\%	& 63.67\%	& 744.56\%	& 1.77\%	& 599589.38\%	\\ \hline
$s_4$	& 41.45\%	& 53.73\%	& 40.58\%	& 15.50\%	& 41.94\%	& 862.41\%	& 8.60\%	& 734135.53\%	\\ \hline
\end{tabular}
\caption{Relative error of 4 query types under 4 query settings for TSensDP and PrivateSQL.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsensdp    & \privatesql    & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  \\ \hline
$s_1$	& 0.246	& 0.124	& 0.932	& 1.721	& 0.692	& 1.756	& 0.476	& 0.169	\\ \hline
$s_2$	& 0.456	& 0.219	& 1.108	& 6.604	& 0.568	& 0.802	& 0.516	& 0.182	\\ \hline
$s_3$	& 0.515	& 0.223	& 1.007	& 1.790	& 0.312	& 0.163	& 0.569	& 0.628	\\ \hline
$s_4$	& 0.255	& 0.123	& 0.589	& 0.350	& 0.362	& 0.250	& 0.558	& 0.673	\\ \hline
\end{tabular}
\caption{Computation time of 4 query types under 4 query settings for TSensDP and PrivateSQL (in seconds).}
\end{table*}


\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 1	& 30	& 50	& 80	& 100	& 1000	\\ \hline 
$s_1$ & 20	& 4.72\%	& 4.60\%	& 21.48\%	& 21.19\%	& 3.72\%	& 93.80\%	\\ \hline
$s_2$ & 24	& 0.86\%	& 1.33\%	& 2.33\%	& 2.28\%	& 2.92\%	& 6.77\%	\\ \hline
$s_3$ & 50	& 0.78\%	& 1.36\%	& 1.15\%	& 1.85\%	& 2.09\%	& 17.02\%	\\ \hline
$s_4$ & 42	& 2.50\%	& 8.91\%	& 3.66\%	& 8.60\%	& 23.68\%	& 23.08\%	\\ \hline
\end{tabular}
\caption{Relative error of triangle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 100	& 10000	& 100000	& 300000	& 500000	& 1000000	\\ \hline 
$s_1$ & 38610	& 36.45\%	& 33.69\%	& 22.66\%	& 46.92\%	& 22.69\%	& 13.64\%	\\ \hline
$s_2$ & 13761	& 4.85\%	& 4.73\%	& 10.08\%	& 1.77\%	& 3.92\%	& 71.67\%	\\ \hline
$s_3$ & 4851	& 5.66\%	& 5.56\%	& 7.49\%	& 15.92\%	& 22.56\%	& 90.27\%	\\ \hline
$s_4$ & 7155	& 37.48\%	& 44.77\%	& 49.72\%	& 53.29\%	& 82.59\%	& 100.00\%	\\ \hline
\end{tabular}
\caption{Relative error of 4path queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 10	& 100	& 500	& 1000	& 1500	& 10000	\\ \hline 
$s_1$ & 122	& 1.19\%	& 1.43\%	& 3.44\%	& 0.84\%	& 4.40\%	& 4.77\%	\\ \hline
$s_2$ & 47	& 0.99\%	& 2.17\%	& 1.61\%	& 24.19\%	& 61.34\%	& 46.03\%	\\ \hline
$s_3$ & 61	& 19.28\%	& 34.63\%	& 13.02\%	& 51.76\%	& 42.63\%	& 99.82\%	\\ \hline
$s_4$ & 304	& 23.16\%	& 23.44\%	& 33.20\%	& 48.59\%	& 43.70\%	& 94.99\%	\\ \hline
\end{tabular}
\caption{Relative error of 4cycle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 1	& 10	& 30	& 50	& 100	& 1000	\\ \hline 
$s_1$ & 19	& 3.60\%	& 3.40\%	& 25.73\%	& 11.76\%	& 80.56\%	& 99.67\%	\\ \hline
$s_2$ & 11	& 4.19\%	& 11.58\%	& 11.61\%	& 7.96\%	& 27.71\%	& 92.16\%	\\ \hline
$s_3$ & 20	& 10.27\%	& 17.96\%	& 17.40\%	& 42.85\%	& 10.10\%	& 51.06\%	\\ \hline
$s_4$ & 20	& 3.04\%	& 3.16\%	& 11.91\%	& 24.32\%	& 9.56\%	& 98.66\%	\\ \hline
\end{tabular}
\caption{Relative error of 4star queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}


\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{1}	& \multicolumn{3}{c|}{30}	& \multicolumn{3}{c|}{50}	& \multicolumn{3}{c|}{80}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{1000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 20	& 13.0 &5.48\% & 4.72\%	& 18.5 &0.00\% & 4.60\%	& 11.0 &18.87\% & 21.48\%	& 12.5 &10.36\% & 21.19\%	& 33.0 &0.00\% & 3.72\%	& 6.5 &55.45\% & 93.80\%	\\ \hline
$s_2$ & 24	& 22.5 &0.22\% & 0.86\%	& 21.0 &2.14\% & 1.33\%	& 41.0 &0.22\% & 2.33\%	& 22.0 &1.07\% & 2.28\%	& 34.5 &1.07\% & 2.92\%	& 192.0 &0.00\% & 6.77\%	\\ \hline
$s_3$ & 50	& 30.0 &1.23\% & 0.78\%	& 29.5 &1.37\% & 1.36\%	& 30.0 &1.02\% & 1.15\%	& 29.5 &1.37\% & 1.85\%	& 29.5 &1.56\% & 2.09\%	& 22.5 &11.82\% & 17.02\%	\\ \hline
$s_4$ & 42	& 22.5 &2.53\% & 2.50\%	& 20.0 &9.42\% & 8.91\%	& 27.0 &0.00\% & 3.66\%	& 21.5 &5.47\% & 8.60\%	& 15.0 &23.53\% & 23.68\%	& 242.0 &0.00\% & 23.08\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of triangle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{10000}	& \multicolumn{3}{c|}{100000}	& \multicolumn{3}{c|}{300000}	& \multicolumn{3}{c|}{500000}	& \multicolumn{3}{c|}{1000000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 38610	& 15870.5 &37.34\% & 36.45\%	& 17155.5 &33.46\% & 33.69\%	& 21713.5 &21.35\% & 22.66\%	& 14503.0 &46.69\% & 46.92\%	& 39623.0 &1.90\% & 22.69\%	& 106709.0 &0.00\% & 13.64\%	\\ \hline
$s_2$ & 13761	& 10761.5 &5.02\% & 4.85\%	& 10879.5 &4.67\% & 4.73\%	& 9825.0 &9.99\% & 10.08\%	& 73070.0 &0.00\% & 1.77\%	& 124692.5 &0.00\% & 3.92\%	& 5567.0 &71.68\% & 71.67\%	\\ \hline
$s_3$ & 4851	& 3629.0 &5.56\% & 5.66\%	& 3700.5 &5.29\% & 5.56\%	& 4576.5 &4.69\% & 7.49\%	& 37302.5 &0.00\% & 15.92\%	& 16009.5 &21.55\% & 22.56\%	& 23682.0 &50.00\% & 90.27\%	\\ \hline
$s_4$ & 7155	& 3506.5 &38.55\% & 37.48\%	& 3186.5 &45.40\% & 44.77\%	& 2989.0 &51.63\% & 49.72\%	& 11697.5 &3.46\% & 53.29\%	& 23191.0 &50.00\% & 82.59\%	& 1720.0 &69.27\% & 100.00\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4path queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{10}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{500}	& \multicolumn{3}{c|}{1000}	& \multicolumn{3}{c|}{1500}	& \multicolumn{3}{c|}{10000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 122	& 111.0 &1.46\% & 1.19\%	& 109.5 &1.74\% & 1.43\%	& 109.0 &2.76\% & 3.44\%	& 292.5 &0.00\% & 0.84\%	& 106.5 &2.35\% & 4.40\%	& 98.0 &5.14\% & 4.77\%	\\ \hline
$s_2$ & 47	& 44.0 &0.71\% & 0.99\%	& 44.0 &0.71\% & 2.17\%	& 151.5 &0.00\% & 1.61\%	& 35.0 &20.93\% & 24.19\%	& 93.0 &50.00\% & 61.34\%	& 1802.0 &0.00\% & 46.03\%	\\ \hline
$s_3$ & 61	& 43.5 &22.75\% & 19.28\%	& 34.0 &34.07\% & 34.63\%	& 91.5 &0.80\% & 13.02\%	& 39.0 &38.29\% & 51.76\%	& 323.0 &0.00\% & 42.63\%	& 644.0 &0.00\% & 99.82\%	\\ \hline
$s_4$ & 304	& 190.0 &23.91\% & 23.16\%	& 197.0 &23.51\% & 23.44\%	& 174.5 &28.40\% & 33.20\%	& 118.0 &48.25\% & 48.59\%	& 179.5 &28.86\% & 43.70\%	& 16.0 &95.25\% & 94.99\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4cycle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{1}	& \multicolumn{3}{c|}{10}	& \multicolumn{3}{c|}{30}	& \multicolumn{3}{c|}{50}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{1000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 19	& 15.0 &0.00\% & 3.60\%	& 17.0 &0.00\% & 3.40\%	& 13.0 &12.88\% & 25.73\%	& 14.5 &3.39\% & 11.76\%	& 5.5 &79.37\% & 80.56\%	& 1.0 &99.70\% & 99.67\%	\\ \hline
$s_2$ & 11	& 10.0 &2.22\% & 4.19\%	& 8.0 &12.80\% & 11.58\%	& 9.5 &3.00\% & 11.61\%	& 8.5 &8.62\% & 7.96\%	& 7.5 &21.96\% & 27.71\%	& 430.5 &0.00\% & 92.16\%	\\ \hline
$s_3$ & 20	& 16.0 &7.82\% & 10.27\%	& 14.5 &16.33\% & 17.96\%	& 35.0 &3.91\% & 17.40\%	& 14.0 &18.37\% & 42.85\%	& 68.0 &0.00\% & 10.10\%	& 148.0 &0.00\% & 51.06\%	\\ \hline
$s_4$ & 20	& 17.0 &3.60\% & 3.04\%	& 18.5 &1.22\% & 3.16\%	& 15.0 &12.30\% & 11.91\%	& 12.5 &24.66\% & 24.32\%	& 33.5 &0.00\% & 9.56\%	& 1.0 &98.72\% & 98.66\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4star queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}


\clearpage
\onecolumn

%\begin{table*}[t!]
%\usepackage{longtable}
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
qtype & setting & $|IN|$ & $|\reprdomain|$ & $|OUT|$ & relations & $|IN|$ & $\reprdomain$ & attr & $\actdomain$ & $\reprdomain$ & mf \\ \hline
\endhead
\multirow{24}{*}{$\qtri$} & \multirow{6}{*}{$s_1$} & \multirow{6}{*}{3434} & \multirow{6}{*}{15107} & \multirow{6}{*}{1844} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{4747} & A & 70 & 101 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 47 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle13} & \multirow{2}{*}{546} & \multirow{2}{*}{7070} & C & 47 & 101 & 27 \\ \cline{9-12} 
& & & & & & & & B & 47 & 70 & 27 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{3290} & C & 101 & 47 & 54 \\ \cline{9-12} 
& & & & & & & & A & 101 & 70 & 54 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{6}{*}{$s_2$} & \multirow{6}{*}{11194} & \multirow{6}{*}{31325} & \multirow{6}{*}{10366} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{2925} & A & 200 & 25 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{5000} & C & 117 & 25 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle2} & \multirow{2}{*}{462} & \multirow{2}{*}{23400} & C & 25 & 117 & 24 \\ \cline{9-12} 
& & & & & & & & A & 25 & 200 & 24 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{6}{*}{$s_3$} & \multirow{6}{*}{12296} & \multirow{6}{*}{46224} & \multirow{6}{*}{20751} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{8424} & A & 200 & 72 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{14400} & C & 117 & 72 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle13} & \multirow{2}{*}{1564} & \multirow{2}{*}{23400} & C & 72 & 117 & 50 \\ \cline{9-12} 
& & & & & & & & A & 72 & 200 & 50 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{6}{*}{$s_4$} & \multirow{6}{*}{3840} & \multirow{6}{*}{11270} & \multirow{6}{*}{3800} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{2940} & A & 70 & 84 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 35 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle12} & \multirow{2}{*}{408} & \multirow{2}{*}{5880} & C & 35 & 84 & 23 \\ \cline{9-12} 
& & & & & & & & B & 35 & 70 & 23 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle4} & \multirow{2}{*}{2126} & \multirow{2}{*}{2450} & C & 84 & 35 & 64 \\ \cline{9-12} 
& & & & & & & & A & 84 & 70 & 64 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{32}{*}{$\qpath$} & \multirow{8}{*}{$s_1$} & \multirow{8}{*}{5422} & \multirow{8}{*}{9415} & \multirow{8}{*}{2807163} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{0} & A & 70 & 0 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 35 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle12} & \multirow{2}{*}{408} & \multirow{2}{*}{5880} & C & 35 & 84 & 23 \\ \cline{9-12} 
& & & & & & & & B & 35 & 70 & 23 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle4} & \multirow{2}{*}{2126} & \multirow{2}{*}{3535} & C & 84 & 35 & 64 \\ \cline{9-12} 
& & & & & & & & D & 84 & 101 & 64 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{0} & E & 101 & 0 & 54 \\ \cline{9-12} 
& & & & & & & & D & 101 & 84 & 54 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_2$} & \multirow{8}{*}{12762} & \multirow{8}{*}{19197} & \multirow{8}{*}{9256927} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{0} & A & 200 & 0 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{14400} & C & 117 & 72 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle13} & \multirow{2}{*}{1564} & \multirow{2}{*}{4797} & C & 72 & 117 & 50 \\ \cline{9-12} 
& & & & & & & & D & 72 & 41 & 50 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{0} & E & 41 & 0 & 30 \\ \cline{9-12} 
& & & & & & & & D & 41 & 72 & 30 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_3$} & \multirow{8}{*}{11660} & \multirow{8}{*}{9797} & \multirow{8}{*}{2012183} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{0} & A & 200 & 0 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{5000} & C & 117 & 25 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle2} & \multirow{2}{*}{462} & \multirow{2}{*}{4797} & C & 25 & 117 & 24 \\ \cline{9-12} 
& & & & & & & & D & 25 & 41 & 24 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{0} & E & 41 & 0 & 30 \\ \cline{9-12} 
& & & & & & & & D & 41 & 25 & 30 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_4$} & \multirow{8}{*}{3570} & \multirow{8}{*}{6567} & \multirow{8}{*}{388576} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{0} & A & 70 & 0 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 47 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle13} & \multirow{2}{*}{546} & \multirow{2}{*}{1820} & C & 47 & 26 & 27 \\ \cline{9-12} 
& & & & & & & & B & 47 & 70 & 27 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle8} & \multirow{2}{*}{136} & \multirow{2}{*}{4747} & C & 26 & 47 & 13 \\ \cline{9-12} 
& & & & & & & & D & 26 & 101 & 13 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{0} & E & 101 & 0 & 54 \\ \cline{9-12} 
& & & & & & & & D & 101 & 26 & 54 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{32}{*}{$\qcycle$} & \multirow{8}{*}{$s_1$} & \multirow{8}{*}{12762} & \multirow{8}{*}{38394} & \multirow{8}{*}{79207} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{4797} & A & 200 & 41 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{14400} & C & 117 & 72 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle13} & \multirow{2}{*}{1564} & \multirow{2}{*}{4797} & C & 72 & 117 & 50 \\ \cline{9-12} 
& & & & & & & & D & 72 & 41 & 50 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{14400} & D & 41 & 72 & 30 \\ \cline{9-12} 
& & & & & & & & A & 41 & 200 & 30 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_2$} & \multirow{8}{*}{11660} & \multirow{8}{*}{19594} & \multirow{8}{*}{19737} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{4797} & A & 200 & 41 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 117 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{5000} & C & 117 & 25 & 76 \\ \cline{9-12} 
& & & & & & & & B & 117 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle2} & \multirow{2}{*}{462} & \multirow{2}{*}{4797} & C & 25 & 117 & 24 \\ \cline{9-12} 
& & & & & & & & D & 25 & 41 & 24 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{5000} & D & 41 & 25 & 30 \\ \cline{9-12} 
& & & & & & & & A & 41 & 200 & 30 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_3$} & \multirow{8}{*}{3570} & \multirow{8}{*}{13134} & \multirow{8}{*}{3825} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{4747} & A & 70 & 101 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 47 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle13} & \multirow{2}{*}{546} & \multirow{2}{*}{1820} & C & 47 & 26 & 27 \\ \cline{9-12} 
& & & & & & & & B & 47 & 70 & 27 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle8} & \multirow{2}{*}{136} & \multirow{2}{*}{4747} & C & 26 & 47 & 13 \\ \cline{9-12} 
& & & & & & & & D & 26 & 101 & 13 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{1820} & D & 101 & 26 & 54 \\ \cline{9-12} 
& & & & & & & & A & 101 & 70 & 54 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{8}{*}{$s_4$} & \multirow{8}{*}{5422} & \multirow{8}{*}{18830} & \multirow{8}{*}{24166} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{3535} & A & 70 & 101 & 45 \\ \cline{9-12} 
& & & & & & & & B & 70 & 35 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle12} & \multirow{2}{*}{408} & \multirow{2}{*}{5880} & C & 35 & 84 & 23 \\ \cline{9-12} 
& & & & & & & & B & 35 & 70 & 23 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle4} & \multirow{2}{*}{2126} & \multirow{2}{*}{3535} & C & 84 & 35 & 64 \\ \cline{9-12} 
& & & & & & & & D & 84 & 101 & 64 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{5880} & D & 101 & 84 & 54 \\ \cline{9-12} 
& & & & & & & & A & 101 & 70 & 54 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{36}{*}{$\qstar$} & \multirow{9}{*}{$s_1$} & \multirow{9}{*}{8784} & \multirow{9}{*}{16220} & \multirow{9}{*}{1328} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{760} & A & 35 & 38 & 45 \\ \cline{9-12} 
& & & & & & & & B & 20 & 20 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle12} & \multirow{2}{*}{408} & \multirow{2}{*}{760} & C & 20 & 38 & 23 \\ \cline{9-12} 
& & & & & & & & B & 20 & 20 & 23 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle4} & \multirow{2}{*}{2126} & \multirow{2}{*}{700} & C & 38 & 20 & 64 \\ \cline{9-12} 
& & & & & & & & A & 38 & 35 & 64 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{3}{*}{tri\_source\_686\_circle\_circle13} & \multirow{3}{*}{4944} & \multirow{3}{*}{14000} & C & 41 & 20 & 346 \\ \cline{9-12} 
& & & & & & & & A & 41 & 35 & 346 \\ \cline{9-12} 
& & & & & & & & B & 41 & 20 & 346 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{9}{*}{$s_2$} & \multirow{9}{*}{9958} & \multirow{9}{*}{12331} & \multirow{9}{*}{1398} & \multirow{2}{*}{source\_686\_circle\_circle0} & \multirow{2}{*}{1306} & \multirow{2}{*}{722} & A & 16 & 19 & 45 \\ \cline{9-12} 
& & & & & & & & B & 35 & 38 & 45 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle4} & \multirow{2}{*}{2126} & \multirow{2}{*}{665} & C & 19 & 19 & 64 \\ \cline{9-12} 
& & & & & & & & B & 38 & 35 & 64 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_686\_circle\_circle9} & \multirow{2}{*}{1582} & \multirow{2}{*}{304} & C & 19 & 19 & 54 \\ \cline{9-12} 
& & & & & & & & A & 19 & 16 & 54 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{3}{*}{tri\_source\_686\_circle\_circle13} & \multirow{3}{*}{4944} & \multirow{3}{*}{10640} & C & 41 & 19 & 346 \\ \cline{9-12} 
& & & & & & & & A & 41 & 16 & 346 \\ \cline{9-12} 
& & & & & & & & B & 41 & 35 & 346 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{9}{*}{$s_3$} & \multirow{9}{*}{127250} & \multirow{9}{*}{8160} & \multirow{9}{*}{1369} & \multirow{2}{*}{source\_348\_circle\_circle1} & \multirow{2}{*}{6246} & \multirow{2}{*}{888} & A & 24 & 24 & 99 \\ \cline{9-12} 
& & & & & & & & B & 37 & 37 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle13} & \multirow{2}{*}{1564} & \multirow{2}{*}{888} & C & 7 & 24 & 50 \\ \cline{9-12} 
& & & & & & & & B & 37 & 37 & 50 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{168} & C & 24 & 7 & 30 \\ \cline{9-12} 
& & & & & & & & A & 24 & 24 & 30 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{3}{*}{tri\_source\_348\_circle\_circle11} & \multirow{3}{*}{118974} & \multirow{3}{*}{6216} & C & 116 & 7 & 2830 \\ \cline{9-12} 
& & & & & & & & A & 116 & 24 & 2830 \\ \cline{9-12} 
& & & & & & & & B & 116 & 37 & 2830 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
& \multirow{9}{*}{$s_4$} & \multirow{9}{*}{147090} & \multirow{9}{*}{19061} & \multirow{9}{*}{1557} & \multirow{2}{*}{source\_348\_circle\_circle11} & \multirow{2}{*}{4486} & \multirow{2}{*}{2952} & A & 24 & 41 & 76 \\ \cline{9-12} 
& & & & & & & & B & 37 & 72 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle13} & \multirow{2}{*}{1564} & \multirow{2}{*}{1517} & C & 16 & 41 & 50 \\ \cline{9-12} 
& & & & & & & & B & 72 & 37 & 50 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_circle8} & \multirow{2}{*}{466} & \multirow{2}{*}{384} & C & 41 & 16 & 30 \\ \cline{9-12} 
& & & & & & & & A & 41 & 24 & 30 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{3}{*}{tri\_source\_348\_circle\_circle1} & \multirow{3}{*}{140574} & \multirow{3}{*}{14208} & C & 194 & 16 & 3426 \\ \cline{9-12} 
& & & & & & & & A & 194 & 24 & 3426 \\ \cline{9-12} 
& & & & & & & & B & 194 & 37 & 3426 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline
\caption{Query meta stat for queries of 4 settings from 4 types. $\qtri$ is a triangle query, $\qpath$ is a path query of 4 nodes, $\qcycle$ is a 4-cycle query, $\qstar$ is a star query of 4 nodes}
\end{longtable}
%\end{tabular}
%\end{table*}

\clearpage
\twocolumn

==> exp_analysis.tex <==




%\note{The info of this figure is included in fig \ref{fig:sens_change_by_n}}
%Figure \ref{fig:sens_change_by_query} compares the tightness of local sensitivity between 'TSens' and 'Elastic' for queries q1, q2 and q3 when scale is 0.01. Notice that the local sensitivity of q3 for 'Elastic' is $1.2e8$ so we cut it in the figure.

%Figure \ref{fig:sens_change_by_table} stratifies the local sensitivity as max tuple sensitivities from each table for q1 and q2 when scale equals to 1. The figure shows if there is only one private table, how the local sensitivity will be. It also strengthen the fact that 'TSens' always achieves lower local sensitivity since it computes the tightest bound.


%	\begin{subfigure}[b]{0.3\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{sens_change_by_query.pdf}
%		\caption{Local Sensitivity vs Queries (scale=0.01)}
%		\label{fig:sens_change_by_query}
%	\end{subfigure}
%	\begin{subfigure}[b]{0.6\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{sens_change_by_table.pdf}
%		\caption{Local Sensitivity vs Tables}
%		\label{fig:sens_change_by_table}
%	\end{subfigure}






==> exp_dp__Yuchao_Tao_s_conflicted_copy_2019-10-22_.tex <==
\subsection{Differential Privacy}

\paratitle{Baseline}. \PrivSQL is a differentially private SQL answering engine that uses the truncation mechanism that truncates the database and adds the noise according to the global sensitivity of query after truncation to generate database synopses which support ad-hoc high-utility SQL query answering. It introduces the concept of policy that given primary private relations, the sensitivity of other related relations should be updated to be non-zero according to the database key constraints. We assume \texttt{CUSTOMER} is the primary private relation for q1 and q3, and \texttt{SUPPLIER} is the primary private relation for q2, so the sensitivity of \texttt{ORDERS} is affected by \texttt{CUSTOMER} and the sensitivity of \texttt{PARTSUPP} is affected by \texttt{SUPPLIER}. The sensitivity of \texttt{LINEITEM} is affected by either of them.

\PrivSQL uses the maximum frequency as the truncation threshold, which is different from using tuple sensitivity to truncate the database. Any tuple whose frequency is beyond the max frequency will be dropped from the database. \PrivSQL runs SVT to learn the truncation threshold for each relation; however, the noise scale of SVT depends on the sensitivity of the relation while it is constantly 1 in \TSensDP. 

Although the privacy budget allocation strategy affects the performance of DP algorithm, we skip exploring the effect of budget allocation and assume \PrivSQL and \TSensDP divide the privacy budget into two halves, one for the threshold learning and the other for adding noise to the query result after truncation. We disable the synopsis generation phase of \PrivSQL and just use Laplace mechanism to answer the SQL query directly.
\begin{figure*}[t!]
	\centering
	\includegraphics[trim={25, 80, 25, 50}, clip, width=.9\textwidth]{{"figures/TPSens - DP - Sheet1"}.pdf}
	\caption{Application to Differential Privacy: Comparing \TSensDP error to \PrivSQL error}
	\label{fig:dp}
	\vspace{-10pt}
\end{figure*}
\paratitle{Result and Analysis}. Figure \ref{fig:dp} shows the statistics of releasing differential private query results by \TSensDP or \PrivSQL. We assume the table size is given and assume the maximum tuple sensitivity of q1 is 100, of q2 is 500 and of q3 is 10. We run each algorithm 10 times and report the average of global sensitivity, the average of relative absolute bias and the average of relative absolute error. 

The result shows that \TSensDP has a stable error for simple or complex queries as its relative error is always below 25\%. It can be more than 1,000,000\% accurate than \PrivSQL for q3. Although \TSens has within 2\% higher relative bias than \PrivSQL for q1 and q3, the global sensitivity is 2x and 800,000x smaller than \PrivSQL.



==> exp_procedure.tex <==




%\am{We solve the "Sensitivity problem" -- find the tuple that corresponds to the highest local sensitivity and compute the local sensitivity. How does elastic sensitivity solve this problem? If it does not, you need to create a baseline method that can extrapolate a tuple that corresponds to the local sensitivity. Also, what is the "error metric" for our problem? If you are returning just LS, then smaller is better. But if you are also returning the tuple with the highest sensitivity, then what is error? }
%\yc{We can mainly focus comparing sensitivity with Elastic, and just report the tuple that we found. The usefulness of tracking the tuple will be emphasized in the application and its experiment.}

==> exp_sensitivity__Yuchao_Tao_s_conflicted_copy_2019-10-22_.tex <==
\vspace{-2em}
\subsection{Local Sensitivity}
\noindent\textbf{Baseline}. \Elastic assumes the maximum frequency of the join attributes in each table is given. This algorithm traverses the join tree to update the local sensitivity by tracking the change of max frequency. We remove the assumption and let \Elastic pre-process the database to compute the max frequency thus the algorithm output is a local sensitivity upper bound. We also extend the algorithm to support cross-product by assigning the max frequency of empty attributes as the size of the table. Since we represent a general join counting query as a join plan, we change the input to \Elastic to be the join plan as \TSens uses so that the join order in the experiment is the same. We define the join order as a post-traversal of the join plan.

\TSens reports the most sensitive tuple by tracking each tuple sensitivity and it also finds the most sensitive tuple for each relation within the procedure; however, \Elastic cannot find the most sensitive tuple, although it can find the local sensitivity upper bound. We report the most sensitive tuple for each relation while also reports its elastic sensitivity by setting this relation as the only sensitive tuple for \Elastic.

\paratitle{Result and Analysis}.
Figure \ref{fig:sens_change_by_n} shows the local sensitivity trend in aspect to the scale. Notice that after scale 0.001, \TSens has in average 7x smaller and 6x smaller of the local sensitivity for q1 and q2  then \Elastic has. Moreover, for q3, \TSens achieves 2,200,000x smaller value for the local sensitivity than \Elastic does when scale equals to 0.1. We didn't run q3 for scale larger than 0.1 due to the memory limit issue.

%\am{What does scale of 0.01 mean? If you had a large machine on AWS, would that query complete?}

Figure \ref{fig:time_change_by_n} shows the time cost for both \TSens and \Elastic for different queries and scales. The third line $q_i\_query$ is the time to evaluate the join plan as a counting query efficiently. For q1 and q2, both \TSens and \Elastic shows a tight relation to the time of query evaluation, which takes in average 1.8x and 0.9x of the query evaluation time after scale 0.001. For q3, although \Elastic is much faster, \TSens only takes in average 4.2x of the query evaluation time to find in average 60,000x smaller local sensitivity before scale 1.

Figure \ref{fig:sens_tuple} shows the most sensitive tuple for each relation for q3 at scale = 0.01. Each tuple sensitivity is below 1,000 while the least elastic sensitivity is beyond 10,000. We skip finding the most sensitive tuple in LINEITEM since it has the superkey in the query head and thus the tuple sensitivity is at most 1.

\begin{figure*}[t!]
	\centering
		\begin{subfigure}[b]{0.44\textwidth}
		\centering
        	\includegraphics[width=.8\textwidth, trim={0 0 10 0}, clip]{sens_change_by_n.pdf}
        	\caption{Local sensitivity reported by \TSens and \Elastic for queries q1, q2 and q3 on datasets of differing scales }
        	\label{fig:sens_change_by_n}
        \end{subfigure} \ 
        \begin{subfigure}[b]{0.48\textwidth}
        	\centering
        	\includegraphics[trim={45, 120, 45, 50}, clip, width=.8\textwidth]{{"figures/TPSens - Experiment - MostSensitiveTuple2"}.pdf}
        	\caption{Most sensitive tuples and their tuple sensitivities for each relation of q3 when scale = 0.01. %The right column is the corresponding elastic sensitivity when setting each relation as the only sensitive relation.
        	}
        	\label{fig:sens_tuple}
        \end{subfigure}
   	\vspace{-10pt}
    \caption{Local sensitivity reported by \TSens versus \Elastic}
    \vspace{-10pt}
\end{figure*}

\begin{figure*}[t!]
	\centering
	\includegraphics[width=\textwidth, trim={10 16 10 10}, clip]{time_change_by_n.pdf}
	\vspace{-20pt}
	\caption{The trend of time usage in terms of various scales for queries q1, q2 and q3 and algorithms \TSens and \Elastic. The base line `query' shows the query evaluation time.}
	\label{fig:time_change_by_n}
	\vspace{-10pt}
\end{figure*}

==> extensions.tex <==
\subsection{Extensions}\label{sec:extensions}

\paratitle{Extension to non-acyclic join queries that satisfies a property on query hypertree}.
%\sr{only a subclass right? update the heading} 
For non-acyclic CQs, we use \emph{generalized hypertree decompositions} of the query \cite{adler2007hypertree}\footnote{There are multiple other equivalent notion of decompositions and width of general CQs, like \emph{tree width, query width}, or \emph{fractional hypertree width} \cite{Gottlob+1999, Abiteboul+1995, Chekuri:1997, Grohe:2001, Gottlob:2016}. Having a bound on these widths leads to polynomial time evaluation for general CQs.}. 
A generalized hypertree $\tree_Q$ associated with a conjunctive query $Q$ is a tree with nodes labeled with attributes of the query $Q$ such that (1) for each relation, there is a node that covers its attributes, 
%each node contains one or multiple relational atoms, 
and (2) for each attribute $A$, the nodes in 
$\tree_Q$ containing the same attribute form a sub-tree. 
A join plan can be derived from a generalized hypertree by replacing each node of the tree with joins among relations whose attributes cover the node attributes as an \emph{inner join plan}, and then the tree itself forms an \emph{outer join plan}. It can be seen that when each node in $\tree_Q$ can be replaced with a unique single relation, it is a simple \emph{join-tree} of $Q$, which holds if and only if $Q$ is acyclic. %(Section~\ref{sec:acyclic}). 

\emph{If we find a join plan where each relation only appears once} (which may not hold for arbitrary CQ), we can extend Algorithm \ref{algo:gj_query} for this join plan, since its outer join plan is an acyclic join tree, and each inner join plan can be regarded as a node in the join tree by computing the join of the relations in that node. After computing topjoins and botjoins, to compute the frequency table for each original relation $R_i$, in step III) of Algorithm~\ref{algo:gj_query} while computing $T^i$, we also include the other relations $R_{\ell}$ in the join expression that belong to the same node in the tree as $R_i$ (see \eqref{eq:general_gj_sub_query}). This computation can be done more efficiently as we discuss in the experiments (Section~\ref{sec:experiments}). 
%joins among other relations as cohorts in the node, and divide them into disjoint groups sharing no common attributes and compute the partial frequency table for each group. 
%We then select the tuple of max frequency from each partial frequency table and merge them back as the most sensitive tuple for this relation. The rest of the algorithm is similar to Algorithm \ref{algo:gj_query}.

Since each node can contain multiple relations, the size of each node can be more than $n$. If there are at most $p$ relations within a node of the join plan, the size of the partial join within this node is $O(n^p)$. Replacing $n$ with $O(n^p)$ in Theorem~\ref{thm:gj_query} results in the time complexity as $O(m p n^{pd} d\log n)$ for non-acyclic join queries satisfying this property on $\tree_Q$. 
%For an \emph{optimal} hypertree decomposition $\tree_Q$, if it also satisfies the property of one relation in at most one node, then $p$ is related to 
($p$ can be replaced with the the \emph{generalized hypertreewidth} for an `optimal' $\tree_Q$ and mapping of relations to nodes of $\tree_Q$). %\sr{verify}

\paratitle{Extension to selection.} 
%Although by default each relation appears in the query body is the original base table, with extra rules, the algorithm 
Algorithm~\ref{algo:gj_query} can handle queries  with arbitrary selection conditions (that can be applied to each tuple individually in any relation) in the body of the query. 
%where $\attributes \subseteq \cup_i \attributes_i$.
%For each tuple: 1) the tuple sensitivity is not affected by projection since we assume projection keeps duplicates. 2) if the tuple fails to satisfy the selection predicates, 
We start with the sub-instance where each tuple in each relation satisfies the selection condition, and when we compute the final $\cnt$ values, we discard the candidate tuples that do not satisfy the selection condition since they cannot affect the result. 
%we set the tuple sensitivity as 0, since it is dropped by selection before it can join other tuples. Applying rules 1 and 2 will not affect the complexity.

\paratitle{Extension to disjoint query components.} 
If the hypergraph of query is not connected, e.g., $Q(A, B, C, D) :- R_1(A, B), R_2(B, C), R_3(D)$, we get a join forest containing multiple disjoint join trees instead of a single join tree for a query. In this case, we run our algorithm for each join tree. We then update the tuple sensitivity by multiplying it with the join size of other join trees, for which we can use existing algorithms for acyclic joins that run in polynomial size in the input and output \cite{Yannakakis:1981}, and algorithms using generalized hypertree decomposition for non-acyclic queries \cite{Gottlob:2016}. The join size of each join tree can be computed as the sum of frequency from the botjoin of each join tree root, so it will not affect the complexity. 

\paratitle{Extension to attributes appearing in only one relation.}
%\sr{for attributes in one relation, please complete}  
If an attribute  $A$ appears in only one relation $R_i$,  and $R_i$ is joined with other relations by other attributes in the query $Q$, then $A$ does not affect the local sensitivity of $Q$, but  the  tuple $t$ with  the maximum tuple sensitivity may be from $R_i$, so we  would  need to choose a value for $t.A$ in the final output. Similar to Algorithm~\ref{algo:ls_pathquery}, if the attributes in $R_i$ except $A$ come from an  existing tuple $t'$  in  the  instance, we augment it with $t'.A$ (for downward sensitivity). If there are no such tuples $t'$, we choose any value from the active domain of $A$ to extend the other attributes to form such a tuple $t$ (for upward sensitivity). 

==> future.tex <==
\revm{
\section{Future Work}\label{sec:future}
\begin{enumerate}
    \item Self-joins. Acyclic join queries with self-joins can not be captured by our algorithms, because we only allow one relation appear once in the query. For each relation, we compute the joins for the rest of relations to summarize how tuples from this relation can affect the full join. A possible workaround is to join the repeated base relations as a single and combined relation, run our algorithm, and then link the effect of adding or removing a tuple from the base relation to the combined relation and the effect of adding a removing a tuple from the combined relation to the rest. However, it is not clear what is the representative domain in this case, which makes the max upward tuple sensitivity unknown.
    \item Top k frequency tables. As the experiment shows, the frequency tables that topjoins and botjoins compute can grow quadratically to the input size or even more depending on the queries. To make it scalable, instead of keeping the full frequency table, we can only keep the top k entries and assume that the rest in the active domain all have frequency 1 and others have frequency 0. This gives an upper bound of the tuple sensitivity, which provides a knob on scalability and tightness.
    \item Infer tuple sensitivities through database constraints. Constraints like functional dependencies can imply tuple sensitivities without computing the frequency table. For example, for query Q(A,B,C) :- R1(\underline{A}), R2(\underline{B}, A), R3(\underline{C}, B) where underlined attributes are keys, the tuple sensitivities for tuples from R3 is always at most 1, since it can at most join one tuple in R2, and this tuple in R2 can at most join one tuple in R1. 
\end{enumerate}
}

==> generaljoin--OLD.tex <==
\section{General Join Query}\label{sec:general}
 
\begin{algorithm}[t]
	\small
	\caption{Compute Local Sensitivity of a General Join Query and the corresponding Most Sensitive Tuple} 
	\label{algo:gj_query}
	\begin{algorithmic}[1]
		\Require General join query $\Qgjoin(\attributes_\database)$
		%$\Qgjoin(\attr_0 \ldots \attr_m)$, 
		the database $\database$
		\Ensure $\LS(Q,D)$, and the most sensitive tuple $\kingtuple$
		\Procedure {LS}{$\Qgjoin, \database$}
		\Statex I) Prepare nodes
		\For{all nodes $v_j\in V$}
		    %\State $v_j = \underset{\forall \R{i} \in v_j }{\superjoin} \R{i}$
		    \State $v_j = \superjoin(\{\R{i} \in v_j\})$
		\EndFor
		\Statex II) Prepare botjoin
		\For{$j$ in postoder}
		\If{$v_j$ is a leaf}
		\State $\botjoin(v_i) = \groupbyagg{\attributes_{v_j,p(v_j)}}(v_j) $
		%\aggregate{\attributes_{v_i,p(v_i)}}{count(*) \as \cntt{v_i}{p(v_i)}}{v_i}$
		%\ElsIf {$v_i$ is the root}
		%\State pass
		\ElsIf{$v_j$ is not the root}
		\State $\botjoin(v_j) =  \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin (v_j, \{\botjoin(v_{j'})~|~v_{j'}\in C(v_j)\})$ 
		%(\und%erset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))$
		%\State $\botjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\EndIf
		\EndFor
		\Statex III) Prepare topjoin
		\For{$j$ in preoder}
		%\If{$v_j$ is the root}
		%\State pass
		\If {$p(v_j)$ is the root}
		%\ElsIf {$p(v_i)$ is the root}
		%\State  $S =
	    %p(v_i) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j), \{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \}) $
		\ElsIf{$v_j$ is not root}
		%\State  $S =
		%p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S $
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j),\topjoin(v_j),\{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \})$
		\EndIf
		\EndFor
		\Statex IV) Prepare frequency tables of nodes
		\For{$j=1, \dots, m'$}
		\If {$v_j$ is the root}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%\aggregate{\attributes_{v_i}}{sum(\underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{} \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j)$		
		\ElsIf {$v_j$ is a leaf}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}} (\topjoin{v_j})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)}) \as  c}{} \topjoin(v_i)$
		\Else 
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\topjoin{(v_j)},\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)} \underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{	\topjoin(v_i) \superjoin ( \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j))}$
		\EndIf
		\EndFor

		\Statex V) Select  the most sensitive tuple
		\For{$i=1, \ldots, m$}
		%\note{Improve the efficiency later}
		\State $T^i = \groupbyagg{\attributes_i}\superjoin(T^{\pi(R_i)}, H(R_i))$
		%$\Qgfreq^i =  \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}	\Qgfreq^{\pi(v_i)} \superjoin 		\underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}		$
		\EndFor
		\State $t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt$
		%\Statex VI) Select most sensitive tuple
		%\For{$i=1, \ldots, m$}
		%\State $t_i = \argmax_{\tsens} \pi_{\tsens_i \as \tsens} \Qgfreq^i$
		%\EndFor 
		%\State $t = \argmax_{\tsens}{t_1, \ldots, t_m}$
		%\State $\LS = t.\tsens$
		\State $\LS = t^*.\cnt$ 
		\State \textbf{return} $\LS, t^*$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}



Path join queries only cover a small subset of all conjunctive queries. In this section, we discuss the general solution to general conjunctive queries (Section~\ref{sec:general-approach}), and then present an efficient algorithm with additional parameters in the running time complexity of the algorithm (Section~\ref{sec:general-algo}). Finally, we  discuss a class of queries that  we call \emph{doubly-acyclic queries} generalizing path  queries where these parameters are gone. 

We assume that there are no self joins in the queries; i.e., there are no duplicated relations in the query body. For simplicity, we assume that the CQ is a full CQ of the following form: 
\begin{align*}
\Qgjoin(\attributes_\database) :- \relation_1(\attributes_1), \ldots, \relation_m(\attributes_m), 
\end{align*}
%where $\attributes_i$ is the attribute set of the table $\relation_i$.
%, which at most has $k$ attributes.
%We also call attributes as variables and relations as atoms. 
We assume that the query hypergraph (Section~\ref{sec:acyclic}) is connected. We also assume each attribute appears in at least two relations in the body. We also assume that there are no selections in the body, and no projections in the head of the query, i.e., $\attributes_\database = \cup_{i=1}^m \attributes_i$, and the total number of attributes $|\attributes_\database|$ is $k$. These assumptions, except the no-self-join assumption (which introduces new challenges and we leave it as a future direction), are without loss of generality as how they can be relaxed using our algorithm is discussed in Section~\ref{sec:extensions}. 

\subsection{Basic Idea and Query Hypertrees}\label{sec:general-approach}
To compute the local sensitivity of a general CQ, the basic idea is similar to that in the path join case. 

\begin{itemize}
    \item[(i)] For each $i=1,\ldots,m$, compute
%For general join queries, we define $\Qgjoin^i(\attributes_\database)$ as:
\begin{align}\label{eq:general_gj_sub_query}
S^i = \superjoin(R_1,\ldots,R_{i-1}, R_{i+1},\ldots, R_m)
%\Qgjoin^i(\attributes_\database) \datalogEQ
%& \relation_1(\attributes_1), \ldots, \relation_{i-1}(\attributes_{i-1}), \nonumber \\
%& \relation_{i+1}(\attributes_{i+1}), \ldots, \relation_m(\attributes_m) 
\end{align}
%which is a sub-query from the original join query by removing the relation $\relation_i$. 
\item[(ii)] For each $i=1,\ldots, m$, compute 
%Then we do a counting group by on attributes $\attributes_i$.
\begin{align}\label{eq:general_gj_freq}
%\Qgfreq^i(\attributes_\database) = 
T^i = \groupbyagg{\attributes_i}(S^i)
%{\aggregate{\attributes_i}{count(*) \as c}{\Qgjoin^i(\attributes_\database)}}
\end{align}
%to count the frequency of each tuple.

\item[(iii)] Finally, return the most sensitive tuple:
%To find the most sensitive tuple, we pick the tuple from the above query who has the largest frequency $c$.
\begin{align} \label{eq:general_gj_most_sensitive_tuple}
%t^*_i = \argmax_{c} \Qgfreq^i(\attributes_\database)
t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt
\end{align}
\end{itemize}

\cut{
\begin{proposition}
The tuple $t^*$ returned by Equation~\eqref{eq:general_gj_most_sensitive_tuple} gives the most sensitive tuple with its sensitivity $t^*.\cnt$.
%as $t^*.\attributes$ and its tuple frequency $t^*.\cnt$ from the domain of table $\relation_i$.
\end{proposition}
\begin{proof}
	By definition, Equation~\eqref{eq:general_gj_freq} computes and stores the tuple sensitivity as $\cnt$ for each $\attributes_i$ appears in $S^i$. $S^i$ covers the \representative domain of $\attributes_i$ by the construction rule. 
    Since all tuples outside this \representative domain has sensitivity 0, searching tuples within this domain can guarantee finding the most sensitive tuple and its corresponding sensitivity. 
\end{proof}

Although this approach gives us the correct result, the size of the sub-query $S^i$ in worst case could be $\Omega(n^{m-1})$.
The size of $T^i$ in worst case could be $\Omega(n^k)$.
In conclusion, this naive approach is polynomial in data complexity, but may be exponential in combined complexity.
}

Once again, the size of the sub-queries $S^i$ can be exponential in $m$ or $k$, which is polynomial in data complexity, but may not be efficient for practical purposes. 
To design an efficient algorithm for general CQs, we use \emph{hypertree decompositions} of the query \cite{Gottlob+1999, Abiteboul+1995}, which we briefly review below\footnote{There are multiple other equivalent notion of decompositions and width of general CQs, like \emph{generalized hypertree width, tree width, query width}, or \emph{fractional hypertree width} \cite{Chekuri:1997, Grohe:2001, Gottlob:2016}. Having a bound on these widths leads to polynomial time evaluation  for general CQs. We choose hypertree width as we needed that each relation in the query appears in only one node in the hypertree decomposition}. 

\stitle{Hypertree Decomposition.}
A hypertree $\tree_Q$ associated with a conjunctive query $Q$ is a tree with nodes labeled with attributes of the query $Q$ such that (1) each node in the  tree contains one or multiple relational atoms and all their attributes, 
%each node contains one or multiple relational atoms, 
and (2) for each attribute $A$, the nodes in 
$\tree_Q$ containing the same attribute forms a sub-tree. It can be seen that when each node in $\tree_Q$ contains a single relation, it is a \emph{join-tree} of $Q$ (Section~\ref{sec:acyclic}). 
%and 3) each relation from the query appears once and only once in the hypertree. The max number of relations within a node is defined as hypertree width. 

Each query has an associated hypertree, and it can be found in polynomial time if its \emph{hypertree-width},  is bounded. Given a hypertree of width $p$ for the input query, we represent this hypertree by 
a join tree $\tree(V,E, \map)$, where $V=\{v_1,\ldots,v_{|V|}\}$, $E=\{e_1,\ldots,e_{|E|}\}$ and $\map$ maps a relation $\R{i}$ to a node $v_j$ and each edge contains the common attributes between two nodes.
%%%Mapping of relations to nodes 
The number of nodes is less than the number of relations ($|V|<m$)
since multiple relations could be merged into one node. If $\R{i}$ is contained in $v_j$, then $\pi(\R{i}) = v_j$. 
%%use i for index of relations
%%use j for index of nodes
%%%Mapping of attributes to edges
We denote the union set of attributes from all relations in $v_j$ as $\attributes_{v_j}$, and the set of join attributes between $v_{j_1}$ and $v_{j_2}$ by $\attributes_{v_{j_1},v_{j_2}}$.
%%%Other notations
Let $p(v_j)$ denote the parent of node $v_j$ in the join tree,
$C(v_j)$ denote the child nodes of $v_j$,
and $N(v_j)$ denote the neighbors of $v_j$, i.e. $C(p(v_j)) \setminus \{v_j\}$. Within a node $\pi(\R{i})$, let $H(\R{i})$ denotes the group of cohorts of $\R{i}$, i.e. $\{\R{i'} \mid \R{i'} \in \pi(\R{i'}), \R{i'} \neq \R{i}\}$.
%; let $A(\R{i})$ denotes the attributes set between $\R{i}$ and $H(\R{i})$, i.e. $\cup_{\R{j} \in H(\R{i})} \attributes_{i, j}$
We denote $\subtree(v_j)$ as the subtree rooted at $v_j$, while $\comptree(v_j)$ is the complementary graph of $\subtree(v_j)$ on the tree $\tree(V, E, \pi)$.
%%%Property of a hypertree decomposition 
Since it's a hypertree decomposition, for each attribute, the nodes that contain this attribute always form a subtree. 
\subsection{Algorithm Details}\label{sec:general-algo}

%\todo{Add an introduction to the hypertree decomposition}. 
We present an algorithm based on a hypertree decomposition of a general join query. 



%\xh{We can add a definition box for this property if it's used later.}\yc{It should be used in efficiency analysis}


\stitle{Definitions.} For each relation $R_i$, let $v_j=\pi(R_i)$, the frequency table (Equation~\eqref{eq:general_gj_freq}) can be computed from the join of three groups of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$. In order to compute $T^i$, we define \emph{topjoin} and $\emph{botjoin}$ for each node $v_j$ in the hypertree:
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\tree(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}
Similar to the frequency table for a relation (Equation~\eqref{eq:general_gj_freq}), we define the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
T^{v_j}=  
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}
For $v_j$ as root or leaf, it has a simpler formula and we will discuss it in the algorithm.
Then the frequency table for a relation can be expressed using the frequency table of its node $\pi(R_i)$ and the cohorts of $R_i$ in $\pi(R_i)$: 
\begin{align}\label{eq:gj_fast_freq}
T^i= \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(T^{\pi(R_i)}), H(\R{i})))
\end{align}

%We use $\superjoin(R_1, R_2,\ldots, R_i)$ to denote the natural join between the relations $R_1,\ldots, R_i$. 

%Similar to Equation~\eqref{eq:general_gj_sub_query}, we capture the join result without the node $v_j$ in a hypertree $T$ as:
%\begin{align}\label{eq:gj_fast_node_sub_query}
%\Qgjoin^{v_j}(\attributes_\database) =
%\superjoin(\comptree(v_j), \{T(v_{j'})~|~v_{j'}\in C(v_j) \})
%\end{align}
%which is a natural join between the complementary tree of $v_j$ and the subtrees at the children of $v_j$. 



%\begin{align}\label{eq:gj_fast_node_sub_query}\Qgjoin^{v_i}(\attributes_\database) = \comptree(v_i) \superjoin \underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j)\end{align}
%\xh{This expression in \eqref{eq:gj_fast_node_sub_query} is not clear. what do you try to join here? } \yc{The symbol $\superjoin$ actually is a natural join and it reduces to cross product if there is no common attributes. Here, I want to join every nodes except $v_i$, so we need to join each child's subtree as $\underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j) = \subtree(v_{j_1})  \superjoin \subtree(v_{j_2})  \ldots \superjoin \subtree(v_{j_p}) $ and the complementary tree $\comptree(v_i)$.} 

\eat{
Now we can rewrite the Equation~\eqref{eq:general_gj_sub_query} in step (1) as \begin{align}\label{eq:gj_fast_sub_query}
\Qgjoin^i(\attributes_\database) 
=\superjoin(\Qgjoin^{\pi(R_i)}(\attributes_\database) , H(R_i))
\end{align}
Let $v_i$ be the corresponding node of $R_i$ in the hypertree, i.e., $v_j=\pi(R_i)$. This expression joins three types of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$.
}
%\begin{align}\label{eq:gj_fast_sub_query} \Qgjoin^i(\attributes_\database) = \Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin \underset{\forall \R{j} \in H(R_i)}{\superjoin} \R{j}\end{align}

\begin{figure}
	\centering
	\includegraphics[scale=0.45]{acyclic_join_recursion.pdf}
	\caption{Example of notations. \todo{Update the figure and description} \note{edit \href{https://docs.google.com/drawings/d/1xTBbD3DY4HEqO5I21m1UiGcjLAM9rrvS0YnmI5qm_J0/edit?usp=sharing}{here} }}
	\label{fig:gj_notations}
\end{figure}

\eat{
Given a table $R_i$ in $T$, as long as we know the maximum frequency of tuples projected on $\attributes_i$ from the joint output between tables other than $R_i$ in a join tree of $\Qgjoin$, as defined by $\Qgjoin^i$, we immediately get the max change to the final joint output due to adding or removing a tuple to $R_i$, and hence the local sensitivity of the query. We define the following invariants to compute the tuple sensitivity of a general query.
}

%\xh{May use this notation earlier}. 
%First, we assume all the relations has additional attribute $C$ to record the multiplicity of the other attribute values. For the base tables, we add attribute $c$ and assign $1$ to this attribute for every tuple. We also use $\superjoinagg(R_1,\ldots,R_i)$ to summarize two steps: (i) a natural join among $R_1, R_2,\ldots, R_i$ except the attribute $c$, and (ii) project the product of these multiplicity attributes to a new multiplicity column, i.e., $$\superjoinagg(R_1,\ldots,R_i)= \pi_{(R_1.C\times \cdots R_i.C)\rightarrow C} (\superjoin(R_1,\ldots, R_i)).$$
%Let $\groupbyagg{A}(R_i)$ represent a group by attribute $A$ and sum the counts and rename the sum as a new attribute $c$, i.e., 
%$$\groupbyagg{A}(R_i)= \aggregate{A}{sum(C) \rightarrow C}{(R_i)}.$$

\eat{
For each node $v_j$, we denote $\botjoin(v_j)$ and $\topjoin(v_j)$ as tables that computes the frequency of tuples projected on attributes shared by $v_j$ and its parent $p(v_j)$ from $\subtree(v_j)$ and $\comptree(v_j)$.
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (T(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}


Denote the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
\Qgfreq^{v_j}(\attributes_\database) =  
%\aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big) 
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}

%\begin{align}\label{eq:gj_fast_node_freq}
%\Qgfreq^{v_i} =  \aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big)
%\end{align}

Now, equation (\ref{eq:general_gj_freq}) can be rewritten as:
\begin{align}\label{eq:gj_fast_freq}
\Qgfreq^i(\attributes_\database) = \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(\Qgfreq^{\pi(R_i)}), H(\R{i}))
%	(\aggregate{\attributes_i}{sum(c) \as c}{\Qgfreq^{\pi(R_i)}}) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
)
\end{align}


\begin{lemma}
	Equation (\ref{eq:general_gj_freq}) and (\ref{eq:gj_fast_freq}) for step (2) are equivalent.
\end{lemma}
\begin{proof}
    
\end{proof}
}

%\begin{proof} 
%	Replacing $\Qgjoin^i(\attributes_\database)$ by equation (\ref{eq:gj_fast_node_sub_query}) and 
%	(\ref{eq:gj_fast_sub_query}), equation (\ref{eq:general_gj_freq}) can be rewritten as
%	\begin{align*}
%	  \Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	  	\Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	  \Qgjoin^{\pi(\R{i})}(\attributes_\database) =~&
%	  	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	which is equivalent to
%	\begin{align*}
%	\Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}
%	R~ \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	R =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	Notice that the intermediate relation $R$ is equivalent to equation (\ref{eq:gj_fast_node_freq}), so 
%	$\Qgfreq^i(\attributes_\database)$ can be rewritten as
%	\begin{align*}
%	\Qgfreq^i =~ \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}\Qgfreq^{v_i} \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
%	\end{align*}
%	, which is equivalent to equation (\ref{eq:gj_fast_freq})
%\end{proof}
%The last step is the same.

\paratitle{Algorithm.} The algorithm first prepares each tree node $v_j$ as the join among tables in $v_j$. Then it prepares $\bot(v_j)$ and $\top(v_j)$ for each node, and use them to compute $T^{v_j}$ for each node $v_j$. Finally, it computes $T^{i}$ for each relation $\R{i}$ and finds the most sensitive tuple and its tuple sensitivity. 

Note that computing  botjoin $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}) and topjoin $\top(v_j)$ (Equation~\eqref{eq:gj_topjoin}) for each node again may require exponential combined complexity, so we give an iterative approach in Algorithm~\ref{algo:gj_query} to compute them in polynomial combined complexity. After preparing botjoin and topjoin for each node, the third step is to combine them together and find the most sensitive tuple. We assume all joins are merge-sort joins.


\note{Illustrate the recursive structure of topjoin and botjoin by figure (\ref{fig:gj_notations}).}


To prepare each node $v_j$, we compute the join between 
%joins as $v_j = \underset{\forall \R{j} \in v_i }{\superjoin} \R{j}$ 
the relations in $v_j$ in an arbitrary join order.

To prepare $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}), we start from the leaf nodes. Next, we compute $\botjoin$ for other nodes in a post-order traversal of the tree with this iterative formula:
\begin{align*}
\bot(v_j) = \groupbyagg{A_{v_i,p(v_i)}} (\superjoinagg(v_j, \{\bot(v_{j'})|  v_{j'}\in C(v_j) \}))
%\botjoin(v_i) =~&  \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
% &v_i \superjoin (\underset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))
\end{align*}
For each $\botjoin(v_j)$, the join starts with $v_j$ and follows by the children of $v_j$ one by one.  
%use $v_i$ to join $\botjoin(v_j)$ $\forall v_j \in C(v_i)$ one by one. %\note{It is clearer in the algorithm box}


\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in C(v_i)$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows, and proving by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}}

To prepare $\top(v_j)$, we start with the root node. Next, we compute $\topjoin$ for other nodes in a pre-order traversal of the tree with this iterative formula:
\begin{align*}
\top(v_j) = \groupbyagg{A_{v_i,p(v_i)}}(
\superjoinagg(p(v_j), \top(p(v_j)), \{\bot(v_{j'}) | v_{j'}\in N(v_j)  \}))
%\topjoin(v_i) =~& \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
%&p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)
\end{align*}
For each $\top(v_j)$, the join starts with $p(v_j)$ and $\top(p(v_j))$ and follows by the botjoin of the neighbors of $v_j$ one by one. 
%The join order is as follows: use $p(v_j)$ to join $\topjoin(p(v_j))$ and $\botjoin(v_j) ~ \forall v_{j'} \in N(v_j)$ one by one.

\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in N(v_i)$ by the definition of botjoin as equation (\ref{eq:gj_botjoin}) shows, and replacing $\topjoin(p(v_i))$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows. Finally, prove it by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}
}
 
After preparing all the topjoins and botjoins, we combine these results to obtain the frequency tables $T^i$  for $i=1,\ldots,m$ based on Equations~\eqref{eq:gj_fast_node_freq} and~\eqref{eq:gj_fast_freq}. Notice that when computing $T^{v_j}$, we drop topjoins for root node and we drop botjoins for leaf nodes; and when computing  $T^{i}$, we drop $H(R_i)$ if $\R{i}$ is the only relation within the node. 
We iterate all the frequency tables $T_i$ and find the tuple with maximum $\cnt$. This tuple is returned as the most sensitive tuple with its $\cnt$ as the local sensitivity of this query on the given database instance.

%Though there exists efficient ways to compute these joins, we leave the analysis of the tightest parameterized complexity for these equations as future work. In this work, we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order.  
 
 
 \eat{
 and find the most sensitive tuple, for each relation $\R{i}$, we need to construct $\Qgfreq^i(\attributes_\database)$ according to equation (\ref{eq:gj_fast_node_freq}) and (\ref{eq:gj_fast_freq}). These equations include joins among $\topjoin(v_j)$, $\botjoin(v_{j'}) ~ \forall v_{j'} \in C(v_j)$ and $\forall \R{i'} \in H(\R{i})$. Although there exists efficient ways to compute these joins, we postpone this to the future work and leave this as an open problem to analyze the tightest parameterized complexity for these equations. Here we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order. }  

\eat{\note{New rule. We need to avoid cross product. This matches the rule in path join.} For the last step, instead of computing $\Qgfreq^i(\attributes_\database)$ with all joins together, we divide joins into several join groups and get disjoint join results in aspect to attributes. Any two join groups share no common attributes from relations inside the group. We later merge them back by choosing max from each cluster. 
\note{Double Hypertree Width} Within each join group, we arrange the join order according to the hypertree decomposition of relations within the group. Denote double hypertree width as the max hypertree width within each join group.}

Instead of computing $T^i$ with merge-sort joins one by one in an arbitrary order, we partition the joins into groups such that relations from different groups share no common attributes. We find the most sensitive tuple per join group. Within each join group, we arrange the join order according to the hpyertree decomposition of relations within the group. We denote the maximum hypertree width within each join group as \emph{double hypertree width} for relation $\R{i}$. Double hypertree width for the enitre query is defined as the max double hypertree width from each $\R{i}$.

\begin{theorem}
	Algorithm~\ref{algo:gj_query} computes the local sensitivity of a general join query and also finds the corresponding most sensitive tuple. Given $m$ tables with size $n$ and $\leq k$ attributes for each, and a hypertree decomposition of the  general join query with hypertree width $p$ and double hypertree width as $q$ and $m' \leq m$ nodes, the time complexity is $O(m p q  \log n \cdot n^{pq} )$ .
\end{theorem}

\begin{proof} Computing the joins within a node has a complexity of $O(\sum_{i=2}^{p}{n^i})$. Given $m'<m$ number of nodes, the first step has an $O(m'n^p)$ complexity.
%	$O(m'n^p)$ for computing joins within a node  * m nodes (consider $O(\sum_{i=2}^{p}{n^i})$ for a single node).

The time to compute the topjoins and botjoins for $m'$ nodes is $O(m'n^p \log n^p)$ as the size of a node is at most $O(n^p)$).
%for computing top/bot joins for $m'$ nodes (the size of a node is at most $O(n^p)$).

Finally, to compute $T^i$ for $m$ relations, the time complexity is 
$O(mn^{pq} \log n^{pq})$.% for computing $T^i$ for $m$ relations.

Hence, the total time complexity is $O(mn^{pq} \log n^{pq})$ or $O(m p q  \log n \cdot n^{pq} )$. 
\end{proof}

\subsection{Extensions}\label{sec:extensions}
\textbf{Extension to selection and projection.~} 

Although by default each relation appears in the query body is the original base table, with extra rules, the algorithm can support using a table after selection and projection of its base table for the query body. For each tuple: 1) the tuple sensitivity is not affected by projection since we assume projection keeps duplicates. 2) if the tuple doesn't match the predication of its table's selection, we set the tuple sensitivity as 0, since it is dropped by selection before it can join other tuples. Applying rules 1 and 2 will not affect the complexity.

\textbf{Extension to disjoint query components.~} 

If the hypergraph of query is not connected, we get a hyperforest containing multiple disjoint hypertrees instead of a single hypertree for a query. In this case, we run our algorithm for each hypertree. We then update the tuple sensitivity by multiplying it with the join size of other hypertrees. The join size of each hypertree can be computed as the sum of frequency from the botjoin of each hypertree root, so it will not affect the complexity. 

\textbf{Extension to attributes appearing in only one relation.~}

%\sr{for attributes in one relation, please complete}  
If an attribute  $A$ appears in only one relation $R_i$,  and the relation is connected with other relations by other attributes, $A$ does not affect the local sensitivity, but  the  tuple $t$ with  the maximum tuple sensitivity may be from $R_i$, so  we  would  need  a value of $t.A$. Similar to Algorithm~\ref{algo:ls_pathquery}, if the  other  attributes in $R_i$ except $A$ come from an  existing  tuple $t'$  in  the  instance, we augment 
it with $t'.A$ (for downward sensitivity). If there are no such tuples $t'$, we choose any value from the active domain of $A$ to extend the other attributes to form such a tuple $t$ (for upward sensitivity). 

\input{double_acyclic_join}

==> generaljoin-EXTENSION-details.tex <==
\section{General Join Query}\label{sec:general}
 
\begin{algorithm}[t]
	\small
	\caption{Compute Local Sensitivity of a General Join Query and the corresponding Most Sensitive Tuple} 
	\label{algo:gj_query}
	\begin{algorithmic}[1]
		\Require General join query $\Qgjoin(\attributes_\database)$
		%$\Qgjoin(\attr_0 \ldots \attr_m)$, 
		the database $\database$
		\Ensure $\LS(Q,D)$, and the most sensitive tuple $\kingtuple$
		\Procedure {LS}{$\Qgjoin, \database$}
		\Statex I) Prepare nodes
		\For{all nodes $v_j\in V$}
		    %\State $v_j = \underset{\forall \R{i} \in v_j }{\superjoin} \R{i}$
		    \State $v_j = \superjoin(\{\R{i} \in v_j\})$
		\EndFor
		\Statex II) Prepare botjoin
		\For{$j$ in postoder}
		\If{$v_j$ is a leaf}
		\State $\botjoin(v_i) = \groupbyagg{\attributes_{v_j,p(v_j)}}(v_j) $
		%\aggregate{\attributes_{v_i,p(v_i)}}{count(*) \as \cntt{v_i}{p(v_i)}}{v_i}$
		%\ElsIf {$v_i$ is the root}
		%\State pass
		\ElsIf{$v_j$ is not the root}
		\State $\botjoin(v_j) =  \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin (v_j, \{\botjoin(v_{j'})~|~v_{j'}\in C(v_j)\})$ 
		%(\und%erset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))$
		%\State $\botjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\EndIf
		\EndFor
		\Statex III) Prepare topjoin
		\For{$j$ in preoder}
		%\If{$v_j$ is the root}
		%\State pass
		\If {$p(v_j)$ is the root}
		%\ElsIf {$p(v_i)$ is the root}
		%\State  $S =
	    %p(v_i) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j), \{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \}) $
		\ElsIf{$v_j$ is not root}
		%\State  $S =
		%p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S $
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j),\topjoin(v_j),\{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \})$
		\EndIf
		\EndFor
		\Statex IV) Prepare frequency tables of nodes
		\For{$j=1, \dots, m'$}
		\If {$v_j$ is the root}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%\aggregate{\attributes_{v_i}}{sum(\underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{} \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j)$		
		\ElsIf {$v_j$ is a leaf}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}} (\topjoin{v_j})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)}) \as  c}{} \topjoin(v_i)$
		\Else 
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\topjoin{(v_j)},\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)} \underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{	\topjoin(v_i) \superjoin ( \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j))}$
		\EndIf
		\EndFor

		\Statex V) Select  the most sensitive tuple
		\For{$i=1, \ldots, m$}
		%\note{Improve the efficiency later}
		\State $T^i = \groupbyagg{\attributes_i}\superjoin(T^{\pi(R_i)}, H(R_i))$
		%$\Qgfreq^i =  \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}	\Qgfreq^{\pi(v_i)} \superjoin 		\underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}		$
		\EndFor
		\State $t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt$
		%\Statex VI) Select most sensitive tuple
		%\For{$i=1, \ldots, m$}
		%\State $t_i = \argmax_{\tsens} \pi_{\tsens_i \as \tsens} \Qgfreq^i$
		%\EndFor 
		%\State $t = \argmax_{\tsens}{t_1, \ldots, t_m}$
		%\State $\LS = t.\tsens$
		\State $\LS = t^*.\cnt$ 
		\State \textbf{return} $\LS, t^*$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}



Path join queries only cover a small subset of all conjunctive queries. In this section, we discuss the general solution to general conjunctive queries (Section~\ref{sec:general-approach}), and then present an efficient algorithm with additional parameters in the running time complexity of the algorithm (Section~\ref{sec:general-algo}). Finally, we  discuss a class of queries that  we call \emph{doubly-acyclic queries} generalizing path  queries where these parameters are gone. 

We assume that there are no self joins in the queries; i.e., there are no duplicated relations in the query body. For simplicity, we assume that the CQ is a full CQ of the following form: 
\begin{align*}
\Qgjoin(\attributes_\database) :- \relation_1(\attributes_1), \ldots, \relation_m(\attributes_m), 
\end{align*}
%where $\attributes_i$ is the attribute set of the table $\relation_i$.
%, which at most has $k$ attributes.
%We also call attributes as variables and relations as atoms. 
We assume that the query hypergraph (Section~\ref{sec:acyclic}) is connected. We also assume each attribute appears in at least two relations in the body. We also assume that there are no selections in the body, and no projections in the head of the query, i.e., $\attributes_\database = \cup_{i=1}^m \attributes_i$, and the total number of attributes $|\attributes_\database|$ is $k$. These assumptions, except the no-self-join assumption (which introduces new challenges and we leave it as a future direction), are without loss of generality as how they can be relaxed using our algorithm is discussed in Section~\ref{sec:extensions}. 

\subsection{Basic Idea and Query Hypertrees}\label{sec:general-approach}
To compute the local sensitivity of a general CQ, the basic idea is similar to that in the path join case. 

\begin{itemize}
    \item[(i)] For each $i=1,\ldots,m$, compute
%For general join queries, we define $\Qgjoin^i(\attributes_\database)$ as:
\begin{align}\label{eq:general_gj_sub_query}
S^i = \superjoin(R_1,\ldots,R_{i-1}, R_{i+1},\ldots, R_m)
%\Qgjoin^i(\attributes_\database) \datalogEQ
%& \relation_1(\attributes_1), \ldots, \relation_{i-1}(\attributes_{i-1}), \nonumber \\
%& \relation_{i+1}(\attributes_{i+1}), \ldots, \relation_m(\attributes_m) 
\end{align}
%which is a sub-query from the original join query by removing the relation $\relation_i$. 
\item[(ii)] For each $i=1,\ldots, m$, compute 
%Then we do a counting group by on attributes $\attributes_i$.
\begin{align}\label{eq:general_gj_freq}
%\Qgfreq^i(\attributes_\database) = 
T^i = \groupbyagg{\attributes_i}(S^i)
%{\aggregate{\attributes_i}{count(*) \as c}{\Qgjoin^i(\attributes_\database)}}
\end{align}
%to count the frequency of each tuple.

\item[(iii)] Finally, return the most sensitive tuple:
%To find the most sensitive tuple, we pick the tuple from the above query who has the largest frequency $c$.
\begin{align} \label{eq:general_gj_most_sensitive_tuple}
%t^*_i = \argmax_{c} \Qgfreq^i(\attributes_\database)
t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt
\end{align}
\end{itemize}

\cut{
\begin{proposition}
The tuple $t^*$ returned by Equation~\eqref{eq:general_gj_most_sensitive_tuple} gives the most sensitive tuple with its sensitivity $t^*.\cnt$.
%as $t^*.\attributes$ and its tuple frequency $t^*.\cnt$ from the domain of table $\relation_i$.
\end{proposition}
\begin{proof}
	By definition, Equation~\eqref{eq:general_gj_freq} computes and stores the tuple sensitivity as $\cnt$ for each $\attributes_i$ appears in $S^i$. $S^i$ covers the \representative domain of $\attributes_i$ by the construction rule. 
    Since all tuples outside this \representative domain has sensitivity 0, searching tuples within this domain can guarantee finding the most sensitive tuple and its corresponding sensitivity. 
\end{proof}

Although this approach gives us the correct result, the size of the sub-query $S^i$ in worst case could be $\Omega(n^{m-1})$.
The size of $T^i$ in worst case could be $\Omega(n^k)$.
In conclusion, this naive approach is polynomial in data complexity, but may be exponential in combined complexity.
}

Once again, the size of the sub-queries $S^i$ can be exponential in $m$ or $k$, which is polynomial in data complexity, but may not be efficient for practical purposes. 
To design an efficient algorithm for general CQs, we use \emph{hypertree decompositions} of the query \cite{Gottlob+1999, Abiteboul+1995}, which we briefly review below\footnote{There are multiple other equivalent notion of decompositions and width of general CQs, like \emph{generalized hypertree width, tree width, query width}, or \emph{fractional hypertree width} \cite{Chekuri:1997, Grohe:2001, Gottlob:2016}. Having a bound on these widths leads to polynomial time evaluation  for general CQs. We choose hypertree width as we needed that each relation in the query appears in only one node in the hypertree decomposition}. 

\stitle{Hypertree Decomposition.}
A hypertree $\tree_Q$ associated with a conjunctive query $Q$ is a tree with nodes labeled with attributes of the query $Q$ such that (1) each node in the  tree contains one or multiple relational atoms and all their attributes, 
%each node contains one or multiple relational atoms, 
and (2) for each attribute $A$, the nodes in 
$\tree_Q$ containing the same attribute forms a sub-tree. It can be seen that when each node in $\tree_Q$ contains a single relation, it is a \emph{join-tree} of $Q$ (Section~\ref{sec:acyclic}). 
%and 3) each relation from the query appears once and only once in the hypertree. The max number of relations within a node is defined as hypertree width. 

Each query has an associated hypertree, and it can be found in polynomial time if its \emph{hypertree-width},  is bounded. Given a hypertree of width $p$ for the input query, we represent this hypertree by 
a join tree $\tree(V,E, \map)$, where $V=\{v_1,\ldots,v_{|V|}\}$, $E=\{e_1,\ldots,e_{|E|}\}$ and $\map$ maps a relation $\R{i}$ to a node $v_j$ and each edge contains the common attributes between two nodes.
%%%Mapping of relations to nodes 
The number of nodes is less than the number of relations ($|V|<m$)
since multiple relations could be merged into one node. If $\R{i}$ is contained in $v_j$, then $\pi(\R{i}) = v_j$. 
%%use i for index of relations
%%use j for index of nodes
%%%Mapping of attributes to edges
We denote the union set of attributes from all relations in $v_j$ as $\attributes_{v_j}$, and the set of join attributes between $v_{j_1}$ and $v_{j_2}$ by $\attributes_{v_{j_1},v_{j_2}}$.
%%%Other notations
Let $p(v_j)$ denote the parent of node $v_j$ in the join tree,
$C(v_j)$ denote the child nodes of $v_j$,
and $N(v_j)$ denote the neighbors of $v_j$, i.e. $C(p(v_j)) \setminus \{v_j\}$. Within a node $\pi(\R{i})$, let $H(\R{i})$ denotes the group of cohorts of $\R{i}$, i.e. $\{\R{i'} \mid \R{i'} \in \pi(\R{i'}), \R{i'} \neq \R{i}\}$.
%; let $A(\R{i})$ denotes the attributes set between $\R{i}$ and $H(\R{i})$, i.e. $\cup_{\R{j} \in H(\R{i})} \attributes_{i, j}$
We denote $\subtree(v_j)$ as the subtree rooted at $v_j$, while $\comptree(v_j)$ is the complementary graph of $\subtree(v_j)$ on the tree $\tree(V, E, \pi)$.
%%%Property of a hypertree decomposition 
Since it's a hypertree decomposition, for each attribute, the nodes that contain this attribute always form a subtree. 
\subsection{Algorithm Details}\label{sec:general-algo}

%\todo{Add an introduction to the hypertree decomposition}. 
We present an algorithm based on a hypertree decomposition of a general join query. 



%\xh{We can add a definition box for this property if it's used later.}\yc{It should be used in efficiency analysis}


\stitle{Definitions.} For each relation $R_i$, let $v_j=\pi(R_i)$, the frequency table (Equation~\eqref{eq:general_gj_freq}) can be computed from the join of three groups of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$. In order to compute $T^i$, we define \emph{topjoin} and $\emph{botjoin}$ for each node $v_j$ in the hypertree:
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\tree(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}
Similar to the frequency table for a relation (Equation~\eqref{eq:general_gj_freq}), we define the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
T^{v_j}=  
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}
For $v_j$ as root or leaf, it has a simpler formula and we will discuss it in the algorithm.
Then the frequency table for a relation can be expressed using the frequency table of its node $\pi(R_i)$ and the cohorts of $R_i$ in $\pi(R_i)$: 
\begin{align}\label{eq:gj_fast_freq}
T^i= \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(T^{\pi(R_i)}), H(\R{i})))
\end{align}
x
%We use $\superjoin(R_1, R_2,\ldots, R_i)$ to denote the natural join between the relations $R_1,\ldots, R_i$. 

%Similar to Equation~\eqref{eq:general_gj_sub_query}, we capture the join result without the node $v_j$ in a hypertree $T$ as:
%\begin{align}\label{eq:gj_fast_node_sub_query}
%\Qgjoin^{v_j}(\attributes_\database) =
%\superjoin(\comptree(v_j), \{T(v_{j'})~|~v_{j'}\in C(v_j) \})
%\end{align}
%which is a natural join between the complementary tree of $v_j$ and the subtrees at the children of $v_j$. 



%\begin{align}\label{eq:gj_fast_node_sub_query}\Qgjoin^{v_i}(\attributes_\database) = \comptree(v_i) \superjoin \underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j)\end{align}
%\xh{This expression in \eqref{eq:gj_fast_node_sub_query} is not clear. what do you try to join here? } \yc{The symbol $\superjoin$ actually is a natural join and it reduces to cross product if there is no common attributes. Here, I want to join every nodes except $v_i$, so we need to join each child's subtree as $\underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j) = \subtree(v_{j_1})  \superjoin \subtree(v_{j_2})  \ldots \superjoin \subtree(v_{j_p}) $ and the complementary tree $\comptree(v_i)$.} 

\eat{
Now we can rewrite the Equation~\eqref{eq:general_gj_sub_query} in step (1) as \begin{align}\label{eq:gj_fast_sub_query}
\Qgjoin^i(\attributes_\database) 
=\superjoin(\Qgjoin^{\pi(R_i)}(\attributes_\database) , H(R_i))
\end{align}
Let $v_i$ be the corresponding node of $R_i$ in the hypertree, i.e., $v_j=\pi(R_i)$. This expression joins three types of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$.
}
%\begin{align}\label{eq:gj_fast_sub_query} \Qgjoin^i(\attributes_\database) = \Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin \underset{\forall \R{j} \in H(R_i)}{\superjoin} \R{j}\end{align}

\begin{figure}
	\centering
	\includegraphics[scale=0.45]{acyclic_join_recursion.pdf}
	\caption{Example of notations. \todo{Update the figure and description} \note{edit \href{https://docs.google.com/drawings/d/1xTBbD3DY4HEqO5I21m1UiGcjLAM9rrvS0YnmI5qm_J0/edit?usp=sharing}{here} }}
	\label{fig:gj_notations}
\end{figure}

\eat{
Given a table $R_i$ in $T$, as long as we know the maximum frequency of tuples projected on $\attributes_i$ from the joint output between tables other than $R_i$ in a join tree of $\Qgjoin$, as defined by $\Qgjoin^i$, we immediately get the max change to the final joint output due to adding or removing a tuple to $R_i$, and hence the local sensitivity of the query. We define the following invariants to compute the tuple sensitivity of a general query.
}

%\xh{May use this notation earlier}. 
%First, we assume all the relations has additional attribute $C$ to record the multiplicity of the other attribute values. For the base tables, we add attribute $c$ and assign $1$ to this attribute for every tuple. We also use $\superjoinagg(R_1,\ldots,R_i)$ to summarize two steps: (i) a natural join among $R_1, R_2,\ldots, R_i$ except the attribute $c$, and (ii) project the product of these multiplicity attributes to a new multiplicity column, i.e., $$\superjoinagg(R_1,\ldots,R_i)= \pi_{(R_1.C\times \cdots R_i.C)\rightarrow C} (\superjoin(R_1,\ldots, R_i)).$$
%Let $\groupbyagg{A}(R_i)$ represent a group by attribute $A$ and sum the counts and rename the sum as a new attribute $c$, i.e., 
%$$\groupbyagg{A}(R_i)= \aggregate{A}{sum(C) \rightarrow C}{(R_i)}.$$

\eat{
For each node $v_j$, we denote $\botjoin(v_j)$ and $\topjoin(v_j)$ as tables that computes the frequency of tuples projected on attributes shared by $v_j$ and its parent $p(v_j)$ from $\subtree(v_j)$ and $\comptree(v_j)$.
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (T(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}


Denote the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
\Qgfreq^{v_j}(\attributes_\database) =  
%\aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big) 
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}

%\begin{align}\label{eq:gj_fast_node_freq}
%\Qgfreq^{v_i} =  \aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big)
%\end{align}

Now, equation (\ref{eq:general_gj_freq}) can be rewritten as:
\begin{align}\label{eq:gj_fast_freq}
\Qgfreq^i(\attributes_\database) = \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(\Qgfreq^{\pi(R_i)}), H(\R{i}))
%	(\aggregate{\attributes_i}{sum(c) \as c}{\Qgfreq^{\pi(R_i)}}) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
)
\end{align}


\begin{lemma}
	Equation (\ref{eq:general_gj_freq}) and (\ref{eq:gj_fast_freq}) for step (2) are equivalent.
\end{lemma}
\begin{proof}
    
\end{proof}
}

%\begin{proof} 
%	Replacing $\Qgjoin^i(\attributes_\database)$ by equation (\ref{eq:gj_fast_node_sub_query}) and 
%	(\ref{eq:gj_fast_sub_query}), equation (\ref{eq:general_gj_freq}) can be rewritten as
%	\begin{align*}
%	  \Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	  	\Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	  \Qgjoin^{\pi(\R{i})}(\attributes_\database) =~&
%	  	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	which is equivalent to
%	\begin{align*}
%	\Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}
%	R~ \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	R =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	Notice that the intermediate relation $R$ is equivalent to equation (\ref{eq:gj_fast_node_freq}), so 
%	$\Qgfreq^i(\attributes_\database)$ can be rewritten as
%	\begin{align*}
%	\Qgfreq^i =~ \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}\Qgfreq^{v_i} \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
%	\end{align*}
%	, which is equivalent to equation (\ref{eq:gj_fast_freq})
%\end{proof}
%The last step is the same.

\paratitle{Algorithm.} The algorithm first prepares each tree node $v_j$ as the join among tables in $v_j$. Then it prepares $\bot(v_j)$ and $\top(v_j)$ for each node, and use them to compute $T^{v_j}$ for each node $v_j$. Finally, it computes $T^{i}$ for each relation $\R{i}$ and finds the most sensitive tuple and its tuple sensitivity. 

Note that computing  botjoin $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}) and topjoin $\top(v_j)$ (Equation~\eqref{eq:gj_topjoin}) for each node again may require exponential combined complexity, so we give an iterative approach in Algorithm~\ref{algo:gj_query} to compute them in polynomial combined complexity. After preparing botjoin and topjoin for each node, the third step is to combine them together and find the most sensitive tuple. We assume all joins are merge-sort joins.


\note{Illustrate the recursive structure of topjoin and botjoin by figure (\ref{fig:gj_notations}).}


To prepare each node $v_j$, we compute the join between 
%joins as $v_j = \underset{\forall \R{j} \in v_i }{\superjoin} \R{j}$ 
the relations in $v_j$ in an arbitrary join order.

To prepare $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}), we start from the leaf nodes. Next, we compute $\botjoin$ for other nodes in a post-order traversal of the tree with this iterative formula:
\begin{align*}
\bot(v_j) = \groupbyagg{A_{v_i,p(v_i)}} (\superjoinagg(v_j, \{\bot(v_{j'})|  v_{j'}\in C(v_j) \}))
%\botjoin(v_i) =~&  \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
% &v_i \superjoin (\underset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))
\end{align*}
For each $\botjoin(v_j)$, the join starts with $v_j$ and follows by the children of $v_j$ one by one.  
%use $v_i$ to join $\botjoin(v_j)$ $\forall v_j \in C(v_i)$ one by one. %\note{It is clearer in the algorithm box}


\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in C(v_i)$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows, and proving by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}}

To prepare $\top(v_j)$, we start with the root node. Next, we compute $\topjoin$ for other nodes in a pre-order traversal of the tree with this iterative formula:
\begin{align*}
\top(v_j) = \groupbyagg{A_{v_i,p(v_i)}}(
\superjoinagg(p(v_j), \top(p(v_j)), \{\bot(v_{j'}) | v_{j'}\in N(v_j)  \}))
%\topjoin(v_i) =~& \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
%&p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)
\end{align*}
For each $\top(v_j)$, the join starts with $p(v_j)$ and $\top(p(v_j))$ and follows by the botjoin of the neighbors of $v_j$ one by one. 
%The join order is as follows: use $p(v_j)$ to join $\topjoin(p(v_j))$ and $\botjoin(v_j) ~ \forall v_{j'} \in N(v_j)$ one by one.

\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in N(v_i)$ by the definition of botjoin as equation (\ref{eq:gj_botjoin}) shows, and replacing $\topjoin(p(v_i))$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows. Finally, prove it by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}
}
 
After preparing all the topjoins and botjoins, we combine these results to obtain the frequency tables $T^i$  for $i=1,\ldots,m$ based on Equations~\eqref{eq:gj_fast_node_freq} and~\eqref{eq:gj_fast_freq}. Notice that when computing $T^{v_j}$, we drop topjoins for root node and we drop botjoins for leaf nodes; and when computing  $T^{i}$, we drop $H(R_i)$ if $\R{i}$ is the only relation within the node. 
We iterate all the frequency tables $T_i$ and find the tuple with maximum $\cnt$. This tuple is returned as the most sensitive tuple with its $\cnt$ as the local sensitivity of this query on the given database instance.

%Though there exists efficient ways to compute these joins, we leave the analysis of the tightest parameterized complexity for these equations as future work. In this work, we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order.  
 
 
 \eat{
 and find the most sensitive tuple, for each relation $\R{i}$, we need to construct $\Qgfreq^i(\attributes_\database)$ according to equation (\ref{eq:gj_fast_node_freq}) and (\ref{eq:gj_fast_freq}). These equations include joins among $\topjoin(v_j)$, $\botjoin(v_{j'}) ~ \forall v_{j'} \in C(v_j)$ and $\forall \R{i'} \in H(\R{i})$. Although there exists efficient ways to compute these joins, we postpone this to the future work and leave this as an open problem to analyze the tightest parameterized complexity for these equations. Here we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order. }  

\eat{\note{New rule. We need to avoid cross product. This matches the rule in path join.} For the last step, instead of computing $\Qgfreq^i(\attributes_\database)$ with all joins together, we divide joins into several join groups and get disjoint join results in aspect to attributes. Any two join groups share no common attributes from relations inside the group. We later merge them back by choosing max from each cluster. 
\note{Double Hypertree Width} Within each join group, we arrange the join order according to the hypertree decomposition of relations within the group. Denote double hypertree width as the max hypertree width within each join group.}

Instead of computing $T^i$ with merge-sort joins one by one in an arbitrary order, we partition the joins into groups such that relations from different groups share no common attributes. We find the most sensitive tuple per join group. Within each join group, we arrange the join order according to the hpyertree decomposition of relations within the group. We denote the maximum hypertree width within each join group as \emph{double hypertree width} for relation $\R{i}$. Double hypertree width for the enitre query is defined as the max double hypertree width from each $\R{i}$.

\begin{theorem}
	Algorithm~\ref{algo:gj_query} computes the local sensitivity of a general join query and also finds the corresponding most sensitive tuple. Given $m$ tables with size $n$ and $\leq k$ attributes for each, and a hypertree decomposition of the  general join query with hypertree width $p$ and double hypertree width as $q$ and $m' \leq m$ nodes, the time complexity is $O(m p q  \log n \cdot n^{pq} )$ .
\end{theorem}

\begin{proof} Computing the joins within a node has a complexity of $O(\sum_{i=2}^{p}{n^i})$. Given $m'<m$ number of nodes, the first step has an $O(m'n^p)$ complexity.
%	$O(m'n^p)$ for computing joins within a node  * m nodes (consider $O(\sum_{i=2}^{p}{n^i})$ for a single node).

The time to compute the topjoins and botjoins for $m'$ nodes is $O(m'n^p \log n^p)$ as the size of a node is at most $O(n^p)$).
%for computing top/bot joins for $m'$ nodes (the size of a node is at most $O(n^p)$).

Finally, to compute $T^i$ for $m$ relations, the time complexity is 
$O(mn^{pq} \log n^{pq})$.% for computing $T^i$ for $m$ relations.

Hence, the total time complexity is $O(mn^{pq} \log n^{pq})$ or $O(m p q  \log n \cdot n^{pq} )$. 
\end{proof}

\subsection{Extensions}\label{sec:extensions}
\textbf{Extension to selection and projection.~} 

Although by default each relation appears in the query body is the original base table, with extra rules, the algorithm can support using a table after selection and projection of its base table for the query body. For each tuple: 1) the tuple sensitivity is not affected by projection since we assume projection keeps duplicates. 2) if the tuple doesn't match the predication of its table's selection, we set the tuple sensitivity as 0, since it is dropped by selection before it can join other tuples. Applying rules 1 and 2 will not affect the complexity.

\textbf{Extension to disjoint query components.~} 

If the hypergraph of query is not connected, we get a hyperforest containing multiple disjoint hypertrees instead of a single hypertree for a query. In this case, we run our algorithm for each hypertree. We then update the tuple sensitivity by multiplying it with the join size of other hypertrees. The join size of each hypertree can be computed as the sum of frequency from the botjoin of each hypertree root, so it will not affect the complexity. 

\textbf{Extension to attributes appearing in only one relation.~}

%\sr{for attributes in one relation, please complete}  
If an attribute  $A$ appears in only one relation $R_i$,  and the relation is connected with other relations by other attributes, $A$ does not affect the local sensitivity, but  the  tuple $t$ with  the maximum tuple sensitivity may be from $R_i$, so  we  would  need  a value of $t.A$. Similar to Algorithm~\ref{algo:ls_pathquery}, if the  other  attributes in $R_i$ except $A$ come from an  existing  tuple $t'$  in  the  instance, we augment 
it with $t'.A$ (for downward sensitivity). If there are no such tuples $t'$, we choose any value from the active domain of $A$ to extend the other attributes to form such a tuple $t$ (for upward sensitivity). 

\input{double_acyclic_join}

==> generaljoin.tex <==
\section{General Join Query}\label{sec:general}
 
\begin{algorithm}[t]
	\small
	\caption{Compute Local Sensitivity of a General Join Query and the corresponding Most Sensitive Tuple} 
	\label{algo:gj_query}
	\begin{algorithmic}[1]
		\Require General join query $\Qgjoin(\attributes_\database)$
		%$\Qgjoin(\attr_0 \ldots \attr_m)$, 
		the database $\database$
		\Ensure $\LS(Q,D)$, and the most sensitive tuple $\kingtuple$
		\Procedure {LS}{$\Qgjoin, \database$}
		\Statex I) Prepare nodes
		\For{all nodes $v_j\in V$}
		    %\State $v_j = \underset{\forall \R{i} \in v_j }{\superjoin} \R{i}$
		    \State $v_j = \superjoin(\{\R{i} \in v_j\})$
		\EndFor
		\Statex II) Prepare botjoin
		\For{$j$ in postoder}
		\If{$v_j$ is a leaf}
		\State $\botjoin(v_i) = \groupbyagg{\attributes_{v_j,p(v_j)}}(v_j) $
		%\aggregate{\attributes_{v_i,p(v_i)}}{count(*) \as \cntt{v_i}{p(v_i)}}{v_i}$
		%\ElsIf {$v_i$ is the root}
		%\State pass
		\ElsIf{$v_j$ is not the root}
		\State $\botjoin(v_j) =  \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin (v_j, \{\botjoin(v_{j'})~|~v_{j'}\in C(v_j)\})$ 
		%(\und%erset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))$
		%\State $\botjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\EndIf
		\EndFor
		\Statex III) Prepare topjoin
		\For{$j$ in preoder}
		%\If{$v_j$ is the root}
		%\State pass
		\If {$p(v_j)$ is the root}
		%\ElsIf {$p(v_i)$ is the root}
		%\State  $S =
	    %p(v_i) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S$
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j), \{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \}) $
		\ElsIf{$v_j$ is not root}
		%\State  $S =
		%p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)$
		%\State $\topjoin(v_i) = \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} S $
		\State $\topjoin(v_j) = \groupbyagg{\attributes_{v_j,p(v_j)}} \superjoin(p(v_j),\topjoin(v_j),\{\botjoin(v_{j'})~|~v_{j'}\in N(v_j) \})$
		\EndIf
		\EndFor
		\Statex IV) Prepare frequency tables of nodes
		\For{$j=1, \dots, m'$}
		\If {$v_j$ is the root}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%\aggregate{\attributes_{v_i}}{sum(\underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{} \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j)$		
		\ElsIf {$v_j$ is a leaf}
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}} (\topjoin{v_j})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)}) \as  c}{} \topjoin(v_i)$
		\Else 
		\State $T^{v_j} = \groupbyagg{\attributes_{v_j}}\superjoin(\topjoin{(v_j)},\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \})$
		%$\Qgfreq^{v_i} = \aggregate{\attributes_{v_i}}{sum(\cntt{i}{p(i)} \underset{j \in C(i)}{\product} \cntt{i}{j}) \as  c}{	\topjoin(v_i) \superjoin ( \underset{\forall j \in C(i)}{\superjoin} \botjoin(v_j))}$
		\EndIf
		\EndFor

		\Statex V) Select  the most sensitive tuple
		\For{$i=1, \ldots, m$}
		%\note{Improve the efficiency later}
		\State $T^i = \groupbyagg{\attributes_i}\superjoin(T^{\pi(R_i)}, H(R_i))$
		%$\Qgfreq^i =  \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}	\Qgfreq^{\pi(v_i)} \superjoin 		\underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}		$
		\EndFor
		\State $t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt$
		%\Statex VI) Select most sensitive tuple
		%\For{$i=1, \ldots, m$}
		%\State $t_i = \argmax_{\tsens} \pi_{\tsens_i \as \tsens} \Qgfreq^i$
		%\EndFor 
		%\State $t = \argmax_{\tsens}{t_1, \ldots, t_m}$
		%\State $\LS = t.\tsens$
		\State $\LS = t^*.\cnt$ 
		\State \textbf{return} $\LS, t^*$
		\EndProcedure
	\end{algorithmic}
\end{algorithm}



Path join queries only cover a small subset of all conjunctive queries. In this section, we discuss the general solution to general conjunctive queries (Section~\ref{sec:general-approach}), and then present an efficient algorithm with additional parameters in the running time complexity of the algorithm (Section~\ref{sec:general-algo}). Finally, we  discuss a class of queries that  we call \emph{doubly-acyclic queries} generalizing path  queries where these parameters are gone. 

We assume that there are no self joins in the queries; i.e., there are no duplicated relations in the query body. For simplicity, we assume that the CQ is a full CQ of the following form: 
\begin{align*}
\Qgjoin(\attributes_\database) :- \relation_1(\attributes_1), \ldots, \relation_m(\attributes_m), 
\end{align*}
%where $\attributes_i$ is the attribute set of the table $\relation_i$.
%, which at most has $k$ attributes.
%We also call attributes as variables and relations as atoms. 
We assume that the query hypergraph (Section~\ref{sec:acyclic}) is connected. We also assume each attribute appears in at least two relations in the body. We also assume that there are no selections in the body, and no projections in the head of the query, i.e., $\attributes_\database = \cup_{i=1}^m \attributes_i$, and the total number of attributes $|\attributes_\database|$ is $k$. These assumptions, except the no-self-join assumption (which introduces new challenges and we leave it as a future direction), are without loss of generality as how they can be relaxed using our algorithm is discussed in Section~\ref{sec:extensions}. 

\subsection{Basic Idea and Query Hypertrees}\label{sec:general-approach}
To compute the local sensitivity of a general CQ, the basic idea is similar to that in the path join case. 

\begin{itemize}
    \item[(i)] For each $i=1,\ldots,m$, compute
%For general join queries, we define $\Qgjoin^i(\attributes_\database)$ as:
\begin{align}\label{eq:general_gj_sub_query}
S^i = \superjoin(R_1,\ldots,R_{i-1}, R_{i+1},\ldots, R_m)
%\Qgjoin^i(\attributes_\database) \datalogEQ
%& \relation_1(\attributes_1), \ldots, \relation_{i-1}(\attributes_{i-1}), \nonumber \\
%& \relation_{i+1}(\attributes_{i+1}), \ldots, \relation_m(\attributes_m) 
\end{align}
%which is a sub-query from the original join query by removing the relation $\relation_i$. 
\item[(ii)] For each $i=1,\ldots, m$, compute 
%Then we do a counting group by on attributes $\attributes_i$.
\begin{align}\label{eq:general_gj_freq}
%\Qgfreq^i(\attributes_\database) = 
T^i = \groupbyagg{\attributes_i}(S^i)
%{\aggregate{\attributes_i}{count(*) \as c}{\Qgjoin^i(\attributes_\database)}}
\end{align}
%to count the frequency of each tuple.

\item[(iii)] Finally, return the most sensitive tuple:
%To find the most sensitive tuple, we pick the tuple from the above query who has the largest frequency $c$.
\begin{align} \label{eq:general_gj_most_sensitive_tuple}
%t^*_i = \argmax_{c} \Qgfreq^i(\attributes_\database)
t^* = \argmax_{t:t\in T^i, i=1,\ldots,m} t.\cnt
\end{align}
\end{itemize}

\cut{
\begin{proposition}
The tuple $t^*$ returned by Equation~\eqref{eq:general_gj_most_sensitive_tuple} gives the most sensitive tuple with its sensitivity $t^*.\cnt$.
%as $t^*.\attributes$ and its tuple frequency $t^*.\cnt$ from the domain of table $\relation_i$.
\end{proposition}
\begin{proof}
	By definition, Equation~\eqref{eq:general_gj_freq} computes and stores the tuple sensitivity as $\cnt$ for each $\attributes_i$ appears in $S^i$. $S^i$ covers the \representative domain of $\attributes_i$ by the construction rule. 
    Since all tuples outside this \representative domain has sensitivity 0, searching tuples within this domain can guarantee finding the most sensitive tuple and its corresponding sensitivity. 
\end{proof}

Although this approach gives us the correct result, the size of the sub-query $S^i$ in worst case could be $\Omega(n^{m-1})$.
The size of $T^i$ in worst case could be $\Omega(n^k)$.
In conclusion, this naive approach is polynomial in data complexity, but may be exponential in combined complexity.
}

Once again, the size of the sub-queries $S^i$ can be exponential in $m$ or $k$, which is polynomial in data complexity, but may not be efficient for practical purposes. 
To design an efficient algorithm for general CQs, we use \emph{hypertree decompositions} of the query \cite{Gottlob+1999, Abiteboul+1995}, which we briefly review below\footnote{There are multiple other equivalent notion of decompositions and width of general CQs, like \emph{generalized hypertree width, tree width, query width}, or \emph{fractional hypertree width} \cite{Chekuri:1997, Grohe:2001, Gottlob:2016}. Having a bound on these widths leads to polynomial time evaluation  for general CQs. We choose hypertree width as we needed that each relation in the query appears in only one node in the hypertree decomposition}. 

\stitle{Hypertree Decomposition.}
A hypertree $\tree_Q$ associated with a conjunctive query $Q$ is a tree with nodes labeled with attributes of the query $Q$ such that (1) each node in the  tree contains one or multiple relational atoms and all their attributes, 
%each node contains one or multiple relational atoms, 
and (2) for each attribute $A$, the nodes in 
$\tree_Q$ containing the same attribute forms a sub-tree. It can be seen that when each node in $\tree_Q$ contains a single relation, it is a \emph{join-tree} of $Q$ (Section~\ref{sec:acyclic}). 
%and 3) each relation from the query appears once and only once in the hypertree. The max number of relations within a node is defined as hypertree width. 

Each query has an associated hypertree, and it can be found in polynomial time if its \emph{hypertree-width},  is bounded. Given a hypertree of width $p$ for the input query, we represent this hypertree by 
a join tree $\tree(V,E, \map)$, where $V=\{v_1,\ldots,v_{|V|}\}$, $E=\{e_1,\ldots,e_{|E|}\}$ and $\map$ maps a relation $\R{i}$ to a node $v_j$ and each edge contains the common attributes between two nodes.
%%%Mapping of relations to nodes 
The number of nodes is less than the number of relations ($|V|<m$)
since multiple relations could be merged into one node. If $\R{i}$ is contained in $v_j$, then $\pi(\R{i}) = v_j$. 
%%use i for index of relations
%%use j for index of nodes
%%%Mapping of attributes to edges
We denote the union set of attributes from all relations in $v_j$ as $\attributes_{v_j}$, and the set of join attributes between $v_{j_1}$ and $v_{j_2}$ by $\attributes_{v_{j_1},v_{j_2}}$.
%%%Other notations
Let $p(v_j)$ denote the parent of node $v_j$ in the join tree,
$C(v_j)$ denote the child nodes of $v_j$,
and $N(v_j)$ denote the neighbors of $v_j$, i.e. $C(p(v_j)) \setminus \{v_j\}$. Within a node $\pi(\R{i})$, let $H(\R{i})$ denotes the group of cohorts of $\R{i}$, i.e. $\{\R{i'} \mid \R{i'} \in \pi(\R{i'}), \R{i'} \neq \R{i}\}$.
%; let $A(\R{i})$ denotes the attributes set between $\R{i}$ and $H(\R{i})$, i.e. $\cup_{\R{j} \in H(\R{i})} \attributes_{i, j}$
We denote $\subtree(v_j)$ as the subtree rooted at $v_j$, while $\comptree(v_j)$ is the complementary graph of $\subtree(v_j)$ on the tree $\tree(V, E, \pi)$.
%%%Property of a hypertree decomposition 
Since it's a hypertree decomposition, for each attribute, the nodes that contain this attribute always form a subtree. 
\subsection{Algorithm Details}\label{sec:general-algo}

%\todo{Add an introduction to the hypertree decomposition}. 
We present an algorithm based on a hypertree decomposition of a general join query. 



%\xh{We can add a definition box for this property if it's used later.}\yc{It should be used in efficiency analysis}


\stitle{Definitions.} For each relation $R_i$, let $v_j=\pi(R_i)$, the frequency table (Equation~\eqref{eq:general_gj_freq}) can be computed from the join of three groups of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$. In order to compute $T^i$, we define \emph{topjoin} and $\emph{botjoin}$ for each node $v_j$ in the hypertree:
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\tree(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}
Similar to the frequency table for a relation (Equation~\eqref{eq:general_gj_freq}), we define the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
T^{v_j}=  
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}
For $v_j$ as root or leaf, it has a simpler formula and we will discuss it in the algorithm.
Then the frequency table for a relation can be expressed using the frequency table of its node $\pi(R_i)$ and the cohorts of $R_i$ in $\pi(R_i)$: 
\begin{align}\label{eq:gj_fast_freq}
T^i= \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(T^{\pi(R_i)}), H(\R{i})))
\end{align}
x
%We use $\superjoin(R_1, R_2,\ldots, R_i)$ to denote the natural join between the relations $R_1,\ldots, R_i$. 

%Similar to Equation~\eqref{eq:general_gj_sub_query}, we capture the join result without the node $v_j$ in a hypertree $T$ as:
%\begin{align}\label{eq:gj_fast_node_sub_query}
%\Qgjoin^{v_j}(\attributes_\database) =
%\superjoin(\comptree(v_j), \{T(v_{j'})~|~v_{j'}\in C(v_j) \})
%\end{align}
%which is a natural join between the complementary tree of $v_j$ and the subtrees at the children of $v_j$. 



%\begin{align}\label{eq:gj_fast_node_sub_query}\Qgjoin^{v_i}(\attributes_\database) = \comptree(v_i) \superjoin \underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j)\end{align}
%\xh{This expression in \eqref{eq:gj_fast_node_sub_query} is not clear. what do you try to join here? } \yc{The symbol $\superjoin$ actually is a natural join and it reduces to cross product if there is no common attributes. Here, I want to join every nodes except $v_i$, so we need to join each child's subtree as $\underset{\forall v_j \in C(v_i)}{\superjoin} \subtree(v_j) = \subtree(v_{j_1})  \superjoin \subtree(v_{j_2})  \ldots \superjoin \subtree(v_{j_p}) $ and the complementary tree $\comptree(v_i)$.} 

\eat{
Now we can rewrite the Equation~\eqref{eq:general_gj_sub_query} in step (1) as \begin{align}\label{eq:gj_fast_sub_query}
\Qgjoin^i(\attributes_\database) 
=\superjoin(\Qgjoin^{\pi(R_i)}(\attributes_\database) , H(R_i))
\end{align}
Let $v_i$ be the corresponding node of $R_i$ in the hypertree, i.e., $v_j=\pi(R_i)$. This expression joins three types of relations: (i) the complementary tree of $v_j$, (ii) the subtrees rooted at the children of $v_j$, and (iii) the group of cohorts of $R_i$ in $v_j$.
}
%\begin{align}\label{eq:gj_fast_sub_query} \Qgjoin^i(\attributes_\database) = \Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin \underset{\forall \R{j} \in H(R_i)}{\superjoin} \R{j}\end{align}

\begin{figure}
	\centering
	\includegraphics[scale=0.45]{acyclic_join_recursion.pdf}
	\caption{Example of notations. \todo{Update the figure and description} \note{edit \href{https://docs.google.com/drawings/d/1xTBbD3DY4HEqO5I21m1UiGcjLAM9rrvS0YnmI5qm_J0/edit?usp=sharing}{here} }}
	\label{fig:gj_notations}
\end{figure}

\eat{
Given a table $R_i$ in $T$, as long as we know the maximum frequency of tuples projected on $\attributes_i$ from the joint output between tables other than $R_i$ in a join tree of $\Qgjoin$, as defined by $\Qgjoin^i$, we immediately get the max change to the final joint output due to adding or removing a tuple to $R_i$, and hence the local sensitivity of the query. We define the following invariants to compute the tuple sensitivity of a general query.
}

%\xh{May use this notation earlier}. 
%First, we assume all the relations has additional attribute $C$ to record the multiplicity of the other attribute values. For the base tables, we add attribute $c$ and assign $1$ to this attribute for every tuple. We also use $\superjoinagg(R_1,\ldots,R_i)$ to summarize two steps: (i) a natural join among $R_1, R_2,\ldots, R_i$ except the attribute $c$, and (ii) project the product of these multiplicity attributes to a new multiplicity column, i.e., $$\superjoinagg(R_1,\ldots,R_i)= \pi_{(R_1.C\times \cdots R_i.C)\rightarrow C} (\superjoin(R_1,\ldots, R_i)).$$
%Let $\groupbyagg{A}(R_i)$ represent a group by attribute $A$ and sum the counts and rename the sum as a new attribute $c$, i.e., 
%$$\groupbyagg{A}(R_i)= \aggregate{A}{sum(C) \rightarrow C}{(R_i)}.$$

\eat{
For each node $v_j$, we denote $\botjoin(v_j)$ and $\topjoin(v_j)$ as tables that computes the frequency of tuples projected on attributes shared by $v_j$ and its parent $p(v_j)$ from $\subtree(v_j)$ and $\comptree(v_j)$.
\begin{align}
\botjoin(v_j) &=  %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{T(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (T(v_j))
\label{eq:gj_botjoin}
\\
\topjoin(v_j) &= %\aggregate{\attributes_{v_j,p(v_j)}}{count(*) \as \cntt{v_j}{p(v_j)}}{\comptree(v_j)}
\groupbyagg{\attributes_{v_j,p(v_j)}} (\comptree(v_j))
\label{eq:gj_topjoin}
\end{align}


Denote the frequency table for $v_j$ as:
\begin{align}\label{eq:gj_fast_node_freq}
\Qgfreq^{v_j}(\attributes_\database) =  
%\aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big) 
\groupbyagg{\attributes_{v_j}}(\superjoinagg(\topjoin(v_j),
\{\botjoin(v_{j'})~|~v_{j'}\in C(v_j) \}))
\end{align}

%\begin{align}\label{eq:gj_fast_node_freq}
%\Qgfreq^{v_i} =  \aggregate{\attributes_{v_i}}{sum(\cntt{v_i}{p(v_i)} \underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as  c}{}
%\big( \topjoin(v_i) \superjoin \underset{\forall v_j \in C(i)}{\superjoin} \botjoin(v_j) \big)
%\end{align}

Now, equation (\ref{eq:general_gj_freq}) can be rewritten as:
\begin{align}\label{eq:gj_fast_freq}
\Qgfreq^i(\attributes_\database) = \groupbyagg{\attributes_i}(
	\superjoinagg(\groupbyagg{\attributes_i}(\Qgfreq^{\pi(R_i)}), H(\R{i}))
%	(\aggregate{\attributes_i}{sum(c) \as c}{\Qgfreq^{\pi(R_i)}}) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
)
\end{align}


\begin{lemma}
	Equation (\ref{eq:general_gj_freq}) and (\ref{eq:gj_fast_freq}) for step (2) are equivalent.
\end{lemma}
\begin{proof}
    
\end{proof}
}

%\begin{proof} 
%	Replacing $\Qgjoin^i(\attributes_\database)$ by equation (\ref{eq:gj_fast_node_sub_query}) and 
%	(\ref{eq:gj_fast_sub_query}), equation (\ref{eq:general_gj_freq}) can be rewritten as
%	\begin{align*}
%	  \Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	  	\Qgjoin^{\pi(\R{i})}(\attributes_\database) \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	  \Qgjoin^{\pi(\R{i})}(\attributes_\database) =~&
%	  	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	which is equivalent to
%	\begin{align*}
%	\Qgfreq^i(\attributes_\database) =~& \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}
%	R~ \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}\\
%	R =~& \aggregate{\attributes_i}{count(*) \as c}{}
%	\comptree(\pi(\R{i}))  \superjoin \underset{\forall v_j \in C(\pi(\R{i}))}{\superjoin} \subtree(v_j) 
%	\end{align*}
%	Notice that the intermediate relation $R$ is equivalent to equation (\ref{eq:gj_fast_node_freq}), so 
%	$\Qgfreq^i(\attributes_\database)$ can be rewritten as
%	\begin{align*}
%	\Qgfreq^i =~ \aggregate{\attributes_i}{sum(c) \as \tsens_i}{}\Qgfreq^{v_i} \superjoin  \underset{\forall \R{j} \in H(\R{i}) }{\superjoin} \R{j}
%	\end{align*}
%	, which is equivalent to equation (\ref{eq:gj_fast_freq})
%\end{proof}
%The last step is the same.

\paratitle{Algorithm.} The algorithm first prepares each tree node $v_j$ as the join among tables in $v_j$. Then it prepares $\bot(v_j)$ and $\top(v_j)$ for each node, and use them to compute $T^{v_j}$ for each node $v_j$. Finally, it computes $T^{i}$ for each relation $\R{i}$ and finds the most sensitive tuple and its tuple sensitivity. 

Note that computing  botjoin $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}) and topjoin $\top(v_j)$ (Equation~\eqref{eq:gj_topjoin}) for each node again may require exponential combined complexity, so we give an iterative approach in Algorithm~\ref{algo:gj_query} to compute them in polynomial combined complexity. After preparing botjoin and topjoin for each node, the third step is to combine them together and find the most sensitive tuple. We assume all joins are merge-sort joins.


\note{Illustrate the recursive structure of topjoin and botjoin by figure (\ref{fig:gj_notations}).}


To prepare each node $v_j$, we compute the join between 
%joins as $v_j = \underset{\forall \R{j} \in v_i }{\superjoin} \R{j}$ 
the relations in $v_j$ in an arbitrary join order.

To prepare $\bot(v_j)$ (Equation~\eqref{eq:gj_botjoin}), we start from the leaf nodes. Next, we compute $\botjoin$ for other nodes in a post-order traversal of the tree with this iterative formula:
\begin{align*}
\bot(v_j) = \groupbyagg{A_{v_i,p(v_i)}} (\superjoinagg(v_j, \{\bot(v_{j'})|  v_{j'}\in C(v_j) \}))
%\botjoin(v_i) =~&  \aggregate{A_{v_i,p(v_i)}}{sum(\underset{v_j \in C(v_i)}{\product} \cntt{v_i}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
% &v_i \superjoin (\underset{\forall v_j \in C(v_i) }{\superjoin} \botjoin(v_j))
\end{align*}
For each $\botjoin(v_j)$, the join starts with $v_j$ and follows by the children of $v_j$ one by one.  
%use $v_i$ to join $\botjoin(v_j)$ $\forall v_j \in C(v_i)$ one by one. %\note{It is clearer in the algorithm box}


\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in C(v_i)$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows, and proving by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}}

To prepare $\top(v_j)$, we start with the root node. Next, we compute $\topjoin$ for other nodes in a pre-order traversal of the tree with this iterative formula:
\begin{align*}
\top(v_j) = \groupbyagg{A_{v_i,p(v_i)}}(
\superjoinagg(p(v_j), \top(p(v_j)), \{\bot(v_{j'}) | v_{j'}\in N(v_j)  \}))
%\topjoin(v_i) =~& \aggregate{A_{v_i,p(v_i)}}{sum(\cntt{p(v_i)}{p(p(v_j))} \cdot  \underset{v_j \in N(v_i)}{\product} \cntt{p(v_i)}{v_j}) \as \cntt{v_i}{p(v_i)}}{} \\
%&p(v_i) \superjoin \topjoin(p(v_i)) \superjoin \underset{v_j \in N(v_i)}{\superjoin}\botjoin(v_j)
\end{align*}
For each $\top(v_j)$, the join starts with $p(v_j)$ and $\top(p(v_j))$ and follows by the botjoin of the neighbors of $v_j$ one by one. 
%The join order is as follows: use $p(v_j)$ to join $\topjoin(p(v_j))$ and $\botjoin(v_j) ~ \forall v_{j'} \in N(v_j)$ one by one.

\eat{The correctness follows as replacing $\botjoin(v_j)$ from the above formula for each $v_j \in N(v_i)$ by the definition of botjoin as equation (\ref{eq:gj_botjoin}) shows, and replacing $\topjoin(p(v_i))$ by the definition of topjoin as equation (\ref{eq:gj_topjoin}) shows. Finally, prove it by induction.\note{Do we need more steps to show the correctness/equivalence?} \xh{Move this correctness to proof.}
}
 
After preparing all the topjoins and botjoins, we combine these results to obtain the frequency tables $T^i$  for $i=1,\ldots,m$ based on Equations~\eqref{eq:gj_fast_node_freq} and~\eqref{eq:gj_fast_freq}. Notice that when computing $T^{v_j}$, we drop topjoins for root node and we drop botjoins for leaf nodes; and when computing  $T^{i}$, we drop $H(R_i)$ if $\R{i}$ is the only relation within the node. 
We iterate all the frequency tables $T_i$ and find the tuple with maximum $\cnt$. This tuple is returned as the most sensitive tuple with its $\cnt$ as the local sensitivity of this query on the given database instance.

%Though there exists efficient ways to compute these joins, we leave the analysis of the tightest parameterized complexity for these equations as future work. In this work, we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order.  
 
 
 \eat{
 and find the most sensitive tuple, for each relation $\R{i}$, we need to construct $\Qgfreq^i(\attributes_\database)$ according to equation (\ref{eq:gj_fast_node_freq}) and (\ref{eq:gj_fast_freq}). These equations include joins among $\topjoin(v_j)$, $\botjoin(v_{j'}) ~ \forall v_{j'} \in C(v_j)$ and $\forall \R{i'} \in H(\R{i})$. Although there exists efficient ways to compute these joins, we postpone this to the future work and leave this as an open problem to analyze the tightest parameterized complexity for these equations. Here we use a naive join algorithm as doing merge-sort join one by one in an arbitrary order. }  

\eat{\note{New rule. We need to avoid cross product. This matches the rule in path join.} For the last step, instead of computing $\Qgfreq^i(\attributes_\database)$ with all joins together, we divide joins into several join groups and get disjoint join results in aspect to attributes. Any two join groups share no common attributes from relations inside the group. We later merge them back by choosing max from each cluster. 
\note{Double Hypertree Width} Within each join group, we arrange the join order according to the hypertree decomposition of relations within the group. Denote double hypertree width as the max hypertree width within each join group.}

Instead of computing $T^i$ with merge-sort joins one by one in an arbitrary order, we partition the joins into groups such that relations from different groups share no common attributes. We find the most sensitive tuple per join group. Within each join group, we arrange the join order according to the hpyertree decomposition of relations within the group. We denote the maximum hypertree width within each join group as \emph{double hypertree width} for relation $\R{i}$. Double hypertree width for the enitre query is defined as the max double hypertree width from each $\R{i}$.

\begin{theorem}
	Algorithm~\ref{algo:gj_query} computes the local sensitivity of a general join query and also finds the corresponding most sensitive tuple. Given $m$ tables with size $n$ and $\leq k$ attributes for each, and a hypertree decomposition of the  general join query with hypertree width $p$ and double hypertree width as $q$ and $m' \leq m$ nodes, the time complexity is $O(m p q  \log n \cdot n^{pq} )$ .
\end{theorem}

\begin{proof} Computing the joins within a node has a complexity of $O(\sum_{i=2}^{p}{n^i})$. Given $m'<m$ number of nodes, the first step has an $O(m'n^p)$ complexity.
%	$O(m'n^p)$ for computing joins within a node  * m nodes (consider $O(\sum_{i=2}^{p}{n^i})$ for a single node).

The time to compute the topjoins and botjoins for $m'$ nodes is $O(m'n^p \log n^p)$ as the size of a node is at most $O(n^p)$).
%for computing top/bot joins for $m'$ nodes (the size of a node is at most $O(n^p)$).

Finally, to compute $T^i$ for $m$ relations, the time complexity is 
$O(mn^{pq} \log n^{pq})$.% for computing $T^i$ for $m$ relations.

Hence, the total time complexity is $O(mn^{pq} \log n^{pq})$ or $O(m p q  \log n \cdot n^{pq} )$. 
\end{proof}

\subsection{Extensions}\label{sec:extensions}
\textbf{Extension to selection and projection.~} 

Although by default each relation appears in the query body is the original base table, with extra rules, the algorithm can support using a table after selection and projection of its base table for the query body. For each tuple: 1) the tuple sensitivity is not affected by projection since we assume projection keeps duplicates. 2) if the tuple doesn't match the predication of its table's selection, we set the tuple sensitivity as 0, since it is dropped by selection before it can join other tuples. Applying rules 1 and 2 will not affect the complexity.

\textbf{Extension to disjoint query components.~} 

If the hypergraph of query is not connected, we get a hyperforest containing multiple disjoint hypertrees instead of a single hypertree for a query. In this case, we run our algorithm for each hypertree. We then update the tuple sensitivity by multiplying it with the join size of other hypertrees. The join size of each hypertree can be computed as the sum of frequency from the botjoin of each hypertree root, so it will not affect the complexity. 

\textbf{Extension to attributes appearing in only one relation.~}

%\sr{for attributes in one relation, please complete}  
If an attribute  $A$ appears in only one relation $R_i$,  and the relation is connected with other relations by other attributes, $A$ does not affect the local sensitivity, but  the  tuple $t$ with  the maximum tuple sensitivity may be from $R_i$, so  we  would  need  a value of $t.A$. Similar to Algorithm~\ref{algo:ls_pathquery}, if the  other  attributes in $R_i$ except $A$ come from an  existing  tuple $t'$  in  the  instance, we augment 
it with $t'.A$ (for downward sensitivity). If there are no such tuples $t'$, we choose any value from the active domain of $A$ to extend the other attributes to form such a tuple $t$ (for upward sensitivity). 

\input{double_acyclic_join}

==> pathjoin_v0.tex <==
\section{Path Join Query}\label{sec:path}


In this section, we give an efficient algorithm for a special class of acyclic queries called \emph{path join queries} or \emph{path queries} that run in polynomial time in combined complexity, {\em irrespective of the output size} (note that the polynomial combined complexity for query evaluation of acyclic and path queries is polynomial in input query, input database, and also the output size, which can be exponential in the query size).  
\cut{
\am{We begin describing an efficient algorithm for the sensitivity problem for a simpler class of \textit{path join queries}.}
}
%Consider a special class of the CQ query in the form as:
A path join query has the following form:
\begin{align*}
    \Qpjoin(\attributes_\database)
    \datalogEQ 
    \relation_1(A_0, A_1),
    \relation_2(A_1, A_2),
    \ldots,
    \relation_{m}(A_{m-1}, A_{m})
\end{align*}
where $\attributes_\database = \{A_0, A_1, \ldots, A_m\}$ and each relation $\relation_i$ contains two attributes: $A_{i-1}$ and $A_i$. %We call this class of CQ queries as path join queries.
Note that the above form can be used when two adjacent relations share more than one attributes, since we can replace multiple attributes with a single attribute using combinations of values for multiple attributes. Path joins can capture natural joins in many scenarios, like joining {\tt Students, Enrollment, Courses, TaughtBy, Instructors, $\cdots$} relations, or, joining {\tt Region, Nation, Customer, Orders, and Lineitem} (e.g., in TPC-H data, see Section~\ref{sec:experiments}). In addition, our algorithm for path join queries will give the basic ideas of our algorithms that can handle general CQs discussed in Section~\ref{sec:general}. 

\cut{
\am{Why is this an interesting class of queries? Give one or two examples? If it does not have direct applications, say that we first present this as it will help understand the our general algorithm.}
}

\begin{figure}[t]
	\begin{center}
		\includegraphics[scale=0.5]{{"figures/Path Join Example"}.pdf}
		\caption{\revc{A path join query $\qpeg(A, B, C, D, E):-R_1(A, B), R_2(B, C), R_3(C, D), R_4(D, E)$ and the procedure of computing tuple sensitivities from $R_2$. 
		%Topjoin $\top(R_1)$ is a group-by count on $B$ from $R_1$, and botjoin $\bot(R_4)$ is a group-by count on $D$ from $R_4$. The join of $R_3$ and $\bot(R_4)$ gives an intermediate table, which is equivalent to a group-by count on attributes $C,D$ from the join between $R_3$ and $R_4$. The following group-by count on $C$ gives the botjoin $\bot(R_3)$. The right bottom table is the result after full join. Now consider a tuple $(b1, c1)$ from $R2$, we found 2 "incoming" paths ending at $b1$ from $\top(R1)$ and 2 "outgoing" paths starting at $c1$ from $\bot(R3)$, so the tuple sensitivity of $(b1, c1)$ is the product of number of "incoming" and "outgoing" paths as $2 \times 2 = 4$.
		}}
		\label{fig:path}
	\end{center}
\end{figure}


\eat{
\begin{algorithm}[t]
\begin{small}
	\caption{Compute Local Sensitivity of a Path Join Query and the corresponding Most Sensitive Tuple}
	\label{algo:ls_pathquery}
	\begin{algorithmic}[1]
	\Require Path join query $\Qpjoin(\attr_0 \ldots \attr_m)$, the DB instance $\database$
	\Ensure $\LS(Q, \database)$, and a most sensitive tuple $\kingtuple$
		\Procedure{LSPathJoin}{} %{LS}{$\Qpjoin, \database$}
		\Statex I) Prepare topjoin
		\State $\topjoin(\R{2}) = \groupbyagg{\attr_1}{\relation_1}$ \emph{ /* also adds the $\cnt$ values */} %\aggregate{\attr_1}{count(*) \as \cnt{}{1}}{\relation_1}$
		\For{$i=3,\ldots,m$}
		    \State $\topjoin(\R{i}) = %\groupbyagg{A_{i-1}}{\topjoin(\R{i-1}) \Join \relation_{i-1}}$ \emph{ /* also multiplies and adds the $\cnt$ values */}
		    \groupbyagg{A_{i-1}}{\superjoinagg{(\topjoin(\R{i-1}), \relation_{i-1}})}$ \emph{ /* also multiplies and adds the $\cnt$ values */}
		    %$\topjoin(\R{i}) = \aggregate{A_{i-1}}{sum(\cnt{}{i-2}) \as \cnt{}{i-1}}{\topjoin(\R{i-1}) \bowtie \relation_{i-1}}$
		\EndFor
		\Statex II) Prepare botjoin
        \State $\botjoin(\R{m}) = \groupbyagg{\attr_{m-1}}{\relation_m}$ \emph{/* also adds the $\cnt$ values */}
        %\aggregate{\attr_{m-1}}{count(*) \as \cnt{}{m-1}}{\relation_m}$
		\For{$i=m-1,\ldots,2$}
		    \State $\botjoin(\R{i}) = %\groupbyagg{A_{i-1}}{\botjoin(\R{i+1}) \bowtie \relation_i}$ 
		    \groupbyagg{A_{i-1}}{\superjoinagg{(\botjoin(\R{i+1}), \relation_i)}}$ 
		    \emph{ /* also multiplies and adds the $\cnt$ values */}
		    %\aggregate{A_{i-1}}{sum(\cnt{}{i}) \as \cnt{}{i-1}}{\botjoin(\R{i+1}) \bowtie \relation_i}$
		\EndFor
		\Statex III) Select most sensitive tuple 
		%\sr{please check -- it seems all are handling single tuples so I removed $\pi$, also took care of tuple insertions in $R_1$ or $R_m$}
		\Statex \emph{/* Select most sensitive tuples $t_i$ from each $R_i$. First find $t_1, t_m$.*/}
		\State $t_1.A_1 = \argmax_{t \in \botjoin(\R{2})} t.\cnt$, ~~ $t_1.A_0 = t.A_0$ if there is a $t \in R_1$ with $t.A_1 = t_1.A_1$, otherwise any value from the active domain of $A_0
		$. 
		%\red{check}
		%\pi_{\attr_1, \max(\cnt{}) \as \tsens } ~ \botjoin(\R{2})$
		\State $t_m.A_{m-1} = \argmax_{t \in \topjoin(\R{m})} t.\cnt$, ~~ $t_m.A_{m} = t.A_m$ if there is a $t \in R_m$ with $t.A_{m-1} = t_m.A_{m-1}$, otherwise any value from the active domain of $A_m$. 
		%\red{check} 
		%\pi_{\attr_{m-1}, \max(\cnt) \as \tsens} ~ \topjoin(\R{m})$
		\State $t^* = \argmax(t_1.\cnt, t_2.\cnt)$ \emph{/* the current max tuple sensitivity value */}
		\For{$i=2,\dots,m-1$}
		    \State $t^{top}_i = \argmax_{t \in \topjoin(\R{i})} t.\cnt$  %$t^{top}_i = \pi_{\attr_{i-1}, \max(\cnt{}{i-1}) \as \tsens_{i-1} } ~ \topjoin(\R{i})$
		    \State $t^{bot}_i =
		    \argmax_{t \in \botjoin(\R{i+1})} t.\cnt$
		     %$t^{bot}_i = \pi_{\attr_{i}, \max(\cnt{}{i}) \as \tsens_{i} } ~ \botjoin(\R{i+1})$
		    \State $t_i.A_{i-1} =  t^{top}_i.A_{i-1},~~ t_i.A_{i} = t^{bot}_i.A_i,~~ t_i.\cnt = t^{top}_i.\cnt * t^{bot}_i.\cnt$ \emph{/* the most sensitive tuple for $R_i$*/} %$t_i = \pi_{\attr_{i-1}, \attr_{i},\tsens_{i-1} *  \tsens_{i} \as \tsens} t_{top}[i], t_{bot}[i]$
		    \State $t^* = \argmax(t^*.\cnt, t_i.\cnt)$ \emph{/* update $t^*$ if needed*/}
		\EndFor
		\State $\LS = t^*.\cnt$
		%\State $\kingtuple = t.\attributes$
		\State \textbf{return} $\LS, t^*$
		\EndProcedure
	\end{algorithmic}
	\end{small}
\end{algorithm}
}

\subsection{Simple but Inefficient Solution}\label{sec:pj_simple_ineffi}
First, we discuss the basic idea of our algorithm using a toy example of path query in Figure~\ref{fig:path} with four relations. Here we have the path query:
$$\qpeg(A, B, C, D, E):-R_1(A, B), R_2(B, C), R_3(C, D), R_4(D, E).$$
%The database instance $\database$
Note that how much adding or removing a tuple $t$ to any of the relations $R_i$ affect the number of overall result tuples, totally depend on the number of ways that $t$ can combine with tuples, or in this case `join-paths', in the remaining relations. For instance, for the tuple $R_2(b1, c1)$, there are two matching tuples in $R_1$ (with the same $B = b1$ value) \revc{indicating "incoming" paths ending at $b1$ as shown in the table $\topjoin(R2)$}, and $1 \times 1 + 1 \times 1= 2$ matching tuples in $R_3 \Join R_4$ (with the same $C = c1$ value) \revc{indicating "outgoing" paths starting at $c1$ as shown in the table $\botjoin(R3)$}, therefore, if $R_2(b1, c1)$ is removed from the database $\database$, $2 \times 2 = 4$ tuples will be removed from the answer of $\qpeg(\database)$. \revc{$\topjoin(R2)$ and $\botjoin(R3)$ will be explained in the next section.}

\reva{Notice that if we only consider removing tuples from the active domain, we can just apply Yannakakis's algorithm \cite{Yannakakis:1981} to compute the size of join output after removing a tuple in $\tilde{O}(n)$ time, and repeat it for $n$ tuples, which results in $\tilde{O}(n^2)$. However, we also need to capture the changes by adding tuples from the representative domain, and it is shown in the proof of \ref{thm:poly-data-complexity} that the size of the representative domain is $O(n^k)$, which means we cannot simply trying each tuple \am{the sentence does not parse}. A better idea is to avoid query evaluation and capture the effects of adding or removing tuples simultaneously.}

\am{In order to get space, I recommend dropping this section on Simple but Inefficient Solution. The first para in 4.1 is useful -- maybe you can call that ``intuition". But, we should drop the Join and group-by with multiplication section and the simple algorithm section. We can replace it with a line or two like this: 

It is easy to see that the sensitivity of adding or removing a row in $(a_i,b_i) \in R_i$ is the product of the number of incoming paths ending in $a_i$, the number of outgoing paths in $b_i$ and the multiplicity of $(a_i, b_i)$ in $R_i$. However, this is inefficient since the number of incoming/outgoing paths can be exponential in the number of relations (and thus not have a polynomial combined complexity).}

\paratitle{Join and group-by with multiplicities.} To capture the above intuition systematically  for  all tuples in the database, as well as all tuples in the representative domain (Definition~\ref{def:repr}) that can be inserted, we introduce some notations. 
We assume that each base or intermediate relation has an additional attribute $\cnt$ to record the multiplicity of the other attribute values in  that relation. For the base tables $R_1, \cdots, R_m$, $\cnt$ has value $1$ for every tuple (but there can be multiple identical tuples in the base relations) \am{This is confusing. Can we just sat $\cnt$ is the multiplicity of a tuple in the base relation?}. For $j > i$, we use the shorthand $\superjoinagg(R_i, \ldots, R_j)$ to summarize two steps: 
%\begin{itemize}
%\itemsep0em
    %\item 
    (a) a natural join among $R_i, R_{i+1},\ldots, R_{j-1}, R_j$ except the attributes $\cnt$, and 
    %\item 
    (b) projection of the product of these multiplicity attributes $\cnt$ to a new multiplicity column\footnote{A more systematic way to propagate the multiplicity for arbitrary queries has been discussed in the literature, e.g., \cite{AhmadKKN12, AmsterdamerDT11}.}, i.e., abusing RA expressions:
    %\begin{equation}\label{equn:i-to-j}
    $\superjoinagg(R_i,\ldots,R_j)= \pi_{\attributes_i,\ldots,\attributes_j,(R_i.\cnt\times \cdots \times R_j.\cnt)\rightarrow \cnt} (R_i \Join \ldots \Join R_j)$. 
    %\end{equation}
%\item 
Further, given any base or intermediate relation $R$, we assume the group-by operation $\groupbyagg{\attributes}(R)$ computes groups according to a set of attributes $\attributes \subseteq \attributes_R$, and also sums the counts as the new count attribute, i.e.,
%\begin{equation}\label{equn:gb-cnt}
$\groupbyagg{\attributes}(R)= \aggregate{\attributes}{sum(\cnt) \rightarrow \cnt}{(R)}$.
%\end{equation}
%\end{itemize}

\paratitle{Simple algorithm.} Using the above operators, we can compute the tuple $t^*$ giving the largest tuple sensitivity as follows: 
%\begin{enumerate}
%\itemsep0em
    %\item[(i)] 
    %(i) and (ii)  
    For each $i = 1, \cdots, m$, compute
    \begin{equation}
    \footnotesize
    \label{eq:simple-1}
    S^i = \big(\superjoinagg(R_1,\ldots,R_{i-1})\big) \superjoin \big(\superjoinagg(R_{i+1},\ldots,R_m)\big)
    %\superjoin(R_1,\ldots,R_{i-1}, R_{i+1},\ldots, R_m)
    \end{equation}
    %\note{yc: replace $\Join$ with $\superjoinagg$? otherwise we have two cnt in $S^i$}
    %\item[(ii)] 
    %(ii) For each $i = 1, \cdots, m$, compute
    \begin{equation} \label{eq:simple-2}
    \footnotesize
    T^i = \groupbyagg{A_{i-1}, A_i}(S^i)
    \end{equation}
    %\item[(iii)] 
    %(iii)  
    Finally, return \change{the tuple with the maximum tuple sensitivity}
    \begin{equation}\label{eq:simple-3}
	\footnotesize       
    t^* = \argmax_{t: t \in T^i, i = 1, \cdots, m} t.\cnt
    \end{equation}
    %as the tuple with the maximum tuple sensitivity.
%\end{enumerate}

Note that the relations in the two sub-joins in (\ref{eq:simple-1}) do not share any attribute, so their join is equivalent to a cross product. Due to the same reason, by (\ref{eq:simple-2}) and (\ref{eq:simple-3}), in $T^i$ we are not only getting the tuples in the active domain of $R_i$, but also considering all the tuples from its representative domain (Definition~\ref{def:repr}) that can lead to a non-zero local sensitivity by joining with tuples in the other relations, which takes care of both \reva{\textbf{upward}} and \reva{\textbf{downward}} tuple sensitivities. 

\cut{
To find the local sensitivity of a CQ query and the corresponding most sensitive tuple, we search for the most sensitive tuple from each table's domain, and then select the most sensitive one from them. Notice that the most sensitive tuple may not exist in the current table. Observe that the query can always be rewritten as a join between a table $\relation$ and the join of other tables. Adding or removing one tuple from $\relation$ results in adding or removing corresponding $x$ tuples from the join of other tables, by the definition of join. The number $x$ can be computed instead of knowing the table $\relation$. So one simple approach to find the most sensitive tuple from $\relation$ is to construct a new sub-query by removeing the table from the original CQ query, and then find the tuple of the maximum frequency from the query result. Notice that the new sub-query may involve cross product.

\am{This english description is vague and hard to understand. Can you just use Fig 1 to give the intuition? }

\note{add an example path query with 4  tables and exaplain how it  works. Show it again for 4.2}

\todo{Emphasize for each i}

\am{Figure 1 is never explained in the text. Based on the figure and the caption, it is not clear to the reader what is happening. Also, can the figure mirror the three steps (1), (2) and (3) more clearly without all the arcs and X's. Maybe label the first with D, the second with $Q^i_{path}(A_D)$ and $Q^i_{pf}(A_D)$}


(1) For path join queries, we define $\Qpjoin^i(\attributes_\database)$ as:
\begin{align}\label{eq:general_sub_query}
    \Qpjoin^i(\attributes_\database)
    \datalogEQ
    & \relation_1(A_0, A_1) ,\ldots, \relation_{i-1}(A_{i-2}, A_{i-1}), \nonumber \\
    & \relation_{i+1}(A_{i}, A_{i+1}) ,\ldots, \relation_m(A_{m-1}, A_m)
\end{align}
which is a sub-query from the original path join query by removing the relation $\relation_i$. 

(2) Then we do a counting group by on attributes $A_{i-1}$ and $A_i$.
\begin{align}\label{eq:general_freq}
    \Qpfreq^i(\attributes_\database) = {\aggregate{A_{i-1}, A_i}{count(*) \as c}{\Qpjoin^i(\attributes_\database)}}
\end{align}
to count the frequency of each tuple.

(3) To find the most sensitive tuple, we pick the tuple from the above query who has the largest frequency $c$. 
\begin{align} \label{eq:general_most_sensitive_tuple}
	t^*_i = \argmax_{c} \Qpfreq^i(\attributes_\database)
\end{align}



\am{Why proposition and not theorem or lemma?}

\begin{proposition}
	The $t^*_i$ from the equation \ref{eq:general_most_sensitive_tuple} contains the most sensitive tuple as $t^*_i.A_{i-1}A_i$ and its tuple frequency $t^*_i.c$ from the domain of table $\relation_i$.
\end{proposition}
\begin{proof}
	By definition, equation (\ref{eq:general_freq}) computes the tuple sensitivity as $count(*)$ $\as$ $c$ for each $A_{i-1}, A_i$ appears in $\Qpjoin^i(\attributes_\database)$. We further show that these tuples forms the \representative domain $\reprdomain^{A_{i-1}, A_i}$.
	The cross product of $\topjoin(R_{i})$ and $\botjoin(R_{i+1})$ includes all tuples from $\actdomain^{A_{i-1}} \times \actdomain^{A_{i}}$, which by definition is the representative domain $\reprdomain^{A_{i-1},A_{i}}$ about $\R{i}$.  Since all tuples outside this domain has sensitivity 0, searching tuples within this domain can guarantee finding the global most sensitive tuple and corresponding sensitivity. 
\end{proof}
}

%\sr{edited up to here}
This approach, however, does not give a polynomial combined complexity for path join queries as desired, since the size of the sub-queries $S^i$-s can be exponential in $m$ if there are many paths from $R_1$ to $R_m$, which we address in the next subsection. 

\cut{
Although this approach gives us the correct result, the size of the sub-query $\Qpjoin^i(\attributes_\database)$ in worst case could be $\Omega(n^{m-1})$.
%which is also linearly related to the time complexity of evaluating this sub-query and finding the most frequent tuple. 
In conclusion, this naive approach is polynomial in data complexity, but may be exponential in combined complexity.
}


\input{pathjoinalgo}


\eat{
\subsection{Efficient Algorithm for Path Queries}\label{sec:pj_effi}
%\am{Change title to \textit{efficient solution}?}
\cut{
We present an optimized algorithm by the following analysis. For step 1 and 2, notice that the last step is to do a group by on attributes $A_{i-1}$ and $A_{i}$ and do a counting as frequency, which means we don't need to keep information other than $A_{i-1}$ and $A_{i}$. \am{What does this mean?} For step 2 and 3, notice that the last step is to find the maximum and we can push down the max operator into the first step. \am{What does this mean?}
}

Algorithm~\ref{algo:ls_pathquery} describes an efficient way to compute steps \eqref{eq:simple-1}, \eqref{eq:simple-2}, \eqref{eq:simple-3} in the simple algorithm by keeping track of the count values in two passes that takes (near-)linear-time for each relation. \reva{This idea is borrowed from Yannakakis's algorithm \cite{Yannakakis:1981}, which tracks the tuple counts in one pass and computes the size of acyclic join in $\tilde{O}(n)$ time. Here we make two passes and store each intermediate tuple counts.} To explain how this algorithm works, we first introduce some notations, and rewrite \eqref{eq:simple-1} and \eqref{eq:simple-2} as follows.

\cut{
For step 1, denote $\Qpjoin(\relation_i 
\ldots \relation_j)$ $\datalogEQ$ $\relation_{i}(A_{i-1}, A_{i}), $ $\ldots,$ $ \relation_{j}(A_{j-1}, A_{j})$
. Now the equation \ref{eq:general_sub_query} can be rewritten as
\begin{align} \label{eq:pj_fast_sub_query}
\Qpjoin^i(\attributes_\database) = \Qpjoin(\relation_1, \ldots, \relation_{i-1}) \times \Qpjoin(\relation_{i+1}, \ldots, \relation_m)
\end{align}
}

\ \\{\bf Topjoin and botjoin.~} We define \emph{topjoin} $\topjoin(\R{i})$ and \emph{botjoin} $\botjoin(\R{i})$ for $\R{i}$ as follows, which respectively compute the multiplicities of the values of  attribute $A_{i-1}$ for the partial path joins from $\R{1}$ to $\R{i-1}$, and $\R{i}$ to $\R{m}$ using the $\superjoinagg$ and $\groupbyagg{}$ operators discussed earlier that take into account multiplicities. 
%(\ref{equn:i-to-j}) and (\ref{equn:gb-cnt}):
{\small
\begin{align}
\topjoin(\R{i}) &= \groupbyagg{\attr_{i-1}}{\big(\superjoinagg(\relation_1, \ldots ,\relation_{i-1})\big)} \label{eq:pj_topjoin}
    \\
    \botjoin(\R{i}) &= \groupbyagg{\attr_{i-1}}{\big(\superjoinagg(\relation_{i}, \ldots ,\relation_m)\big)} \label{eq:pj_botjoin}
\end{align}
}    
Therefore, 
%$\botjoin(\R{i+1}) = \aggregate{\attr_{i}}{count(*) \as \cnt{}{i}}{\Qpjoin(\relation_{i+1}, \ldots ,\relation_m)}$.
{\small
\begin{equation}
    \botjoin(\R{i+1}) = \groupbyagg{\attr_{i}}{\big(\superjoinagg(\relation_{i+1}, \ldots ,\relation_m)\big)}. 
\end{equation}
}
and, (\ref{eq:simple-2}) can be rewritten for $i = 2, \cdots, m-1$ (abusing RA expressions)
{\small
    \begin{equation}\label{eq:better-2}
    T^i = \pi_{\attr_{i-1}, \attr_{i}, (\cnt \times \cnt) \rightarrow \cnt } \big( \topjoin(\R{i}) \times \botjoin(\R{i+1})\big)
    \end{equation}
} 
In addition,
{\small
    \begin{equation}\label{eq:better-2-extremes}
    T^1 = \botjoin(\R{2}) ~~~~ \text{and} ~~~~  T^m = \topjoin(\R{m}) %\red{~~~~~S: check} correct
    \end{equation}
}
    \cut{
\begin{align}\label{eq:pj_fast_freq}
    \Qpfreq^i(\attributes_\database) = \pi_{\attr_{i-1}, \attr_{i}, (\cnt{}{i-1} * \cnt{}{i}) \rightarrow c } (\topjoin(\R{i}) \times \botjoin(\R{i+1}))
\end{align}
}
Note that $\topjoin(\R{i})$ and $\botjoin(\R{i+1})$ do not share any attribute, so the join in (\ref{eq:simple-1}), and can be written as a cross product in (\ref{eq:better-2}). Further, we multiply the $\cnt$ values of the joining tuples and store them in the new $\cnt$ attribute.

\cut{
If $\topjoin(\R{i})$ or $\botjoin(\R{i+1})$ is not defined, we simply remove it and corresponding items from the above query. \am{When are they not defined?} Notice that we don't use $\Qpjoin^i(\attributes_\database)$ in the equation. Later in Lemma~\ref{blah} we show that (\ref{eq:general_freq}) and (\ref{eq:pj_fast_freq}) compute the same table in two different ways, and therefore we can again select the tuple with maximum value of $c$ in the step 3. \am{Since the lemma comes immediately next, you can say, "Next we show that ..." }
}

%\sr{removing lemma for equivalence as it is simple}

\cut{
\begin{lemma}
Equation (\ref{eq:general_freq}) and (\ref{eq:pj_fast_freq}) are equivalent.
\end{lemma}

\begin{proof}
	Replacing $\Qpjoin^i(\attributes_\database)$ by equation (\ref{eq:pj_fast_sub_query}), equation (\ref{eq:general_freq}) can be rewritten as  $\Qpfreq^i(\attributes_\database)$ = $\aggregate{A_{i-1}, A_i}{count(*) \as c}{}$ $\Qpjoin$ $(\relation_1,$ $\ldots,$  $\relation_{i-1})$ $\times$ $\Qpjoin(\relation_{i+1}, \ldots, \relation_m)$. Notice that this is a counting group-by query on attributes $A_{i-1}$ and  $A_i$. Since $A_{i-1}$ only appears in $\Qpjoin(\relation_1, \ldots, \relation_{i-1})$ while $A_i$ only appears in $\Qpjoin(\relation_{i+1}, \ldots, \relation_m)$, it is equivalent to do group by on each path join query first and then merge them together.
\end{proof}
}

\paratitle{Algorithm.~} 
%The algorithm basically prepares topjoin and botjoin first and then use them to find the most sensitive tuple. 
Note that explicitly computing topjoin (\ref{eq:pj_topjoin}) and botjoin (\ref{eq:pj_botjoin}) again may require exponential combined complexity, so we give an iterative approach in Algorithm~\ref{algo:ls_pathquery} to compute them in polynomial combined complexity. After preparing topjoin and botjoin, the third step is to combine them together and find the most sensitive tuple as in (\ref{eq:simple-3}). The efficiency of this step is also boosted by pushing down the max operator to the sub-queries. 
\cut{
We assume all joins are merge-sort joins. \am{Is that a reasonable assumption? Do you need to sort each relation twice once on the left attribute and one on the right attribute?}
}

To prepare topjoin (\ref{eq:pj_topjoin}), we first compute $\topjoin(\R{2})$ as a base case in the way as topjoin is defined in equation (\ref{eq:pj_topjoin}). Next, we iteratively compute $\topjoin(\R{i})$ for $i =   $ 
3 to m in the algorithm. 
%For each iteration, notice we only join a base table with a topjoin table , which has already been "group-by"ed on join attributes, so the size of $\topjoin(\R{i})$-s cannot be larger than the size of $\R{i}$ and is $O(n_i)$ for each. 
As in the efficient query evaluation for acyclic queries\cite{Abiteboul+1995}, we use \emph{sort-merge joins} to compute the pairwise joins and the then groupby (sort both relations on the join column, join together, then groupby and add the $\cnt$ values).  which can be implemented in 
\revm{$O(n_i \log n_i)$}
time
\revc{as $R_{i-1}$ can join at most one tuple in $\topjoin(R_{i-1})$} 
.
%\footnote{This complexity holds only when join selectivity is a constant. All joins in algorithm \ref{algo:ls_pathquery} has join selectivity as 1 so this complexity holds.}. 
Similarly, $\botjoin(\R{i})$-s are computed. In total, these two steps take 
\revm{$\sum_{i=1}^{m} O(n_i \log n_i) = O(n \log n)$}
time. 
\par
Then in III) we find the tuples $t_i$ with maximum tuple sensitivity for every table $R_i$, and the maximum tuple sensitivity over these $t_i$-s give $t^*$ - the tuple giving the local sensitivity of $\Qpjoin$. For $R_1$, the sensitivity depends on the join $\botjoin(R_2)$, i.e., the join of the rest of the tables $R_2, \cdots, R_m$. Suppose $C_1^*$ is the maximum $\cnt$ value in $\botjoin(R_2)$ and $a_1$ be the corresponding value of $A_1$. But $\botjoin(R_2)$ only has attribute $A_1$, while a tuple to be inserted to or deleted from $R_1$ needs both $A_0, A_1$. The tuple  with $\cnt = C_1^*$ from $\botjoin(R_2)$ gives the value of $A_1 = a_1$ for $t_1$. If there is an existing tuple $t \in R_1$ such that $t.A_1 = a_1$, we can choose $t$ as $t_2$, as removing $t$ from $R_1$ will change the size of the result by $C_1^*$. Otherwise, inserting a new tuple $t_1 = (a_0, a_1)$ with  $A_1 = a_1$ and any value $a_0$ from the active domain (or, the domain) of $A_0$ will change the size of the result by $C_1^*$.   Similarly,  the tuple giving maximum tuple sensitivity for $R_m$ is computed using $\topjoin(R_m)$. 
\par
Then we find the tuple $t_i$ with maximum tuple sensitivity for $R_i$, $i = 2, \cdots, R_{m-1}$ using both $\topjoin(R_i)$ (giving the value of $A_{i-1}$) and $\botjoin(R_{i+1})$ (giving the value of $A_i$) that gives the maximum change in the size of the result. The maximum over all these tuples gives the tuple $t^*$ with the local sensitivity. 
\revm{Note that finding the max in any of these relations can be done in $O(n_i)$ time, taking $O(n)$ time in total.}

}

Figure \ref{fig:path} illustrates  Algorithm \ref{algo:ls_pathquery} for the toy example $\qpeg(A, B, C, D, E)$. %Suppose we want to compute topjoins and botjoins related to $\R{2}$ and get the most sensitive tuple from $\R{2}$. 
The table $\topjoin(\R{2})$ from the figure with attributes (B, cnt) shows the topjoin of $\R{2}$ by $\groupbyagg{B}(\R{1})$. To prepare botjoin of $\R{3}$, we need to first compute the botjoin of $\R{4}$ as $\groupbyagg{D}(\R{4})$ and then make a join with $\R{3}$ as $\groupbyagg{C}(\superjoin(\botjoin(\R{4}), \R{3})$, as shown by tables $\botjoin(\R{3})$ and $\botjoin(\R{4})$. Finally, we combine $\topjoin(\R{2})$ and $\botjoin(\R{3})$ together to get the frequency table $T^2$ through $\pi_{B, C, (\cnt \times \cnt) \rightarrow \cnt } \big( \topjoin(\R{2}) \times \botjoin(\R{3})\big)$. Table $T^2$ shows the tuple sensitivity of (b1, c1) from $\R{2}$ as 4, which is the most significant tuple sensitivity since others are all zero. We store this tuple as a candidate and repeat the procedure for each relation and the most sensitive tuple is selected from all candidates. Note that each topjoin or botjoin is computed only once.
  With the analysis of algorithm \ref{algo:ls_pathquery}, we have the following theorem for path join queries:

\cut{
\begin{align*}
\topjoin(\R{i}) = \aggregate{A_{i-1}}{sum(\cnt{}{i-2}) \as \cnt{}{i-1}}{\topjoin(\R{i-1}) \bowtie \relation_{i-1}}
\end{align*}
The correctness follows from replacing $\topjoin(\R{i-1})$ by the definition of topjoin as equation (\ref{eq:pj_topjoin}) shows, and proving by induction.


To prepare botjoin, we follow a similar way as preparing topjoin does.

To combine topjoin and botjoin together and find the most sensitive tuple, we need to construct $\Qpfreq^i(\attributes_\database)$ on top of $\topjoin(\R{i})$ and $\botjoin(\R{i+1})$ as equation (\ref{eq:pj_fast_freq}) shows. Notice that the next step as equation (\ref{eq:general_most_sensitive_tuple}) shows is to choose the tuple from $\Qpfreq^i(\attributes_\database)$ that has the maximum $(\cnt{}{i-1} * \cnt{}{i}) \rightarrow c$. Since $\max(\cnt{}{i-1} * \cnt{}{i}) = \max(\cnt{}{i-1}) * \max(\cnt{}{i})$, we construct two tuples to find the maximum count as lines 14 and 15 shows, and combine together as lines 16 and 17 shows. Lines 10 to 12 are for corner cases. At the end, lines 19 to 21 extract the most sensitive tuple and corresponding sensitivity.
}


\begin{theorem}\label{thm:path}

 Algorithm~\ref{algo:ls_pathquery} solves the sensitivity problem and finds the most sensitive tuple for path join queries. The time complexity is \revm{$O(n \log n)$} where $n$ is the size of the database instance irrespective of the size of the output. 
\end{theorem}

However, the above theorem is not generalizable to even all acyclic queries (recall Theorem~\ref{thm:combined-nphard}). In the next section, we give algorithms that can handle acyclic CQs in parameterized polynomial time and run in sub-quadratic time for a class called `doubly acyclic queries' that generalizes path queries.

\cut{
\am{Can you use the term "sensitivity problem".}
\begin{proof}
	We first prove the time complexity of computing topjoin $\topjoin$ and botjoin $\botjoin$ for all tables is $O(m n \log n)$. For bases cases, there is a single group by query, so it takes $O(n \log n)$ time. For analyzing one step of the iteration, the time complexity only depends on the data size of the subroutine, not its running time. For topjoin or botjoin, they both join a relation to the subroutine on the primary key of the size $n$, so it takes $O(n)$ and outputs a $O(n)$ temporary table. The further group by query takes $O(n \log n)$ time. In total, it takes $O(n \log n)$ time. Since we need to compute topjoin and botjoin for $m$ relations, the total time is $O(m n \log n)$.
	
	Next, we show that the time complexity of selecting most sensitive tuple is $O(mn)$. For each relation, we do at most 2 aggregation query as finding the max frequency from related topjoin or botjoin, which takes $O(n)$ time. This is repeated for $m$ relations, so the total time complexity is $O(mn)$. 
	
	Combining together, the total time complexity is $O(mn \log n)$.
\end{proof}
}








==> proof_ls_correctness.tex <==
The local sensitivity of a counting query is defined as the upper bound of the maximum row change of the table when adding or removing one tuple. As discussed above, we only need to consider adding one tuple. Define freq(R, A, a) as the frequency of the tuple in the table "R" that the attribute "A" equals to "a". For example, freq(student, gpa, 3.7) means the number of students that has gpa as 3.7. The definition of "freq" in the form of relation algebra is:

\begin{eqnarray}
freq(R, A, a) &=& \pi_C(\sigma_{A=a}(A~\mathbf{G}~count(*) ~ as ~ C ~ (R)))
\end{eqnarray}

Without the loss of generosity, we assume adding one tuple ($\Al{i} = a_{i-1}$, $\Ar{i}=a_{i+1}$) or simply as ($a_{i-1}$, $a_{i+1}$) to the table $R_i$. The path join can be rewritten as:

\begin{align*}
  &[\R{1},\dots,\R{k}]\\
=~&[\R{1},\dots,\R{i-1}]~::~\R{i}~::~[\R{i+1},\dots,\R{k}]\\
=~&[\R{1},\dots,\R{i-1}]\pjoin{i-1}{i}\R{i}\pjoin{i}{i+1}[\R{i+1},\dots,\R{k}]
\end{align*}

The proof is divided into three cases:

Case 1: $i \in [2, k-1]$

The join operation can magnify the little change in one table. The number of new tuples in the entire join result introduced by the tuple ($a_{i-1}$, $a_{i+1}$) in table $R_i$ is:

\begin{align*}
	\#~of~new~tuples &=&&~\\
		&&& freq([\R{1},\dots,\R{i-1}], \Ar{i-1}, a_{i-1})\\
		&&& * freq([\R{i+1},\dots,\R{k}], \Al{i+1}, a_{i+1})\\
		&=&&\pi_C(\sigma_{\Ar{i-1}=a_{i-1}}(\prejoin([\R{1},\dots,\R{i-1}])))\\
		&&&*\pi_C(\sigma_{\Al{i+1}=a_{i+1}}(\postjoin([\R{i+1},\dots,\R{k}])))\\
		&\leq&& \max_C \prejoin([\R{1},\dots,\R{i-1}])\\
		&&&*  \max_C \postjoin([\R{i+1},\dots,\R{k}])
\end{align*}

Case 2: $i = 1$
\begin{align*}
	\#~of~new~tuples &=&&~\\
		&&& freq([\R{2},\dots,\R{k}], \Al{2}, a_{2})\\
		&=&&\pi_C(\sigma_{\Al{2}=a_{2}}(\prejoin([\R{2},\dots,\R{k}])))\\
		&\leq&& \max_C \postjoin([\R{2},\dots,\R{k}])
\end{align*}

Case 2: $i = k$
\begin{align*}
	\#~of~new~tuples &=&&~\\
		&&& freq([\R{1},\dots,\R{k-1}], \Ar{k-1}, a_{k-1})\\
		&=&&\pi_C(\sigma_{\Ar{k-1}=a_{k-1}}(\prejoin([\R{1},\dots,\R{k-1}])))\\
		&\leq&& \max_C \prejoin([\R{1},\dots,\R{k-1}])
\end{align*}

In conclusion, the upper bound of the number of changes to the transformation is the maximum bound from all cases. Thus, equation~\ref{equation:LSq} holds.


==> recycle_bin.tex <==
If not specified otherwise, the queries that we discuss in the following sections only include the class of join queries with equi-joins. We also assume the database $\database$ contains multiple tables. 
\note{m tables, n tuples, k attributes}

Given a query $q$ and an attribute $A$ from the table $S$, we denote the full domain of this attribute as $\domain^A$.   If the context is clear, we drop $A$ and simply denote as $\domain$. If there are multiple attributes $\attributes = A_1 \ldots A_k$, we define the full domain as $\domain^\attributes = \domain^{A_1} \times \ldots \times \domain^{A_k}$. Specially, we denote $\attributes_i$ as all attributes in the schema of the table $S$. 

\note{$\domain^{A_i}$ or $\domain_i$ ? The photo is blurred}

Given a tuple $t$ from the table $\relation_i$, we define the frequency $f$ of the value $t[\attributes]$ \note{What is t[A]} as 
$$\freq{t[\attributes]} =  | \{r \in S \mid r[\attributes] = t[\attributes]\} | $$


We say that a tuple $t$ is in the active domain if and only if $t[\attributes_S]$ is in its active domain $\actdomain^{\attributes_S}$. Otherwise, it is in the idle domain $\idldomain^{\attributes_S}$. We can get the following corollary immediately:

\begin{corollary}
If $t$ is in the idle domain, $\dtsens = 0$ 
\end{corollary}
\begin{proof}
Since $t$ doesn't exist in the table, $q(\database \setminus \{t\}) = q(\database)$
\end{proof}


We are interested in knowing tuple sensitivities for all tuples, which is important in many cases. For example, to compute the local sensitivity of a query, we can find the maximum tuple sensitivity as the solution. However, if the full domain is unbounded, it is impossible to check the tuple sensitivity for each tuple. Previous research \note{I'm not sure} addressed this problem by only considering tuples in the active domain, which is not correct. We will analyze the tuple sensitivity in the full domain and show that there is a representative subset of the full domain which is bounded. 

\note{I don't know how to use this hardness to prove that compute $LS(q)$ is NP-hard. Shall we prove a more general theorem? Like, given a threshold t, check whether $LS(q) > t$ is NP-hard. \href{http://www.vldb.org/pvldb/1/1453949.pdf}{See this 2008 VLDB paper} 
One idea is, if computing $LS(q)$ is not NP-hard, then deciding $LS(q)$ is no NP-hard. So computing $LS(q)$ is NP-hard.
}

\section{Path Join Query}

\note{1. new notations. 2. represent the algortithm (pseudo). 3. Correctness 4. Efficiency and the theorem.}

\todo{Add an example for the path join}

\note{Use a simpler notation with one attribute for the join.}

A path join query joins a sequence of tables in the database, denoted by
\[\Qpjoin(R_1,\ldots,R_m) = R_1 \pjoin{1}{2} R_2 \ldots \pjoin{k-1}{k} R_m,\]
where $\mathbf{A}_{i}$ represents the attribute set of relation $R_i$. $\Ar{i}$ is the set of attributes in $\mathbf{A}_i$ that are used for the join between $\R{i}$ and $\R{i+1}$. Similarly, $\Al{i}$ is the set of attributes in $\mathbf{A}_i$ that are used for the join between $\R{i-1}$ and $\R{i}$.

We present an efficient representation and computation for the local sensitivity of a path join query, and the corresponding most sensitive tuple.

\subsubsection{Invariant Definition}
We first introduce two key invariants for the representation of local sensitivity.
\begin{align}
\topjoin(\R{i}) &=  \aggregate{\Ar{i-1}}{count(*) ~ as ~ \cnt{r}{i}}{\Qpjoin(\R{1}, \ldots, \R{i-1})} \\
\botjoin(\R{i}) &=  \aggregate{\Al{i}}{count(*) ~ as ~ \cnt{l}{i}}{\Qpjoin(\R{i}, \ldots, \R{m})}
\end{align}

\subsubsection{Computing Tuple Sensitivities}

To find the tuple of maximum tuple sensitivity, for each table $S$, we will create a table $\RTS{i}$ to track the tuple sensitivity for each representative tuple from $\reprdomain^{\attributes_S}$. The schema of $\RTS{i}$ is composed of at most two attributes: $\Ar{i}$ and $\Al{i}$, and one sensitivity attribute: $\tsens_i$. Other attributes from the original table are not included in $\RTS{i}$, since their values can be arbitrary. 

We construct the instance of $\RTS{i}$ as follows:
\begin{align}
\RTS{i} = 
\begin{cases}
\pi_{\Ar{i-1} \as \Al{i},~ \Al{i+1} \as \Ar{i},~ C_{i-1}^r * C_{i+1}^l \as  \tsens_i } \\
\big( \topjoin(\R{i}), \botjoin(\R{i+1}) \big) &, 1 < i < m \\
\pi_{\Al{i+1} \as \Ar{i}, C_{i+1}^l \as  \tsens_i} \botjoin(\R{i+1}) &, i = 1 \\
\pi_{\Ar{i-1} \as \Al{i}, C_{i-1}^r \as  \tsens_i} \topjoin(\R{i}) &, i = m 
\end{cases}
\end{align}

For each table $R_i$, the most sensitive tuple $t^*_i$ can be retrieved from $\RTS{i}$:
\begin{align}
t^*_i = \argmax_{t \in \RTS{i}} ~ t[\tsens_i] 
\end{align}
, whose attributes other than $\Ar{i}$ or $\Al{i}$ could be arbitrary.

The most sensitive tuple $t^*$ is thus the max among all table-wise most sensitive tuples:
\begin{align}
t^* = \argmax_{i} ~ t^*_i[\tsens_i]
\end{align}

The local sensitivity is correspondingly to be $t^*[\tsens]$

\subsubsection{Correctness Analysis}

\begin{theorem}
$\RTS{i}$ covers tuples from the representative domain $\reprdomain^{\attributes_{R_i}}$
\end{theorem}

\begin{proof}
The cross product of $\topjoin(R_{i-1})$ and $\botjoin(R_{i+1})$ includes all tuples from $\Ar{i-1} \times \Al{i+1}$, each of which is the representative domain about $\R{i}$. Since $\RTS{i}$ implicitly allow the domain of missing attributes to be full, these tuples cover $\reprdomain^{\attributes_{R_i}}$. The case is similar for  i = 1 or m.
\end{proof}

\begin{theorem}
$\RTS{i}$ computes the correct tuple sensitivity for each tuple.
\end{theorem}

\begin{proof} Rewrite the entire path join query $\Qpjoin(\R{1},\ldots,\R{m})$ as 
$$\Qpjoin(\R{1},\ldots,\R{i-1}) \pjoin{i-1}{i} \R{i} \pjoin{i}{i+1} \Qpjoin(\R{i+1},\ldots,\R{m})$$

so the change of a given tuple $t$ from $\R{i}$ can be expressed as:
$$\Qpjoin(\R{1},\ldots,\R{i-1}) \pjoin{i-1}{i} t \pjoin{i}{i+1} \Qpjoin(\R{i+1},\ldots,\R{m})$$

the change of join size can be expressed as 
\begin{align*}
\aggregate{\Ar{i-1}}{count(*) ~ as ~ \cnt{r}{i}}{\Qpjoin(\R{1}, \ldots, \R{i-1})} \pjoin{i-1}{i} t \\ \pjoin{i}{i+1} \aggregate{\Al{i}}{count(*) ~ as ~ \cnt{l}{i}}{\Qpjoin(\R{i+1}, \ldots, \R{m})}    
\end{align*}
, which is
$$\topjoin(\R{i})  \pjoin{i-1}{i} t \pjoin{i}{i+1} \botjoin(\R{i+1})$$

\end{proof}

\subsubsection{Efficiency Analysis}
The naive way to compute $\topjoin$ and $\botjoin$ is of linear time to the join size, which would be exponential to the query size and data size. However, since we have a group by clause, we can speed up by a recursive computation.

Rewrite $\topjoin$ and $\botjoin$ in a recursive way:
\begin{align}
\topjoin(\R{i}) =
\begin{cases}
    \aggregate{\Ar{i}}{sum(C^r_{i-1}) \as C_{i}^r }{}\\
    \quad \topjoin(\R{i-1}) \underset{\Ar{i-1}=\Al{i}}{\rightouterjoin} \R{i} &, i > 1 \\
    \aggregate{\Ar{i}}{count(*) ~ as ~ \cnt{r}{i}}{\R{i}} &, i = 1
\end{cases}
\end{align}
\begin{align}
\botjoin(\R{i}) =
\begin{cases}
    \aggregate{\Al{i}}{sum(C^l_{i+1}) \as C_{i}^l }{} \\
    {\quad \R{i} \underset{\Ar{i}=\Al{i+1}}{\leftouterjoin}  \botjoin(\R{i+1}) } &, i < m \\
    \aggregate{\Al{i}}{count(*) ~ as ~ \cnt{l}{i}}{\R{i}} &, i = m
\end{cases}
\end{align}

Note that for left or right outer join, if it joins a NULL attribute, we change the corresponding counting attribute $C$ by default as 0.

\begin{theorem}
The recursive $\topjoin$ and $\botjoin$ satisfy their invariant definitions, and the time complexity is $O(n \log n)$.
\end{theorem}

\begin{proof} (sketch)
It is an special case of the acyclic join. See the theorem in the next section.
\end{proof}

To compute $\RTS{i}$, since there is a cross product, the time complexity is quadratic to the size of $\actdomain$. However, to compute the most sensitive tuple, we don't need to know the entire $\RTS{i}$. We will show a faster way, which is linear in the size of $\actdomain$, to find the most sensitive tuple. 

Let 

$$t^{r*}_i = \argmax_{t \in \topjoin(\R{i})} t[C_{i}^{r}], \quad
t^{l*}_i = \argmax_{t \in \botjoin(\R{i})} t[C_{i}^{l}]$$

, then we have
\begin{align}
    t^*_i = 
\begin{cases}
\pi_{\Ar{i-1} \as \Al{i},~ \Al{i+1} \as \Ar{i}, \\
\quad C_{i-1}^r * C_{i+1}^l \as  \tsens_i }\big( t^{r*}_{i-1}, t^{l*}_{i+1}  \big) &, 1 < i < m \\
\pi_{\Al{i+1} \as \Ar{i}, C_{i+1}^l \as  \tsens_i} (t^{l*}_{i+1}) &, i = 1 \\
\pi_{\Ar{i-1} \as \Al{i}, C_{i-1}^r \as  \tsens_i} (t^{r*}_{i-1}) &, i = m 
\end{cases}
\end{align}

The correctness follows from the definition of $\RTS{i}$ and $t^*_i$. To find the maximum of $C^r_{i-1} * C^l_{i+1}$, it is equivalent to find the maximum of $C^r_{i-1}$ and $C^l_{i+1}$ separately since both are independent.

\begin{theorem}
The time complexity to find the most sensitive tuple and the local sensitivity of a path join query is $O(mn \log n)$.
\end{theorem}

\begin{proof}
Since there are $m$ $\topjoin$ and $\botjoin$ to compute, it takes $O(mn \log n)$. To find $t^*_i$, it takes another $O(mn)$ time. In conclusion, the time complexity is $O(mn \log n)$.
\end{proof}

\begin{figure}[t]
	\begin{center}
		\includegraphics[width=0.8\linewidth, trim=0 460 0 0, clip]{{"figures/Path Join Example"}.pdf}
		\caption{$\Qpjoin(\attributes_\database) \datalogEQ \relation_1(A,B), \relation_2(B,C), \relation_3(C,D), \relation_4(D,El)$}
		\label{default}
	\end{center}
	\begin{center}
		\includegraphics[width=0.8\linewidth, trim=0 290 0 170, clip]{{"figures/Path Join Example"}.pdf}
		\caption{$\Qpjoin^2(\attributes_\database)$}
		\label{default}
	\end{center}
	\begin{center}
		\includegraphics[width=0.8\linewidth, trim=0 180 0 350, clip]{{"figures/Path Join Example"}.pdf}
		\caption{$\topjoin(\relation_2)$, $\botjoin(\relation_3)$, $\botjoin(\relation_4)$}
		\label{default}
	\end{center}
	\begin{center}
		\includegraphics[width=0.8\linewidth, trim=0 0 0 460, clip]{{"figures/Path Join Example"}.pdf}
		\caption{$\Qfreq^2(\attributes_\database)$}
		\label{default}
	\end{center}
\end{figure}


\todo{Finish the draft}

\note{\\General conjunctive join query \\ $\rightarrow$ hypertree \\ $\rightarrow$ double acyclic hypertree}

or

\note{\\acyclic join \\$\rightarrow$ double acyclic join}

\todo{equivalence: correctness}

\todo{discuss efficiency}

In the previous section, we have shown how to compute topjoin and botjoin efficiently in polynomial time combined complexity. However, for step 2, there is no guarantee that this sub query can be computed by an algorithm in polynomial time combined complexity.

\note{Definition} Here we introduce a sub class of the acyclic join query class: double acyclic join queries. For an acyclic join query $\Qajoin(\attributes_\database)$, if removing one relation from the query body and the remaining query $\Qajoin^i(\attributes_\database)$ is still an acyclic join query, we call this query as a double acyclic join query.

\note{Efficiency} Since it is double acyclic, we can find a query plan to compute step 2 in polynomial time combined complexity. 

\note{We argue that for a double acyclic join query, any acyclic join tree is also a double acyclic join tree.}

The efficiency can be further boosted by propagating the max operator in step 3 to step 2. We leave this as the future work.

\begin{theorem}
	For double acyclic join queries, algorithm~\ref{algo:as_pathquery} computes the local sensitivity of a path join query and also  finds the corresponding most sensitive tuple. The time complexity is $O(mn \log n)$ where $m = $ the number of attributes and $n = |D|$.
\end{theorem}


==> responses.tex <==
\twocolumn
\section*{Response Letter for Paper 609: ``Computing Local Sensitivities of Counting Queries with Joins''}\label{sec:response}
We thank the reviewers for the revision opportunity and their valuable comments. We have addressed all comments and revised the paper significantly according to reviewers' suggestions as described in detail below. Updates made in response to specific
comments are color coded as follows. 
%In addition, we have improved the general presentation of the paper that we have not highlighted.
\begin{itemize}
	\itemsep0em
	\item \revm{General improvement and common changes for multiple reviewers are in BLUE.}
	\item \reva{Reviewer 1 in RED.}
	\item \revb{Reviewer 2 in GREEN.}
	\item \revc{Reviewer 4 in MAGENTA}. 
\end{itemize}

%{The paper is appended after the response letter starting page number 5, and the section/table/figure references can be clicked in the responses to reach the corresponding changes in the main paper.}

We use R1-W1 to denote the first weak point from Reviewer 1 and so on. 
%Reviewers' comments are in italics. 
The letter is divided into two parts: (1) A summary of changes, and (2) detailed responses to all reviewers.


\eat{
\section*{Meta Review Comments}
%(We copy the comments for required changes for easy reference).
\begin{itemize}[leftmargin=*]
\itemsep0em
	\item \textbf{(R1):} \ques{Based on the \#R1/D3 comment, it would be nice to either see such a support or see some comments with respect to the limitations/effort to support more general data-flow processing systems.} \\
	\revm{We have implemented \proto\ in Presto (version 0.216). It primarily required instrumentation to periodically collect resource consumption metrics from each DriverContext. {\bf The complete details are given in Section~\ref{subsec:discussion} and Appendix~\ref{sec:app_presto}.}}
	
	
		
\end{itemize}
\par 
}


\section*{Summary of changes}
\revm{
\begin{enumerate}
\setlength\itemsep{0.5em}
        \item {\bf We have updated the experiments section significantly as follows}:
        \begin{itemize}
            \item \textbf{Experiments on real world datasets and non PK-FK join queries: \cut{(R1-W2, R1-W3, R1-D6. R1-R1, R2-D3, R2-R1, R4-D14):}}
            We added a new dataset from SNAP, the ego network of Facebook, and prepared a triangle query $\qtri$, a 4-path query $\qpath$, a 4-cycle query $\qcycle$ and a star join query $\qstar$. The experiment results show that the sensitivity bound improvement of \TSens ranges from $\times 3$ to $\times 80k$, and \TSensDP achieves $< 6 \%$ error for the triangle, 4-path and cycle queries while \PrivSQL get $> 100\%$ error for the 4-cycle and star queries. Unlike TPC-H, the Facebook dataset has tuples with skewed join multiplicities and the queries are not FK-joins. 
        
            
    \item \textbf{Experiments on the effects of the tuple sensitivity upper bound $\ell$ to the performance of \\
    \TSensDP:
    %(R2-D2):
    } We added an experiment about changing $\ell$ at the end of Section \ref{sec:exp_dp}. As $\ell$ increases, the noise of $\hat{\CQ}$ in the $SVT$ routine get larger. This causes the learned tuple sensitivity threshold to deviate more from the local sensitivity, which is considered the optimal threshold by the rule of thumb. When $\ell$ is too small, the learned tuple sensitivity threshold could also be small, which increases the bias.
    
        \end{itemize}
   
        
    \item \textbf{We extended discussion on the comparison with Yannakakis's algorithm. 
    %(R1-W1, R1-D1, R1-D4, R1-R2).
    }  This is in Sections 4.2 and 5.2.
    %Please see the detailed response for R1. 
    
    \cut{
    We added discussions in Section~     %\ref{sec:pj_simple_ineffi}, 
    \ref{sec:pj_effi} and Section~\ref{sec:general-algo} 
    to clarify how our algorithms are inspired from Yannakakis's algorithm and what is the difference between them. We borrow the idea of tracking multiplicity tables from Yannakakis's algorithm, but we also support tracking multiplicity tables for the joins of the complementary tree, which is not included in the work "Scalable computation of acyclic joins [A Pagh, R Pagh PODS 2006]". We also discussed the challenge if we repeat evaluating the query after adding or removing a tuple by Yannakakis's algorithm which could result in exponential time complexity in combined complexity. While evaluating the size of acyclic queries is not NP-hard, it is NP-hard to evaluate the local sensitivity of acyclic queries shown by Theorem~\ref{thm:combined-nphard} and our Algorithm \ref{algo:gj_query} gives a $\tilde{O}(mn^d)$ solution. \am{Sudeepa: Please make a pass.}
    }
    
    \item \textbf{We extended discussion on the future work and extensions.}
    %(R1-W4, R2-W3, R2-R3):} 
In Section \ref{sec:extensions}, we discuss extensions to \TSens that include selection operators, disconnected join trees, and general joins. The extension to general non-acyclic queries has been implemented (see queries $q_3$, $\qtri$ and $\qcycle$ in Section~\ref{sec:experiments}). Moreover, we added a discussion on efficient approximations (R2-R3) and self joins (R2-W3).
    


    \item \textbf{We have revised the presentation of the paper significantly to improve its readability.} The specific changes are mentioned in response to individual reviewer's  comments. 
    
    
    \cut{
    We have made the following changes to the paper:
    
    
    \begin{itemize}
        \item  \textbf{(R1-D2,D3,D5; R2-W1,R2,...\todo{update the list}) } Clarified definitions and intuitions: (i) definition for ``counting queries'' in Section 2, Definition 2.1 and 2.2, representative domain in Definition 3.1; (ii) NP-hardness for acylic queries in Theorem 3.2; (iii) bag semantics for our algorithms; (iii) examples for DP; (iv) description of GYO decomposition; (iv) intuitions for ``incoming'' and ``outgoing'' paths in Section 4.1 with examples; .... 
        \item \textbf{(R2-W2)} Added discussion for the scalability issue at Section 7.2 .....
        \item \textbf{(R4-D4,D5)} Shortened the proofs of Theorem 3.1 and 3.2 and other texts due to space constraint.
    \end{itemize}
    
    \todo{Reorganize the points below to the above template.}
    
    %\eat{
    \begin{itemize}
    \setlength\itemsep{0.2em}
        \item \textbf{(R1-D2)} We clarified the definition of "counting queries" in Section \ref{sec:prelim}
        \item \textbf{(R1-D3)} We clarified that the NP-hardness also holds for acyclic queries.
        \item \textbf{(R1-D5, R1-author-feedback, R4-D6)} We clarified in the preliminary section (Section \ref{sec:prelim}) that our algorithms work with bag semantics, not set semantics. 
        \item \textbf{(R2-W1, R2-R2)} \todo{An example in intro about DP }
        \item \textbf{(R2-W2)} We added a discussion about the scalability issue at Section \ref{sec:exp_ls}.
        %\item \textbf{(R2-D1)} We fixed typos in Section \ref{sec:general-alg} and \ref{sec:exp_ls}.
        \item \textbf{(R4-W3)} We added more descriptions of DP in Section \ref{subsec:dp} and simplified the discussion.
        \item \textbf{(R4-D1)} We clarified the definition of adding or removing a tuple t in Definition \ref{def:tuple_sens} and \ref{def:local_sens}.
        \item \textbf{(R4-D2)} We added a description of GYO decomposition steps in \ref{fig:gyo} 
        \item \textbf{(R4-D3)} We clarified the definition of the representative domain in Definition \ref{def:repr}.
        \item \textbf{(R4-D4)} We shortened the proof of Theorem \ref{thm:poly-data-complexity}.
        \item \textbf{(R4-D5)}  We shortened the proof of Theorem \ref{thm:combined-nphard}
        \item \textbf{(R4-D7)} We added the intuition about "incoming" and "outgoing" paths in Section \ref{sec:pj_simple_ineffi}.
        \item \textbf{(R4-D8)} We illustrated in Section \ref{sec:pj_simple_ineffi} that the algorithm hardness is from adding tuples. 
        \item \textbf{(R4-D9)} We added the transformation step in Figure \ref{fig:path}.
        \item \textbf{(R4-D11)} We added the intuition in Section \ref{sec:general-approach}.
        \item \textbf{(R4-D12)} We illustrated the iterative step of topjoin in the description of Figure \ref{fig:gj_notations}.
        \item \textbf{(R4-D13)} We rewrote Section \ref{sec:extensions} to clarify extensions.
        \item \textbf{(other)} The time complexity in Theorem \ref{thm:path} is updated from $O(m n \log n)$ to $O(n \log n)$, which is tighter.
        \item \textbf{(other)} The time complexity in Theorem \ref{thm:path} is updated from $O(m ~d~ n^{d+1}~\log n)$to $O(m ~d~ n^{d}~\log n)$ as a typo fix. 
    \end{itemize}
    }
    %}
\end{enumerate}
}
%\section*{Individual Reviewer Comments}

%\section*{{\color{red} {Reviewer 1}}}
%\vspace{2mm}
\section*{Meta-review}

\ques{The reviewers have discussed and considered the author feedback and would like to provide an opportunity for revision. Please apply the revisions you suggest in the feedback and address the review concerns.}

\revm{All comments have been addressed as discussed below.}

\section*{Reviewer 1}


\noindent
\reva{{\bf {\large Comparison with Yannakakis's algorithm and bag. vs. set semantics:}}}\\

\textbf{(R1-W1)}. \ques{Straightforward algorithms with nothing interesting happening on a technical level. This is not to say that the proposed ideas are not useful, but the results follow from folklore use of Yannakakis algorithm for computing the full join size in linear time of full CQs.}

\textbf{(R1-D1)}. \ques{In its present form, the paper is more suitable for a short paper rather than a full paper. This was a very easy paper to review (aided by the excellent writing and formal presentation of the results). The authors have done a good job of identifying a nice problem and present decent algorithmic results but they are very straightforward with not much going on technically (elaborated in great detail below). But since the problem is important and leads to real world impact, it is worth announcing it to wider community.} %\xh{Do we need to include this point? It is a positive point}

\textbf{(R1-D4)}. \ques{Section 4 contains the core algorithmic contribution of the paper. The authors provide intuition on how they can solve the problem for path queries. Once the algorithm is established, it can be extending to arbitrary join trees (at the cost of some blowup in running time due to branching in the tree which is unavoidable). The topjoin and botjoin in section 4.2 is using (a trivial extension of) Yannakakis algorithm. Although [35] talks about how to evaluate Q(D) in time O(IN + OUT), the same algorithm is also used for semijoin reduction, eliminating dangling tuples and calculating the |Q(D)| in O(IN) time -- these are folklore applications of results in [35] and full reducers since they are a straightforward (if not trivial) extension of the algorithm. A (incomplete) list of references that use [35] in the way described above is added below.

Scalable computation of acyclic joins [A Pagh, R Pagh PODS 2006] -- see section 4 and section 5.2 that talks about computing join sizes very similar to how topjoin / botjoin work. I believe that topjoin / botjoin are a simple modification of the ideas here.
DunceCap: Compiling Worst-Case Optimal Query Plans [Perelman, Re SIGMOD 2015] -- section 1.1 talks about full reducers.

I would like to see the authors acknowledge that their algorithms are based on [35]. I also think that section 4.1 is not required at all -- the first thought on how to compute the change in query output by adding / deleting a tuple is to use Yannakakis style algorithm for acyclic queries. }


%\textbf{(R1-after feedback)} \ques{After reading the author feedback, it is clear that the observation in D5 holds for set semantics, and not the bag semantics that the authors consider. This should be made clear by the authors.}


\textbf{(R1-R2)}. \ques{Mention that the algorithms are based on [35] and full reducers.\\}

%\reva{Although we borrowed the idea from Yanakakis's algorithm about how to compute tuple counts efficiently, we don't use Yannakakis algorithm to compute the full join size and repeat it for all possible adding or removing tuples.  \\}

\reva{Please see the new discussions comparing with Yannakakis's algorithm at the end of Section~\ref{sec:pj_effi} (after Theorem~\ref{thm:path}) and in  Section~\ref{sec:general-algo} (after Theorem~\ref{thm:gj_query}).
\par
As mentioned in the feedback letter, our algorithms for computing multiplicity tables (topjoins and botjoins) are indeed inspired by Yannakakis's algorithm~\cite{Yannakakis:1981}, and we have made the comparisons clearer. Also thank you for pointing out that a simple variation of Yannakakis's algorithm \cite{Yannakakis:1981} tracks the tuple counts in one pass and can compute the size of acyclic join in $\tilde{O}(n)$ time, where $n$ is the total data size. 

\textbf{More discussions:} For path join query, we make two passes and store the intermediate topjoins and botjoins in Algorithm~\ref{algo:ls_pathquery} and hence have a similar computation complexity. We clarified the complexity in Theorem~\ref{thm:path}. On the other hand, query evaluation and sensitivity computation have a separation for general acyclic join queries. Computing the join size for acyclic join queries can be done in polynomial time in combined complexity, but it is NP-hard to find the maximum join size change (Theorem~\ref{thm:combined-nphard}). The first pass of Algorithm~\ref{algo:gj_query} computes the botjoins tables in a similar way as Yannakakis's algorithm and the work "Scalable computation of acyclic joins [A Pagh, R Pagh PODS 2006], but the second pass of the algorithm for computing the topjoin tables still requires joins of multiple tables instead of simply removing the dangling tuples from the first pass. In addition, we give a parameterized polynomial time analysis for Algorithm \ref{algo:gj_query}), which is $\tilde{O}(m n^d)$. Here $m$ is the number of relations and $d$ is the join tree degree. We also find a class of queries, doubly acyclic join queries, that Algorithm \ref{algo:gj_query} can run in polynomial time in combined complexity. 

We replace the simple and inefficient algorithm in Section~\ref{sec:pj_simple_ineffi} by an intuition to our efficient algorithm. In our evaluation (Section~\ref{sec:exp_ls}), we also discuss a naive baseline for sensitivity computation which applies Yannakakis's algorithm to evaluate query on all possible databases formed by adding or removing a tuple, but we need to check tuples from the full representative domain of size  (Definition~\ref{def:repr}) instead of active domain alone. As the full domain size is large (above 10k) for all the queries, this approach will take $\times 10k+$ time than our algorithm \TSens. \\
}

%\reva{To compute the local sensitivity, we can also naively apply existing efficient query evaluation algorithms, such as Yannakakis's algorithm \cite{Yannakakis:1981}, to evaluate the given query on all possible databases formed by adding or removing a tuple from the representative domain instead of the full domain. However, the representative domain can still be large and result in an inefficient algorithm. Next we will show the sensitivity problem is NP-hard in combined complexity even for acyclic queries. }


%\reva{We borrow the idea of tracking multiplicity tables from Yannakakis's algorithm, but we also support tracking multiplicity tables for the joins of the complementary tree, which is not included in the work "Scalable computation of acyclic joins [A Pagh, R Pagh PODS 2006]". }\\

%\reva{What's more, Yannakakis's algorithm and related work focus on computing join sizes in $\tilde{O}(n)$ time, but if we consider computing join sizes after all possible tuple insertions and deletions of full CQ joins one at a time, it can be exponential in combined complexity. We avoid this approach and use topjoin and botjoin to store intermediate tuple counts, which are used to summarize all possible join size changes due to adding or removing tuples from the representative domain. Notice that Algorithm \ref{algo:ls_pathquery} for path join queries has the same complexity as just computing the join size, but it takes all possible tuple insertions and deletions into account. \\

%For acyclic queries, although computing the join size can be done in polynomial time in combined complexity, it is NP-hard to find the maximum join size change. We give a parameterized polynomial time solution as Algorithm \ref{algo:gj_query} does, which is $\tilde{O}(m n^d)$ and $d$ is the join tree degree. We also find a class of queries, doubly acyclic join queries, that Algorithm \ref{algo:gj_query} can run in polynomial time in combined complexity. \\

%We added clarifications in Sec \ref{sec:pj_simple_ineffi}, \ref{sec:pj_effi} and \ref{sec:general-algo}

%\note{Mention full reducer}
%}~\\


\textbf{(R1-D5)}. \ques{Section 5 extends topjoin and botjoin to arbitrary acyclic queries (Theorem 5.1). The notion of doubly acyclic join queries is interesting. The most interesting part of this section is the example Q(A,B,C) :- R1(A,B,C), R2(A, B), R3(B,C), R4(C,A). This query is acyclic but since it is not double acyclic the authors argue that superlinear time is required to compute the frequency tables (which is true). But observe that computing local sensitivity when removing one tuple from any of the input relations can be done in constant time once Q(A,B,C) has been computed which takes O(|D|) time. Computing local sensitivity when adding a tuple to R2, R3, R4 is linear time because one can go over the tuples in R1, find all (a,b) valuations that did not participate in the output and then check whether the connecting c's with the fixed (a,b) form a triangle or not -- a linear time operation since the size of R1 is O(|D|). The only hard case that requires the frequency tables is when you want to add a tuple to R1 -- in this case, we need to know if the added tuples will form a triangle or not. But adding something to R1 can only change the local sensitivity by just one. If any of the previous steps give you a local sensitivity greater than one, then you need not even do this step. This means that $n^{3/2}$ time operation can be skipped completely at the cost of assuming that local sensitivity is one (for the case of adding a tuple to R1), that too if any of the other deletion local sensitivities are zero -- an extremely mild loss in utility to avoid expensive computations. I was hoping to see that the authors build on such observations to skip or defer some of the computations but this was not the case. I believe there are other clever observations that can also be made to get a small upper bound on local sensitivity in lesser preprocessing time than computing the frequency tables. I was also disappointed to see no discussion on a gap between the hardness of computing local sensitivity when you delete a tuple from D vs adding a tuple to D.}



\textbf{(R1-author-feedback)} \ques{After reading the author feedback, it is clear that the observation in D5 holds for set semantics, and not the bag semantics that the authors consider. This should be made clear by the authors.}\\

\reva{
Please see the updates in Section~\ref{sec:prelim}, Section~\ref{sec:pj_simple_ineffi}, and at the end of Section~\ref{sec:general-algo}.

(Set vs. bag)~ We clarified in Section~\ref{sec:prelim} and Section~\ref{sec:pj_simple_ineffi} that our algorithms work with bag semantics, and thus duplicates are not eliminated. Therefore, adding a tuple to a relation may lead to a large change in the query output, e.g. the product of the multiplicities of the edges forming the triangle. In Section~\ref{sec:general-algo} after giving the example for a hard query, we briefly discussed the intuition, but could not discuss the nice example given by the reviewer in detail due to space constraints.

(Tuple insertion vs. deletion)~ We had discussed the difference between complexities of tuple deletion (called downward tuple sensitivity) and tuple addition (called upward tuple sensitivity) in Section~\ref{sec:poly-data}. We have highlighted it in color for easy reference. 

%\xh{Missing: We added discussion of the gap between the hardness of computing local sensitivity when deleting a tuple from $D$ v.s. adding a tuple to $D$ in Section ~\ref{sec:pj_simple_ineffi}. }

As the reviewer pointed out, there are special cases where we can skip computing the multiplicity tables, such as when some attributes are unique. We believe more rules can be found through the analysis on functional dependencies and foreign-primary key constraints. Due to space constraint, we will leave the discussion to the full version of the paper. \\

}

\eat{
\reva{ D5 shows an interesting case that in set semantics, queries like Q(A,B,C) :- R1(A,B,C), R2(A, B), R3(B,C), R4(C,A) can have a special rule to compute local sensitivity without computing all multiplicity tables. Since set semantics eliminate duplicates, relations like R1 that contains all attributes appearing the query head has a trivial multiplicity table that all tuples has tuple sensitivities at most 1. \\

Our algos work with bag semantics and not set semantics, thus duplicates are not eliminated and D5 doesn't hold in our case. Adding an R1 row may increase the sensitivity by a lot (product of the multiplicities of the edges forming the triangle). This is clarified in Section \ref{sec:prelim}\\

Although D5 doesn't hold in our setting as bag semantics, it is true that there are other interesting observations that can help skip computing the multiplicity tables. We observe that for queries like Q(A,B,C) :- R1(\underline{A}), R2(\underline{B}, A), R3(\underline{C}, B) where underlined attributes are keys, the tuple sensitivities for tuples from R3 is always at most 1, since it can at most join one tuple in R2, and this tuple in R2 can at most join one tuple in R1. We believe more rules can be found through the analysis on functional dependencies and foreign-primary key constraints
%, and we leave the discussion about this work in the future work section
.\\

We also added a discussion in Section \ref{sec:pj_simple_ineffi} to show the hardness of computing local sensitivity is from tuple additions .\\
}
}



\noindent
\reva{{\bf {\Large Experiments:}}}\\

\textbf{(R1-W2)}. \ques{Weak experimental section -- An empirical analysis over just *3* queries to claim better performance over competing systems.}

\textbf{(R1-W3)}. \ques{Experiments only over PK-FK joins (TPC-H) rather than a wide variety of datasets where things are more difficult to do.}

\textbf{(R1-D6)}. \ques{My biggest issue with the paper in its present form is the experimental section. The authors perform experiments on just 3 queries. This is not enough to make an empirical superiority argument at all. Further, the experiments are done on TPC-H pk-fk joins but the algorithms in section 4,5 are not built for PK-FK joins. PK-FK joins make sure that *all* full CQs will have a result <= O(|D|). This means that there is no blow up in join queries at all. This also means that perhaps there are algorithms where you can compute Q(D) since it only requires linear time and design smarter techniques. Indeed, the authors mention in the introduction that their algorithms work "irrespective of the output size." but this may not be the best thing to do if you can compute Q(D) in linear time and then use it for local sensitivity computation. I would like to see more experiments on datasets from say SNAP that lead to large number of triangles or 4-cycles and try more interesting queries like Q(A,B,C) :- R1(A,B,C), R2(A, B), R3(B,C), R4(C,A) to see how the algorithms behave. I do not doubt that botjoin/topjoin will perform well on these but for completeness and confidence in the applicability of the proposed ideas, this needs to be done.}
\textbf{(R1-R1)}. \ques{Add more experiments over different datasets and other queries as outlined in D6.\\}

\reva{We added a new dataset from SNAP, the ego network of Facebook, and prepared a triangle query $\qtri$, a 4-path query $\qpath$, a 4-cycle query $\qcycle$ and a star join query $\qstar$. The experiment results show that the sensitivity bound improvement of \TSens ranges from $\times 3$ to $\times 80k$, and \TSensDP achieves $< 6 \%$ error for the triangle, 4-path and cycle queries while \PrivSQL get $> 100\%$ error for the 4-cycle and star queries. }\\

\noindent
\reva{{\bf {\Large Other comments:}}}\\

\textbf{(R1-D2)}. \ques{The paper title, introduction and definition 6.2, 6.3 talk about "counting queries" but it is not defined formally in the paper. The preliminaries section says "We focus on counting the number of output tuples for the class of full conjunctive queries..." -- so a counting query is a query that returns the size of the full join result i.e |Q(D)|? It seems this is the right definition but I was confused since it is not clarified in the paper.\\}

\reva{We agree with the reviewer that a counting query is a query that returns the size of the full join result i.e |Q(D)|. We clarified the definition of counting query in the preliminary section (Section~\ref{sec:prelim}). \\}

\textbf{(R1-D3)}. \ques{Section 3 is good overall. Theorem 3.2 is not surprising at all given that evaluating Q(D) itself is NP-hard (let alone $|Q(D \cup t)| - |Q(D)|$). Indeed, this is the observation that is exploited in the proof by encoding a SAT instance and distinguishing a zero vs non-zero Q(D).\\}

\reva{We updated Theorem \ref{thm:combined-nphard} to emphasize the observation that while it is not NP-hard to evaluate acyclic queries, it is NP-hard to find local sensitivity of acyclic queries. }
\\


\textbf{(R1-W4)}. \ques{All interesting variants of the problems are deferred to future work.\\}

\reva{We implemented the extension of supporting non-acyclic queries ($q_3$, $\qtri$ and $\qcycle$) in evaluation section (Section~\ref{sec:experiments}).

We extended our discussion in Section~\ref{sec:extensions} on how to support more general queries including selections and self-joins and how to speed up our algorithm by tracking only the top k entries of the multiplicity table. %In particular, self-join requires tracking find-grained tuple provenance. 
%Furthermore, we can skip computing tuple sensitivities if specific functional dependencies exists. 
%These discussions are added at Section \ref{sec:extensions} 
}

%\xh{a line about what have been covered in this paper. a few more lines to summarize future work and link to the new section.}





\section*{Reviewer 2}
\noindent

\textbf{(R2-W1)}. \ques{The only complaint I have about the paper is the introduction Section. It would be better to use a running example based on differential privacy to give the reader a better sense of the problem that you are trying to solve. I know that you have a whole section about the use of your algorithm in DP, but it would be great to have a concrete example early in the introduction.
}

\textbf{(R2-R2)}. \ques{Introduce a running example of differential privacy early in the introduction.} \\

\revb{We reorganized our introduction to first present the challenges and contributions for the local sensitivity problem and then elaborate its relevance to differential privacy application. For differential privacy, we clarified its definition and general approaches to achieve this mechanism in the introduction.  In Section~\ref{subsec:dp}, we reused the running example from Figure~\ref{fig:full_conjunctive} to show the difference between global sensitivity and local sensitivity -- the local sensitivity of the query on the database instance in Figure~\ref{fig:full_conjunctive} is 4 but its global sensitivity can be unbounded. 


Adding a DP example in introduction was somewhat difficult as it needed some concepts to be defined first, therefore, we have added an example of DP in Section~\ref{sec:app_dp} (before Section \ref{subsec:dpalgo}).
} \\
%\note{do we still need an example in intro in DP?}\\

\textbf{(R2-W2)}. \ques{In section 7.2 (Results and Analysis), the authors stated that they didn’t run q3 for a scale larger than 0.1 due to the memory limit issue. I didn't see and discussion as of why this is the case and how limiting this problem to the applicability of their proposed algorithm.}\\

\revb{We have added the following discussion in Section \ref{sec:exp_ls}.
The multiplicity tables for this cyclic query grows nearly quadratically with the input table size. Our future work will extend our algorithm to maintain the top $k$ frequent values instead of all the frequencies which can reduce the intermediate size and further speed up runtime (Section~\ref{sec:extensions}). \\
} 
%\xh{add the discussion here so that reviewer does not have to read the text.}\\

\textbf{(R2-W3)}. \ques{The authors clearly stated that developing an algorithm for finding local sensitivity in queries with self-join is left for future work. But as a reader, I was hoping to see a brief discussion about what needs to be considered for developing such an algorithm.}\\

\revb{We have added the following discussion in Section \ref{sec:extensions} to include the details of a possible solution for supporting acyclic join queries with self-joins and its challenge. 
Acyclic join queries with self-joins can not be captured by our algorithms, because we only allow a relation to appear once in the query. For each relation, we compute the joins for the rest of relations to summarize how tuples from this relation can affect the full join. A possible workaround is to join the repeated base relations as a single and combined relation, run our algorithm, and then link the effect of adding or removing a tuple from the base relation to the combined relation and the effect of adding or removing a tuple from the combined relation to the rest. However, it is challenging to find all possible insertions to the base relation that allows the combined relation to join all possible pairs of "incoming" and "outcoming" path. We defer this line of research to future work. 
}\\
%Basically, it requires a fine-grained tuple provenance that can find all possible tuple insertions that allows the self-join to connect to all possible join paths. \xh{Jut place the discussion from the main text here.}} 



%\note{Should we state the concern for self-joins? e.g., it fails the algorithm because we assume one tuple can only make changes in one atom of the query body.}\\

%\xh{Add a discussion for self-joins: why it is challenging and what is the naive cost by reusing our algorithm.}

\textbf{(R2-D1)}. \ques{Minor typos:
Section 5.2: To prepare $\top(R_i)$, we start with the children of the root note [node].
Section 7.2: "Notice that after scale 0.001, TSens has in [on] average 7x smaller and 6x smaller of the local sensitivity for q1 and q2 then [than] Elastic has.}\\

\revb{We've fixed typos.}\\

\textbf{(R2-D2)}. \ques{In Section 6.2, the authors stated: "Our truncation algorithm assumes an estimated upper bound of tuple sensitivity $\ell$ is given." I would like to see an experiment about the effect of $\ell$ on your TSenDP algorithm.}\\

\revb{We have performed an experiment about changing $\ell$ and included the following discussion at the end of Section \ref{sec:exp_dp}.

 To find how 
%the estimated upper bound of tuple sensitivity 
the upper bound parameter for tuple sensitivity 
$\ell$ affects the performance, we vary $\ell$ through 1, 10, 30, 50, 100, 1000 and repeat \TSensDP 20 times for the star query $\qstar(A,B,C)$ whose true local sensitivity is 13 when $R_2$ is the primary private relation for DP.
%(we only consider adding or removing one tuple from $R_2$ for the DP experiment). 
For each bound, the median global sensitivity, which is also the tuple sensitivity threshold learned from the SVT routine, is [11, 13, 9, 4, 48, 160], the median bias error is [3\%, 1\%, 13\%, 55\%, 0\%, 0\%], and the median relative error is [5\%, 4\%, 17\%, 56\%, 32\%, 98\%]. The optimal $\ell$ in this case is 10, with the corresponding error as 4\%, while the worst error is 98\% when $\ell = 1000$. 

Notice that as $\ell$ increases, the noise added to $\hat{\CQ}$ in the SVT routine gets larger. This causes the learned tuple sensitivity threshold to deviate more from the local sensitivity, which is considered the optimal threshold by the rule of thumb. When $\ell$ is too small, the learned tuple sensitivity threshold could also be small, which increases the bias.
} \\

\textbf{(R2-D3)}. \ques{All experiments used the TPC-H dataset. It would've been great to see how your algorithms performs under different types of datasets.} 

\textbf{(R2-R1)}. \ques{Strengthen your experiments by testing more queries, and involving more real and synthetic datasets to evaluate non-FK joins and skewed distributions } \\

\revb{%Please see the response to R1-D6.
We added a new dataset from SNAP, the ego network of Facebook, and prepared a triangle query $\qtri$, a 4-path query $\qpath$, a 4-cycle query $\qcycle$ and a star join query $\qstar$. The experiment results show that the sensitivity bound improvement of \TSens ranges from $\times 3$ to $\times 80k$, and \TSensDP achieves $< 6 \%$ error for the triangle, 4-path and cycle queries while \PrivSQL get $> 100\%$ error for the 4-cycle and star queries. 
} \\

\textbf{(R2-R3)}. \ques{Please discuss how your algorithms can be extended to improve runtime and query expressibility} \\

%\revb{We added a discussion in Section \ref{sec:extensions}  about keeping top k entries for each multiplicity table 
%and applying rules to skip computing multiplicity tables 
%to improve the runtime, and supporting self-joins to extend query expressibility. Other extensions, including selections, disconnected join trees, and general joins, are also discussed and rewrote in Section \ref{sec:extensions}. 

%\xh{Use the original text from the main body for the top-k entries if it is the first time mentioned. }
%} \\

\revb{We added a discussion in Section \ref{sec:extensions}  about self-joins to extend query expressibility. Other extensions, including selections, disconnected join trees, and general joins, are also discussed and rewrote in Section \ref{sec:extensions}. 

We have also added the following discussion in Section \ref{sec:extensions} to include the details of a possible extension to improve the runtime. We can extend our algorithm to tradeoff accuracy in the sensitivity for better runtime. As our experiment will show, the multiplicity tables that topjoins and botjoins compute can grow quadratically or faster in the input size depending on the query. To make the computation scalable, we can maintain the top $k$ frequent values instead of all the frequencies in the top and botjoins. We can set the frequencies of the rest of the active values in the top and botjoins to the kth largest frequency. This approach gives an upper bound of  tuple sensitivity but can speed up runtime.}

%\xh{Yes, keeping only top-k frequencies can be an extension. For query experessibility, we can add discussion on other aggregates, self-joins. }

\section*{Reviewer 4}
\noindent

\textbf{(R4-W1)} \ques{The paper is poorly written. There are typos in formulas, many general typos, and a lack of intuitive examples and illustrations.}\\

%\revc{We made improvements on writings as stated in the following responses. }\\
\revc{We fixed the typos and added more examples to the paper. 
%: please see new Examples 
}\\

%\xh{List the examples we added to the paper.} }


\textbf{(R4-W2)} \ques{I could not completely follow the discussion about the extension to trees and doubly acyclic queries, but based on my own independent analysis it seems correct.} \\

%\note{What should we respond ?} 
%\xh{Due to space constraint, we cannot add all the details, but we will elaborate them in the full version.  }\\

\revc{Due to space constraint, we cannot add all the details, but we will elaborate them in the full version.} \\


%\note{I'm not sure how to respond R4-W1 and R4-W2}

\textbf{(R4-W3)} \ques{The DP related discussion assumes familiarity with the area and currently would be almost incomprehensible for a broad section of the SIGMOD community.} \\

\revc{We added more descriptions of DP in Section \ref{subsec:dp} so that readers can easily follow without knowing DP before. We explained the difference between local sensitivity and global sensitivity through an example, and simplified the discussion about the challenge of unbounded global sensitivity and existing solutions such as Lipshitz extensions. } \\

\textbf{(R4-D1)} \ques{I did not really understand the difference between local and global sensitivity, maybe because of typos in the formal definitions. Local sensitivity is about adding/removing a single tuple to/from a single relation. Then why does Def 2.1 state that t is drawn from the schema of the join output? How is deletion of t propagated to the individual relations that contain only a subset of the attributes? Are all tuples removed that are the projection of t to the corresponding relation schema? Most likely this is a typo in Def 2.1 and it should be fixed to make clear that t is a tuple from any of the $R_i$.} \\

\revc{The reviewer is correct that the tuple $t$ can be added to or deleted from any of the input tables $R_i$, and not from the schema of the join output. We have updated Definition \ref{def:tuple_sens} and \ref{def:local_sens}.} \\

%\revc{We've modified Def 2.1 (SR) -- NEED TO EXPLAIN WHY THE PREVIOUS DEFN WAS CORRECT AND HOW WE MADE IT CLEARER.}

\textbf{(R4-D2)} \ques{In Fig 2, show the GYO decomposition steps to help readers who are less familiar with it.} \\

\revc{We added a brief description of the GYO decomposition steps in Figure \ref{fig:gyo}.} \\

\textbf{(R4-D3)} \ques{I did not understand the definition of the representative domain (Def 3.1) and it might have typos as well. The intuition seems clear: consider only the values from the active domain that are relevant for a relation based on relations it joins with. Add intuition and a concrete example that illustrates the definition.} \\

\revc{We added an intuition before Definition \ref{def:repr}, an example after Definition \ref{def:repr} and also fixed the typo in Definition \ref{def:repr}.} \\

\textbf{(R4-D4)} \ques{The proof of Thm 3.1 could probably be removed. It seems straightforward if one explains that the main issue is the insert operations and that there cannot be more than $n^k$ possible candidate tuples that need to be considered for insertion.} \\

\revc{The proof of Theorem \ref{thm:poly-data-complexity} 
is removed to make room for new material. The full proof will be in the full version.} \\

\textbf{(R4-D5)} \ques{The proof of Thm 3.2 would need a more comprehensive example to be really clear. I suggest removing it as well. It is not very surprising or interesting.} \\

\revc{The proof of Theorem \ref{thm:combined-nphard}  is removed as well to make room for new material. The full proof will be in the full version. We have also added a reference to Section 5.2 for some intuitions of hard acyclic queries.} \\

\eat{
\note{What should we do for Thm 3.2?} \\

\xh{We can have a shorter version of proof for Thm 3.2 to explain the approach and add a discussion why it is interesting. Have the full proof in the appendix or full paper.}
}

\textbf{(R4-D6)} \ques{In Sec 4, clarify if you are working with set or bag (multiset) semantics for the relations. If you use set semantics, then you have to be careful about the path query if relations contain additional attributes that could cause "duplicates" for the combinations of join attributes. Consider R1(A,B), R2(B,C), R3(C,D) vs R1(A,X,B), R2(B,Y,C), R3(C,Z,D). The former has at most $n^2$ results while the latter can have $n^3$. Clean up Sec 4 and clarify this.}\\

\revc{ Our framework considers bag semantics and not set semantics, duplicates are not eliminated. This is now clarified in Section \ref{sec:prelim}, Section 4.1, and also at the end of Section 5.2. } \\

%\note{Shall we clarify the bag semantics in the preliminary section?} \note{Shouldn't Fig 3 have illustrated this idea? Shall we add more descriptions in figure 3 to explain the intuition?}

\textbf{(R4-D7)} \ques{Sec 4.1 explains a nice and simple insight in a convoluted way. State the intuition more clearly and add a figure: For a tuple (x,y) in a relation, you determine the number of "incoming" paths ending at x and the number of "outgoing" paths starting at y. The product of those numbers is the local sensitivity for removing the tuple. Similar for inserting a new tuple (x,y).} \\ 

\revc{We added the intuition about "incoming" and "outgoing" paths in the example of Section \ref{sec:pj_simple_ineffi}. Due to the space constraint, we reuse the figure \ref{fig:path} to show the number of "incoming" and "outgoing" paths.} \\

\textbf{(R4-D8)} \ques{It seems that the main reason for algorithm complexity is the computation of upward tuple sensitivity, because many possible value combinations need to be considered. Explain this more clearly where complexity is analyzed in Sec 4 and Sec 5. And explain better what footnote 3 is trying to say.} \\

\revc{We agree with the reviewer that the algorithm complexity is mainly from considering the effect of tuple insertions, and we extended the discussion at the end of Section \ref{sec:pj_simple_ineffi} to show the complexity of considering all possible combinations of "incoming" and "outgoing" paths. }

\revc{Foornote 3 is replaced by explanations in text in the algorithm analysis of Section 4.2.} \\

\textbf{(R4-D9)} \ques{In Sec 4.2, show a simple figure to illustrate how $\top(R_{i+1})$ is computed from $\top(R_i)$.} \\

\revc{We modified Figure \ref{fig:path} to illustrate how to obtain the botjoin $\bot(R_3)$ from the botjoin $\bot(R_4)$ and $R_3$. We explain the details in Example~\ref{eg:pathjoin}. The transformation for the topjoins is similar.} \\

\textbf{(R4-D10)}\ques{ In Sec 5, what do you mean by "we also assume that each attribute appears in at least two relations in the body?" How is that possible for a path or tree?} \\

\revc{This assumption is used to simplified the algorithm analysis and is not necessarily needed. We added the following discussion at the end of Section \ref{sec:extensions}. 
For attributes that appear only once in the query body, we ignore them in Algorithm~\ref{algo:gj_query} but in the end we extrapolate a value for these attributes. 
} \\
 

\textbf{(R4-D11)}\ques{ In Sec 5.1, first state the intuition of what you want to compute before describing how you do it.} \\

\revc{We added the intuition and add example in Section \ref{sec:general-approach}.} \\

\textbf{(R4-D12)}\ques{ In 5.2, show a computation step according to Eq 15 in detail in a figure.} \\

\revc{We added descriptions in Figure \ref{fig:gj_notations} to illustrate the structure of a join tree and how a topjoin is iteratively computed.} \\

%\note{Shall we add more description in Fig 4? Or modify the figure to show one step. Maybe we can remove the left part of the figure, so can use the extra space to illustrate the step.} \\

%\xh{rather than adding more description in Fig 4, we can write the steps for Fig 4 in a bullet points form to clarify Eqn 15.}

\textbf{(R4-D13)}\ques{ I was not able to follow the discussion in Sec 5.4. Expand and clarify with examples or figures.} \\ 

\revc{We rewrote Section \ref{sec:extensions} and listed each extension in a single paragraph. One major extension, `general joins', is implemented in the experiment to support non-acyclic queries. Figure \ref{fig:queries} shows three non-acyclic queries $q3$, $\qtri$, and $\qcycle$ and their generalized hypertree decompositions.} \\

%\note{Add an example?} \\

%\xh{This might be addressed together with R2-R3's comments. We can reorganize and rewrite Sec 5.4. It sounds confusing to me as well. Let's go through it and see how to rewrite it. Do we have a query that need generalized hpyertree decomposition? }

\textbf{(R4-D14)}\ques{ TPC seems like a poor benchmark choice for the experiments. Doesn't it have uniform distributions all over? For realistic experiments, find real data or at least generate skewed input.} \\

\revc{%Please see the response to R1-D6.
We added a new dataset from SNAP, the ego network of Facebook, and prepared a triangle query $\qtri$, a 4-path query $\qpath$, a 4-cycle query $\qcycle$ and a star join query $\qstar$. The experiment results show that the sensitivity bound improvement of \TSens ranges from $\times 3$ to $\times 80k$, and \TSensDP achieves $< 6 \%$ error for the triangle, 4-path and cycle queries while \PrivSQL get $> 100\%$ error for the 4-cycle and star queries. 
} 

%\note{SNAP - Facebook social network data. The data is about ego-network for each user. Each user has a list of friends categorized into multiple circles (a circle table). Friends are also connected into a network (an edge table). Each friend also has a feature vector.

%We can divide the edge table into multiple small tables, so that each edge within one small table belongs to the same circle or cross the same two circles. For example, R0 contains edges from the circle 0. We can also have a triangle table contains triangles all from the same circle. For example, T3 contains triangles from the circle 3.

%Now we can write queries like R(A, B, C) :- R1(A, B), R2(B, C), R3(A, C), T4(A, B, C), which means the number of triangles in circle 4 but each edges also comes from circle 1, 2 and 3 separately.
%}

\balance

==> tables.tex <==
\begin{figure}[h]
\includegraphics[width=8cm]{figures/facebook_distribution.pdf}
\caption{Circle-edges distribution (facebook) }
\end{figure}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsens    & \elastic    & \tsens    & \elastic  & \tsens    & \elastic  & \tsens    & \elastic  \\ \hline
$s_1$	& 24	& 2430	& 38610	& 155520	& 1207	& 376200	& 19	& 996480	\\ \hline
$s_2$	& 76	& 7524	& 115650	& 376200	& 906	& 225720	& 19	& 1195776	\\ \hline
$s_3$	& 76	& 7524	& 115650	& 225720	& 218	& 65610	& 29	& 14008500	\\ \hline
$s_4$	& 42	& 2880	& 30780	& 65610	& 304	& 155520	& 29	& 13018800	\\ \hline
\end{tabular}
\caption{Local sensitivity of 4 query types under 4 query settings for TSens and Elastic. $\qtri$ is a triangle query, $\qpath$ is a path query of 4 nodes, $\qcycle$ is a 4-cycle query, $\qstar$ is a star query of 4 nodes}
\end{table*}
\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
\def\qtime{$Q(D)$}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{3}{l|}{$\qtri$} & \multicolumn{3}{l|}{$\qpath$} & \multicolumn{3}{l|}{$\qcycle$} & \multicolumn{3}{l|}{$\qstar$} \\ \cline{2-13} 
                  & \tsens    & \elastic    & \qtime    & \tsens    & \elastic  & \qtime    & \tsens    & \elastic  & \qtime    & \tsens    & \elastic  & \qtime    \\ \hline
$s_1$	& 0.109	& 0.004	& 0.111	& 0.215	& 0.009	& 0.164	& 0.506	& 0.008	& 0.459	& 0.311	& 0.007	& 0.175	\\ \hline
$s_2$	& 0.391	& 0.006	& 0.393	& 0.221	& 0.010	& 0.167	& 0.453	& 0.008	& 0.395	& 0.404	& 0.008	& 0.180	\\ \hline
$s_3$	& 0.440	& 0.007	& 0.391	& 0.227	& 0.010	& 0.177	& 0.115	& 0.005	& 0.132	& 0.371	& 0.059	& 0.184	\\ \hline
$s_4$	& 0.120	& 0.004	& 0.128	& 0.217	& 0.007	& 0.169	& 0.221	& 0.005	& 0.163	& 0.386	& 0.068	& 0.175	\\ \hline
\end{tabular}
\caption{Time of computing local sensitivity of 4 query types under 4 query settings for TSens, Elastic and query evaluation (in seconds).}
\end{table*}


\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsensdp    & \privatesql    & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  \\ \hline
$s_1$	& 7.97\%	& 179.53\%	& 17.17\%	& 8.49\%	& 0.34\%	& 238.20\%	& 6.20\%	& 95015.23\%	\\ \hline
$s_2$	& 10.03\%	& 39.53\%	& 2.00\%	& 2.59\%	& 16.06\%	& 614.71\%	& 13.94\%	& 70474.03\%	\\ \hline
$s_3$	& 0.99\%	& 43.46\%	& 4.16\%	& 5.89\%	& 63.67\%	& 744.56\%	& 1.77\%	& 599589.38\%	\\ \hline
$s_4$	& 41.45\%	& 53.73\%	& 40.58\%	& 15.50\%	& 41.94\%	& 862.41\%	& 8.60\%	& 734135.53\%	\\ \hline
\end{tabular}
\caption{Relative error of 4 query types under 4 query settings for TSensDP and PrivateSQL.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multicolumn{2}{l|}{$\qtri$} & \multicolumn{2}{l|}{$\qpath$} & \multicolumn{2}{l|}{$\qcycle$} & \multicolumn{2}{l|}{$\qstar$} \\ \cline{2-9} 
                  & \tsensdp    & \privatesql    & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  & \tsensdp    & \privatesql  \\ \hline
$s_1$	& 0.246	& 0.124	& 0.932	& 1.721	& 0.692	& 1.756	& 0.476	& 0.169	\\ \hline
$s_2$	& 0.456	& 0.219	& 1.108	& 6.604	& 0.568	& 0.802	& 0.516	& 0.182	\\ \hline
$s_3$	& 0.515	& 0.223	& 1.007	& 1.790	& 0.312	& 0.163	& 0.569	& 0.628	\\ \hline
$s_4$	& 0.255	& 0.123	& 0.589	& 0.350	& 0.362	& 0.250	& 0.558	& 0.673	\\ \hline
\end{tabular}
\caption{Computation time of 4 query types under 4 query settings for TSensDP and PrivateSQL (in seconds).}
\end{table*}


\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 1	& 10	& 30	& 50	& 100	& 1000	\\ \hline 
$s_1$ & 68	& 1.84\%	& 1.23\%	& 2.28\%	& 1.86\%	& 1.34\%	& 4.86\%	\\ \hline
\end{tabular}
\caption{Relative error of triangle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 100	& 10000	& 20000	& 30000	& 50000	& 100000	\\ \hline 
$s_1$ & 24552	& 4.89\%	& 4.79\%	& 4.96\%	& 4.56\%	& 6.71\%	& 8.14\%	\\ \hline
\end{tabular}
\caption{Relative error of 4path queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 10	& 100	& 500	& 1000	& 1500	& 10000	\\ \hline 
$s_1$ & 213	& 2.23\%	& 1.97\%	& 2.82\%	& 5.57\%	& 8.20\%	& 18.38\%	\\ \hline
\end{tabular}
\caption{Relative error of 4cycle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{setting} & \multirow{2}{*}{LS} & \multicolumn{6}{c|}{$\ell$} \\ \cline{3-8} 
&& 1	& 10	& 30	& 50	& 100	& 1000	\\ \hline 
$s_1$ & 13	& 5.15\%	& 4.23\%	& 16.88\%	& 56.14\%	& 31.74\%	& 98.46\%	\\ \hline
\end{tabular}
\caption{Relative error of 4star queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}



\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{1}	& \multicolumn{3}{c|}{10}	& \multicolumn{3}{c|}{30}	& \multicolumn{3}{c|}{50}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{1000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 68	& 41.0 &1.75\% & 1.84\%	& 43.0 &1.26\% & 1.23\%	& 39.0 &2.08\% & 2.28\%	& 41.0 &1.82\% & 1.86\%	& 43.0 &1.33\% & 1.34\%	& 64.0 &1.55\% & 4.86\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of triangle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{10000}	& \multicolumn{3}{c|}{20000}	& \multicolumn{3}{c|}{30000}	& \multicolumn{3}{c|}{50000}	& \multicolumn{3}{c|}{100000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 24552	& 17396.5 &4.90\% & 4.89\%	& 17496.5 &4.80\% & 4.79\%	& 17471.5 &4.90\% & 4.96\%	& 17746.0 &4.39\% & 4.56\%	& 16094.0 &6.96\% & 6.71\%	& 15574.5 &8.18\% & 8.14\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4path queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{10}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{500}	& \multicolumn{3}{c|}{1000}	& \multicolumn{3}{c|}{1500}	& \multicolumn{3}{c|}{10000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 213	& 163.5 &2.24\% & 2.23\%	& 167.0 &1.83\% & 1.97\%	& 163.0 &2.24\% & 2.82\%	& 144.5 &5.50\% & 5.57\%	& 146.0 &5.35\% & 8.20\%	& 230.5 &2.90\% & 18.38\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4cycle queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}

\begin{table*}[t!]
\tiny
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsensdp{TSensDP}
\def\privatesql{PrivateSQL}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{3}{*}{setting} & \multirow{3}{*}{LS} & \multicolumn{18}{c|}{$\ell$} \\ \cline{3-20} 
&& \multicolumn{3}{c|}{1}	& \multicolumn{3}{c|}{10}	& \multicolumn{3}{c|}{30}	& \multicolumn{3}{c|}{50}	& \multicolumn{3}{c|}{100}	& \multicolumn{3}{c|}{1000}	\\ \cline{3-20} 
&& GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err & GS & Bias & Err \\ \hline 
$s_1$ & 13	& 11.0 &3.18\% & 5.15\%	& 13.0 &0.83\% & 4.23\%	& 9.0 &12.72\% & 16.88\%	& 4.0 &54.58\% & 56.14\%	& 48.0 &0.00\% & 31.74\%	& 160.0 &0.00\% & 98.46\%	\\ \hline
\end{tabular}
\caption{Average global sensitivity, relative bias error and relative total error of 4star queries under 4 query settings across different esitmated tuple sensitivity bound $\ell$ for TSensDP. The corresponding local sensitivity is shown for each query.}
\end{table*}


\clearpage
\onecolumn

%\begin{table*}[t!]
%\usepackage{longtable}
%for \Yup
%\usepackage{stmaryrd}
%for \square \sqcap
%\usepackage{mathabx}
\def\qtri{q_\triangle}
\def\qpath{q_\sqcap}
\def\qcycle{q_\square}
\def\qstar{q_\Yup}
\def\tsens{TSens}
\def\elastic{Elastic}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\begin{longtable}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
qtype & setting & $|IN|$ & $|\reprdomain|$ & $|OUT|$ & relations & $|IN|$ & $\reprdomain$ & attr & $\actdomain$ & $\reprdomain$ & mf \\ \hline
\endhead
\multirow{6}{*}{$\qtri$} & \multirow{6}{*}{$s_1$} & \multirow{6}{*}{13520} & \multirow{6}{*}{62257} & \multirow{6}{*}{30699} & \multirow{2}{*}{source\_348\_circle\_dabfae} & \multirow{2}{*}{6830} & \multirow{2}{*}{13857} & A & 200 & 93 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 149 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_4d72cf} & \multirow{2}{*}{4818} & \multirow{2}{*}{18600} & C & 149 & 93 & 76 \\ \cline{9-12} 
& & & & & & & & B & 149 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_cd20fc} & \multirow{2}{*}{1872} & \multirow{2}{*}{29800} & C & 93 & 149 & 68 \\ \cline{9-12} 
& & & & & & & & A & 93 & 200 & 68 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{8}{*}{$\qpath$} & \multirow{8}{*}{$s_1$} & \multirow{8}{*}{14146} & \multirow{8}{*}{27391} & \multirow{8}{*}{17555419} & \multirow{2}{*}{source\_348\_circle\_dabfae} & \multirow{2}{*}{6830} & \multirow{2}{*}{0} & A & 200 & 0 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 149 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_4d72cf} & \multirow{2}{*}{4818} & \multirow{2}{*}{18600} & C & 149 & 93 & 76 \\ \cline{9-12} 
& & & & & & & & B & 149 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_cd20fc} & \multirow{2}{*}{1872} & \multirow{2}{*}{8791} & C & 93 & 149 & 68 \\ \cline{9-12} 
& & & & & & & & D & 93 & 59 & 68 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_9939a6} & \multirow{2}{*}{626} & \multirow{2}{*}{0} & E & 59 & 0 & 43 \\ \cline{9-12} 
& & & & & & & & D & 59 & 93 & 43 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{8}{*}{$\qcycle$} & \multirow{8}{*}{$s_1$} & \multirow{8}{*}{14146} & \multirow{8}{*}{54782} & \multirow{8}{*}{142903} & \multirow{2}{*}{source\_348\_circle\_dabfae} & \multirow{2}{*}{6830} & \multirow{2}{*}{8791} & A & 200 & 59 & 99 \\ \cline{9-12} 
& & & & & & & & B & 200 & 149 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_4d72cf} & \multirow{2}{*}{4818} & \multirow{2}{*}{18600} & C & 149 & 93 & 76 \\ \cline{9-12} 
& & & & & & & & B & 149 & 200 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_cd20fc} & \multirow{2}{*}{1872} & \multirow{2}{*}{8791} & C & 93 & 149 & 68 \\ \cline{9-12} 
& & & & & & & & D & 93 & 59 & 68 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_9939a6} & \multirow{2}{*}{626} & \multirow{2}{*}{18600} & D & 59 & 93 & 43 \\ \cline{9-12} 
& & & & & & & & A & 59 & 200 & 43 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline\multirow{9}{*}{$\qstar$} & \multirow{9}{*}{$s_1$} & \multirow{9}{*}{18272} & \multirow{9}{*}{16008} & \multirow{9}{*}{786} & \multirow{2}{*}{source\_348\_circle\_dabfae} & \multirow{2}{*}{6830} & \multirow{2}{*}{899} & A & 29 & 29 & 99 \\ \cline{9-12} 
& & & & & & & & B & 28 & 31 & 99 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_4d72cf} & \multirow{2}{*}{4818} & \multirow{2}{*}{812} & C & 17 & 29 & 76 \\ \cline{9-12} 
& & & & & & & & B & 31 & 28 & 76 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{2}{*}{source\_348\_circle\_cd20fc} & \multirow{2}{*}{1872} & \multirow{2}{*}{493} & C & 29 & 17 & 68 \\ \cline{9-12} 
& & & & & & & & A & 29 & 29 & 68 \\ \cline{9-12} 
 \cline{6-12} 
& & & & & \multirow{3}{*}{tri\_source\_348\_circle\_9939a6} & \multirow{3}{*}{4752} & \multirow{3}{*}{13804} & C & 54 & 17 & 362 \\ \cline{9-12} 
& & & & & & & & A & 54 & 29 & 362 \\ \cline{9-12} 
& & & & & & & & B & 54 & 28 & 362 \\ \cline{9-12} 
 \cline{6-12} 
\cline{2-12} 
\hline
\caption{Query meta stat for queries of 4 settings from 4 types. $\qtri$ is a triangle query, $\qpath$ is a path query of 4 nodes, $\qcycle$ is a 4-cycle query, $\qstar$ is a star query of 4 nodes}
\end{longtable}
%\end{tabular}
%\end{table*}

\clearpage
\twocolumn

==> tail.tex <==
\am{Some thoughts on this section:
\squishlist
\item Shorten the intro. Add section headers: dataset, queries, ...
\item Divide the experiments into two subsection: Local sensitivity and DP query answering. You can talk about elastic sensitivity and runtime in the first subsection, and PrivSQL in the second subsection
\item I did not understand how you construct the most sensitive tuple for elastic? Just drop it from the experiments for now and just compare the LS. 
\item Some of the graphs like Fig 7 can be dropped. 
\item Is there way to make figure 6 smaller. Do we need all the information there? 
\item The description is sometimes very verbose and sometimes too concise. 
\squishend}

==> tech.tex <==
\section{Relaxation}
Recall that we have shown the time complexity for computing $\botjoin$ and $\topjoin$ is $O(n 
\log n (deg^*-1)$. When $n$ is large, the algorithm can still take a long time to stop. Here we present a way to speed up the computation by relaxing the information completeness. Instead of storing frequencies for each domain value, we only keep top $k$ frequencies and thus reduce the storage of $\topjoin$ and $\topjoin$ and their computation time.

Denote $\topk{k}{A}$ as an operator that takes k tuples from the table with top $A$ values. We define this operator by this algorithm:

\begin{algorithm}
	\caption{$\topk{k}{A}$ algorithm}
	\label{algo:new_ls_pathquery}
	\begin{algorithmic}[1]
		\Require A table of size $n$, $k$ and $A$
		\Ensure  Top k tuples about $A$
		\State create a min-heap $H$ of size k
		\For{each tuple $t$}
		    \If{$t[A] <$ H.getMin()$[A]$}
		        \State{H.extractMin()}
		        \State{H.insert($t$)}
		    \EndIf
		\EndFor
	\end{algorithmic}
\end{algorithm}

If the size of the input table is $n$, the time complexity of $\topk{k}{A}$ is $O(n\log k)$

Now, we redefine the invariant definition of $\botjoin$ and $\topjoin$ as:
\begin{align}
\ktopjoin(\R{i}) &=  \topk{k}{\cnt{r}{i}}(\topjoin(\R{i})) \\
\kbotjoin(\R{i}) &=  \topk{k}{\cnt{l}{i}}(\botjoin(\R{i}))
\end{align}

The recursive approach of computing $\botjoin$ and $\topjoin$ is the same, except that when you do a join, if it joins a NULL attribute, we change the corresponding counting attribute $C$ by default as the minimum frequency of another top k table.

\todo{Add a algorithm box to explain this special join behavior}

\begin{theorem}
The time complexity of $\ktopjoin$ and $\kbotjoin$ is $O(nk  $ $\log k (deg^*-1) )$. The size of $\ktopjoin$ and $\kbotjoin$ is $k$.
\end{theorem}

\begin{proof}
For each join in the star join, the sizes of two tables are $O(n)$ and $O(k)$, so the join complexity is $O(nk)$. Since there are at most $O(deg^*-1)$ joins in a star join, the time complexity is $O(nk(deg^*-1))$. The last $\topk{k}{\cdot}$ operation makes the entire complexity as $O(nk(deg^*-1)\log k)$
\end{proof}

To find the most sensitive tuple, we define

\begin{align}
    \kstartuple_{i, j} = 
\begin{cases}
    \argmax_{t \in \kbotjoin(\R{j})}
        t[C_{i, j}]
        &, j \in C(i) \\
    \argmax_{t \in \ktopjoin(\R{i})}
        t[C_{i, j}]
        &, j = p(i)
\end{cases}
\end{align}

\begin{align}
    \kstartuple_i = 
\begin{cases}
\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\kstartuple_{i,j} \mid j \in C(i) \cup \{ p(i)\} \}) &, other \\
\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\kstartuple_{i,j} \mid j \in C(i) \}) &,  \text{$R_i$ is the root} \\
\pi_{A_{i}, \underset{j}{\product} C_j \as \tsens_i} (\{\kstartuple_{i,j} \mid j \in \{ p(i)\} \}) &, \text{$R_i$ is a leaf}
\end{cases}
\end{align}

\begin{theorem}
The time complexity to find the most sensitive tuple and the local sensitivity of a acyclic join query by relaxation parameter $k$ is $O(mnk  $ $\log k (deg^*-1) )$.
\end{theorem}

\begin{proof}
Since there are $m$ $\ktopjoin$ and $\kbotjoin$ to compute, it takes $O(mnk  $ $\log k (deg^*-1) )$. To find $t^*_i$, it takes another $O(mk(deg^*-1))$ time. In conclusion, the time complexity is $O(mn \log n (deg^*-1))$.
\end{proof}

\subsection{SPJ- Queries}

We only consider cases that S and P happen before J. This doesn't change the conclusion of path joins and acyclic joins.

\subsection{General Queries}

\todo{
Can we find a representative sub domain for a general query?
}

\subsection{Baseline}

The elastic sensitivity \cite{DBLP:journals/corr/JohnsonNS17} describes a fast way to compute an upper bound of the local privacy. We will show that when k=1, our relaxed tuple sensitivity computation can find the same bound as the elastic one. 

\todo{Analyze the algorithm of the elastic sensitivity. Prove our maximum tuple sensitivity equals to that result.}

\note{Our algorithm can also find the most sensitive tuple when k = 1. Use it as the baseline}







